Upfront Commitment in Online Resource Allocation with Patient Customers

In many on-demand online platforms such as ride-sharing, grocery delivery, or shipping, some arriving agents are patient and willing to wait a short amount of time for the resource or service as long as there is an upfront guarantee that service will be ultimately provided within a certain delay. Motivated by this, we present a setting with patient and impatient agents who seek a resource or service that replenishes periodically. Impatient agents demand the resource immediately upon arrival while patient agents are willing to wait a short period conditioned on an upfront commitment to receive the resource. We study this setting under adversarial arrival models using a relaxed notion of competitive ratio. We present a class of POLYtope-based Resource Allocation (POLYRA) algorithms that achieve optimal or near-optimal competitive ratios. Such POLYRA algorithms work by consulting a particular polytope and only making decisions that guarantee the algorithm's state remains feasible in this polytope. When the number of agent types is either two or three, POLYRA algorithms can obtain the optimal competitive ratio. To design these polytopes, we construct an upper bound on the competitive ratio of any algorithm, which is characterized via a linear program (LP) that considers a collection of overlapping worst-case input sequences. Our designed POLYRA algorithms then mimic the optimal solution of this upper bound LP via its polytope's definition, obtaining the optimal competitive ratio. When there are more than three types, our overlapping worst-case input sequences do not necessarily result in an attainable competitive ratio, and so we present a class of simple and interpretable POLYRA algorithm which achieves at least 80% of the optimal competitive ratio. We complement our theoretical studies with numerical analysis which shows the efficiency of our algorithms beyond adversarial arrivals

==> body.tex <==







==> intro_related_works.tex <==
% Title Ideas 

% Main Idea: Online Resource Allocation with Flexible/Patient Agents who Require Upfront Commitment 
% Leveraging Patience at the Cost of Commitment in Online Resource Allocation
% Promising Future Resources to Patient Customers in Online Resource Allocation 
% Online Resource Allocation with Partially Patient Customers 


%\textbf{Title Proposal: Online Resource Allocation with Partially Patient Customers} 



==> sections/1_-_intro.tex <==
\section{Introduction}
{\color{black}Online resource allocation is a fundamental problem that arises in almost every {\color{black}industry} from government and healthcare (e.g., during a pandemic crisis), to e-commerce and online services. In such problems, the decision-maker strives to best allocate a set of scarce resources to agents with varying levels of value. While even an offline resource allocation problem can be difficult, the online setting brings extra challenges because we must make irrevocable decisions without having full information regarding the future. The critical property of the online setting is that arriving agents must be allocated the resource immediately or otherwise leave the system forever. Such a property creates the following trade-off: allocating a resource now to a low-value agent has a potential opportunity cost in the future, while saving resources for the future can hurt if no higher-valued agents arrive.}

{
\color{black}
In practical applications, one way of mitigating the challenge of the online setting is to exploit agents' patience. The assumption that all agents demand the resource immediately can be relaxed if some agents are patient and willing to wait a short period  for the resource. If a decision-maker were able to delay the acceptance/rejection decision for patient agents, then they would be certainly able to make better decisions as they can observe more of the demand. However, in many applications, it is unreasonable to assume that  agents are willing to wait for a resource and risk being ultimately rejected. This is especially true in the allocation of scarce services in on-demand online platforms such as ride-sharing, grocery delivery, or shipping. An agent may agree to receive their ride, grocery, or package within a longer time window, but only if there is an upfront guarantee that service will be ultimately provided within this window. We refer to such agents who are patient only if provided with an upfront guarantee as \textit{partially patient} or flexible. 

The existence of partially patient agents is challenging because we face a new dilemma: accepting a partially patient agent results in greater short-term flexibility in our decision-making process, but it comes at the cost of a future resource commitment that  cannot be allocated to a future higher-reward agent. We present a novel model for online resource allocation with the existence of such partially patient agents and  provide simple algorithms which achieve optimal or near-optimal performance under an adversarial arrival process.
}





\subsection{Our Contributions}
We describe the contributions of our work as follows.
 
{\color{black}\textbf{A novel extension of a classic revenue management model to include partially patient agents who require commitment (Section \ref{sec:model}).} A famous model for online resource allocation is the single-leg revenue management model under adversarial arrivals by \cite{BallandQueyrenne2009}. In this problem, a decision-maker has  $C$ units of a single resource and must allocate them to arriving agents with heterogeneous rewards $r_1 < \ldots < r_K$ in an online fashion. The goal is to design algorithms which maximize the competitive ratio, the worst-case ratio of an online algorithm's cumulative reward to that of a clairvoyant optimal solution that knows the arrival sequence in advance. We present an extension of this model with the following main modifications, which we define formally in Section \ref{sec:model}.}


\begin{itemize} [leftmargin=*]
    \item {\color{black}\textbf{Multiple periods with partially patient agents. } We generalize the model to a multi-period setting with $T \geq 1$ periods, during each of which agents arrive in an online fashion. Each time period $t \in [T]$ is divided into an arrival phase and service phase. During the arrival phase, agents arrive in an online fashion and we still must make an irrevocable decision about whether  to accept or reject each one. During the service phase, we must choose how to allocate the $C$ capacity we have in each period to the accepted agents.  When an agent is accepted, we provide an upfront \textit{commitment} to providing service to that agent in the near future. Agents in our new model differ not only in terms of reward but also in their level of patience. Out of these $K$ types of agents, the first $M$ are partially patient, while the remaining $K-M$ are impatient. For impatient agents accepted in period $t \in [T]$, they must be serviced in period $t$'s service phase.  For any accepted partially patient agents in time period  $t \in [T]$,  we are committed to serving  them either in  period $t$ or $t+1$'s service phase. See Section \ref{sec:application} for more details.}
    

    
    \item {\color{black}\textbf{Competitive ratio (CR) definition.} While we continue to study adversarial arrival sequences, we employ a relaxed CR analysis called \textit{resource augmented CR}. Introduced by \cite{kalyanasundaram2000speed}, this relaxed notion of CR (that {\color{black}we refer to} as feature-augmented CR) bounds the worst-case performance of an online algorithm augmented with an additional feature versus an optimal offline solution that cannot utilize the feature. In our case, the feature is the time-flexibility of the first $M$ types of agents. Such a relaxed  notion of CR is standard/common in the literature (see e.g, \cite{resource_augmentation_1, resource_augmentation_2, resource_augmentation_3} or \cite{roughgarden} for a survey) and is often necessary to characterize the benefit of an additional feature because features often disproportionately benefit the offline clairvoyant benchmark, resulting in a decreased {\color{black}CR} after introducing the feature (see Section \ref{sec:resource_augmented_cr} for details). As we will show in this work, considering this relaxed notion of CR results in  practical and easy-to-implement algorithms with great performance in realistic scenarios under both feature-augmented and traditional notions of CR  (see our numerical studies in Section \ref{sec:numerical_studies}).}  
\end{itemize}





\textbf{Polytope-based resource allocation (POLYRA) algorithm (Section \ref{sec:polyra}).} We present a general class of resource allocation algorithms that consist of two components: a state $\stateB$ and a feasible region $\feasible$. At any moment in the arrival sequence, the state $\stateB$ encapsulates all the decisions the algorithm has made so far. For our specific model, $\stateB$ keeps track of the number of agents of each type that the algorithm has accepted but not yet served, including how many of them require resource in the current time period. A \po{} algorithm makes decisions in a greedy fashion while maintaining the invariant that $\stateB \in \feasible$; see Section \ref{sec:polyra} for more details. By cleverly defining the state $\stateB$ and constructing the feasible polytope $\feasible$, we design optimal or near-optimal algorithms for our model. (We will provide more details later.) {\color{black}Some of our designed algorithms---called nested \po{} algorithms---have a simple \emph{nested} structure and can be viewed as an extension of the nested booking policies from \cite{BallandQueyrenne2009} that are designed for a setting without flexibility.
The nested booking policies  reserve a capacity for higher reward agents in a nested fashion. We generalize this notion of nested booking limits to our multi-period setting with partially patient agents through the definition of a nested polytope (Definition \ref{def:nested}). This generalization also leads to the following benchmark algorithm.}

{\color{black}\textbf{Benchmark algorithm.}
The key challenge in designing a nested booking policy is choosing the size of the booking limits, or nests as we will refer to them. The  benchmark algorithm that we refer to as the \emph{BQ nested \po{} algorithm} uses the nest sizes from the nested booking policies of \cite{BallandQueyrenne2009}, which are designed to achieve good performance in a setting without partially patient agents. We will compare this benchmark algorithm with our nested \po{} algorithms whose nest sizes are carefully optimized through solving a linear program (LP). Theoretically, we show that optimizing these nest sizes results in a strictly better theoretical performance in terms of feature augmented CR. (See Theorem \ref{theorem:our_alg_beats_bq}.) {\color{black} Numerically, we show that our optimized nested \po{} algorithms outperform the BQ nested \po{} algorithm in terms of both the our feature-augmented CR as well as the more traditional CR definition (Section \ref{sec:numerical_studies}). While obtaining a higher feature-augmented CR was expected given our theoretical results, it is quite interesting that our optimized nested \po{} algorithms yield higher traditional CR than the BQ nested \po{} algorithm.}}
 

\textbf{Optimality of POLYRA algorithms for two types (Section \ref{section:two_type}).} When there are two types of agents with rewards $r_1 < r_2$ and type 1 partially patient and type 2 impatient, we characterize a simple nested \po{} algorithm that achieves the optimal {\color{black}feature-augmented}  
CR of $\frac{2}{3 - r_1/r_2}$ (Theorem \ref{thm:opt_2}). 
In contrast, our benchmark, the BQ nested \po{} algorithm obtains a strictly smaller CR of $\frac{1}{2 - r_1/r_2}$. {\color{black}We present a concrete example (Example 
\ref{example:two_types}) demonstrating why optimizing the nest sizes is crucial to achieve the higher CR, compared with the BQ nested \po{} algorithm.}



\textbf{Optimal POLYRA algorithms with three types (Section \ref{section:three_type}).} When there are three types of agents with one  or two partially patient types, we present two {\color{black}(feature-augmented CR)} optimal \po{} algorithms with feasible polytopes $\feasible^{(K, M)}$ for $K =3$ and $M\in \{1, 2\}$.  See Theorem \ref{thm:opt_alg_M=1} for  $\feasible^{(3, 1)}$ and  Theorem \ref{theorem:three_type_M=2} for $\feasible^{(3, 2)}$. To design both these feasible polytopes, we first present an upper bound on the feature-augmented CR of any non-anticipating resource allocation algorithm (Theorem \ref{thm:3_type_upper_bound}). This upper bound, which is characterized by an LP, is constructed by considering four overlapping arrival sequences (across two time periods) that are truncated versions of a particular worst-case arrival sequence. Our \po{} algorithms then mimic the optimal solution to this LP in constructing their feasible polytopes, yielding the optimal CR. Interestingly, the feasible polytope $\feasible^{(3, 1)}$  is not  of the simple nested structure (as per Definition \ref{def:nested}), highlighting the challenges of exploiting agents' temporal flexibility optimally beyond two types of agents. We provide intuitions for why this is the case in Section \ref{section:three_type}.


%{\color{black}\textbf{Optimality of POLYRA algorithms for two and three types (Sections \ref{section:two_type} and \ref{section:three_type}).} For two types of agents, with rewards $r_1 < r_2$ and distinct patience levels, we introduce a nested \po{} algorithm yielding an optimal feature-augmented CR of $\frac{2}{3 - r_1/r_2}$ (Theorem \ref{thm:opt_2}), surpassing the BQ nested \po{} algorithm's CR. An example (Example \ref{example:two_types}) elucidates the significance of optimizing nest sizes. For three agent types (K=3), we propose optimal \po{} algorithms associated with polytopes $\feasible^{(K, M)}$ for $M\in \{1, 2\}$. The upper bound on the feature-augmented CR is derived from a particular worst-case sequence and an associated LP, guiding our \po{} algorithms to achieve the optimal CR. Notably, the structure of $\feasible^{(3, 1)}$ deviates from the standard nested form, underlining complexities when addressing beyond two agent types. Further insights are detailed in Section \ref{section:three_type}.}

\textbf{Near optimality of nested POLYRA algorithms for more than three types (Section \ref{section:beyond_three}).} When there are at least four types of agents, a generalization of our upper bound LP from three types is no longer tight as it is difficult to characterize the worst-case input sequence. Considering this challenge, we turn our attention back to the class of nested polytopes and show that finding the nested polytope with the highest CR  of $\crr_{\text{nest}}^*$ can be done by solving a simple LP (Theorem \ref{theorem:polyra_nested_performance}). We also show that while characterizing a tight upper bound is challenging, we can easily characterize a looser upper bound $\crr_{\text{up}}$ on the CR of any non-anticipating algorithm for any number of types (Theorem \ref{thm:loose_upper_bound}). Finally, we show that $\crr_{\text{nest}} / \crr_{\text{up}} \geq 0.8$, which proves that the class of nested polytopes is near-optimal (Theorem \ref{thm:optimality_gap}) in the sense that it obtains at least $80\%$ of the optimal CR.


{\color{black} \textbf{Numerical Studies (Section \ref{sec:numerical_studies}).} %{\color{red} updated this } 
We've undertaken extensive numerical studies to supplement our theoretical findings. Specifically, when contrasting our optimized nested \po{} algorithm with the BQ nested \po{} algorithm, both under traditional and feature-augmented CRs, the results are illuminating. Our algorithm clearly outpaces the BQ nested \po{} algorithm across both metrics, with improvements ranging from 1\% to 19\% in average (traditional) CR and up to 45\% in worst-case (traditional) CR, highlighting its superior capability in harnessing flexibility.

To ensure a holistic understanding, we evaluated our algorithm's performance against the BQ nested \po{} algorithm in terms of the distribution of traditional CRs, and notably, in its worst-case value. The results are consistent: our algorithm stochastically surpasses the BQ nested \po{} algorithm in the distribution of traditional CRs, a trend that also holds for the feature-augmented CR. 



%We complement our theoretical results under adversarial arrivals with numerical studies under stochastic arrivals. We compare our optimized nested \po{} algorithm against the BQ nested \po{} benchmark algorithm, which is not designed with flexible agents in mind. 
% Using both the feature-augmented CR and the traditional CR definitions, our algorithm consistently outperforms the benchmark. The improvement ranges from 1\% to 19\% for the average empirical (traditional) CR and reaches up to 45\% for the worst-case scenario. Additionally, we observe that the difference in performance grows linearly with the increase in the number of flexible types and the volatility of the arrival sequence. These results emphasize the importance of algorithms tailored for flexible agents and highlight the value of flexibility in obtaining better performance.
 
%Under both our feature-augmented CR definition as well as a more standard CR definition, our algorithm significantly outperforms the benchmark, improving the average empirical CR of 1\% to 19\% and the worst-case empirical CR by up to 45\%. In particular, we observe that this performance gap increases linearly with the number of flexible types as well as with amount of volatility in the arrival sequence. Our results highlights the need to design algorithms specifically designed for flexible agents as well as the value of flexibility in creating robustness.

% % Both our optimized nested algorithm and the BQ nested algorithm achieve CRs that are higher than our theoretical worst-case guarantees. 
% , our optimized nested \po{} algorithm improves the average empirical CR by $1\%$ to $19\%$ and improves the worst-case empirical CR by up to $45\%$. This improvement is associated with as the number of flexible types as well as variability in the arrival sequences. 




\subsection{Managerial Insights}
 Together, our theoretical results and numerical studies lead to the following managerial insights.

\textbf{Trade-off between commitment and flexibility.} The presence of partially patient customers, who require an upfront commitment, presents a unique trade-off between \textit{flexibility in the current period} and \textit{burden in future periods}. An effective algorithm must delicately balance this trade-off: while accepting many partially flexible agents (with low rewards) provides robustness against uncertainty in the current period's arrival sequence, the commitment to serve such agents places a burden on future resources. Despite the inherent challenges in understanding this trade-off, our study offers optimal or near-optimal algorithms that achieve this delicate balance.

\textbf{Recognizing Flexibility in Algorithm Design and its Value.} The enhanced performance of our optimized nested \po{} algorithm, compared to the BQ nested \po{} algorithm, accentuates the significance of tailoring algorithms with flexible agents in consideration. While flexibility is undeniably valuable, it necessitates thoughtful exploitation. Our numerical analyses affirm this: our approach consistently surpasses the BQ nested \po{} algorithm in both feature-augmented and traditional CR metrics. Moreover, our findings underscore the intrinsic value of flexibility. Introducing flexibility has been observed to boost the traditional CR by margins ranging from 0.8\% to 12\%, contingent on the number of flexible agents $M$ and fluctuations in the arrival sequence. Notably, the gain amplifies with an increase in both $M$ and sequence volatility.



\textbf{Merits of increased flexible types.} Our findings challenge the widely accepted idea that ``a little bit of flexibility goes a long way." In contrast, as we introduce more flexible agent types, the growth in both the traditional and feature-augmented CRs remains linear, not showing signs of diminishing returns. This suggests that businesses stand to gain by encouraging a broader base of customers to adopt flexibility.

\textbf{Design of simple nested policies.} Nested booking limit policies are a proven approach for resource allocation in traditional settings without flexible agents. Our research indicates that such a paradigm can be extended to settings with partially flexible agents. Although the introduction of partially flexible agents adds complexity to the optimization of the nested booking limits, we demonstrate that this optimization is tractable, resulting in algorithms that achieve strong performance both theoretically and empirically.

\textbf{Adversarial design enhancing real-world performance.} Designing algorithms with adversarial arrivals as a foundation often proves beneficial, even in more typical stochastic environments. Essentially, these algorithms, primed for worst-case scenarios, tend to outshine expectations in standard conditions, a trend our numerical studies echo. Delving into the intricacies of arrival sequence volatility in our numerical studies, we observed performance pressures on both our algorithm and the BQ nested \po{} algorithm as volatility surges. However, as volatility escalates, the performance disparity between our algorithm and the BQ nested \po{} algorithm grows more pronounced. This emphasizes the pivotal role flexibility plays in managing unpredictable agent inflows. Moreover, our algorithm often surpasses its theoretical benchmarks, especially in the context of the feature-augmented CR.
}

% \begin{itemize}
% \item \textbf{Agent patience and online decision-making.}
% In practical scenarios, recognizing agent patience is vital for optimizing online resource allocation. Delaying decisions for patient agents enhances allocation outcomes by revealing demand patterns. Yet, not all agents are patient, especially in on-demand platforms, where they seek upfront service guarantees. This emphasizes the need to understand diverse agent behaviors, like patience, in resource allocation. Our numerical results underscore that neglecting agent flexibility can substantially impact performance. {\color{red} let's add sth to the}

% \item \textbf{Trade-off: commitment vs. agent flexibility.} A critical trade-off emerges when dealing with flexible agents. Accepting partially patient agents offers short-term flexibility but commits resources for future service. As our comparison with the BQ nested \po{} algorithm shows, this balance between commitment and agent flexibility is central to optimizing resource
% allocation

% \item \textbf{Extending nested policies with flexibility.}
% Nested policies are a proven approach for resource allocation in traditional settings without flexible agents. Our research successfully extends nested policies to accommodate flexible agents, maintaining their robust performance. Introducing partially patient agents adds complexity, but our work demonstrates that optimal or near-optimal policies remain practical and effective.
% \end{itemize}


==> sections/2_-_related_works.tex <==

\section{Related Works}\label{sec:related_work}
Our work fits in with existing literature in the following research areas:

\textbf{Single-leg revenue management.} Our work is an extension of the single-leg revenue management (RM) problem to a setting where agents not only have different rewards, but also different temporal flexibility levels. The single-leg RM problem, which is a fundamental RM problem, involves allocating multiple units of a single resource to arriving agents of various types (i.e. demand), each with some fixed reward. The main challenge is deciding in an online fashion how many low-reward agents to accept while making sure there is enough capacity for potential higher-reward agents. A classic result from \cite{littlewood1972} shows that the optimal number of lower type agents to accept can be given by a simple threshold-based policy. Extensive further work has been done on this model, with numerous variations such as adding a network resource structure,  customers' choice models, and sample information and machined-learned advice about the arrival process (see e.g., \cite{ Talluri1998Network, Talluri2004choicemodel, Perakis2010Robust, golrezaei2014real,Gallego2015OnlineCustomerChoice, Ke2019networkRMpricing, Ma2020Network, Sun2020QBNRM, golrezaei2022online, balseiro2022single, golrezaei2023online}, and \cite{Strauss2018ChoiceSurvey} for a survey). 

\textbf{Adversarial demand modeling.} Most previous work in the single-leg RM problem and its variations model demand using a stochastic process (e.g. \cite{asadpour2020limitedflexibility, Talluri1998Network, Talluri2004choicemodel}) or robust uncertainty sets (e.g. \cite{Perakis2010Robust,birbil2006robust}). In both cases, we must make certain assumptions about how demand behaves. However, in an adversarial framework with CR analysis, no assumptions about demand are made as the performance of any algorithm is given by its worst-case performance over any possible demand arrival. One of the first lines of work in adversarial demand modeling was \cite{BallandQueyrenne2009}, whose work is a special case of our model. The authors show that the optimal policy initially accepts all arriving agents, but gradually only accepts higher reward agents once certain capacity thresholds are reached. Their solution structure is similar to that of Littlewood in that both reserve a certain fraction of the capacity exclusively for higher type reward agents, but differ in that the thresholds are set based on knowing the demand distribution, {\color{black}not only based on the ratios between agent rewards}. Other works in this area have explored variations such as setting posted prices instead of making binary accept/reject decisions in \cite{eren2010pricing}, relaxing the adversarial arrival order by assuming that {\color{black} part of the arrival sequence} is stochastic in \cite{Hwang2018partiallypredictable} or by removing the assumption of independent demand classes (the idea that higher type agents never choose the lower-priced option) in \cite{ma2021singleleg}. Our work contributes to the literature on adversarial single-leg RM problems by studying how to optimally exploit  demand time-flexibility in  adversarial single-leg RM problems.  

Our work is also related to the literature on flexibility. Papers in this area can be divided into three streams: supply side, demand side, and time-based flexibility. 
% candidate for deletion in the online version (these other types of flexibility are not really as relevant since we have so much timing flexibility discussion)

\textbf{Supply-side flexibility. } Supply side flexibility refers to the ability of a firm to satisfy demand for a product with more than a single combination of raw goods or underlying resources. This kind of production-side flexibility has been well studied in the literature. In particular, it has been shown that a limited amount of flexibility (e.g. the long chain design) is almost as good as a fully flexible system (see e.g. \cite{jordan1995principles,simchi2012understanding, simchi2015worst, desir2016sparse, chen2019optimal, devalve2021understanding}). (See \cite{petrick2012survey} for a survey).\footnote{See also \cite{mak2009stochastic,lu2015reliable, shen2019reliable} for works that study supply-side flexibility in the presence of disruptions to  demand and supply and \cite{armony2004customer,castro2020matching} for works that study flexibility in queuing systems.} While most work understanding production-side flexibility has been in an offline setting, the adage ``a little flexibility goes a long way'' also seems to be true in the online setting from \cite{asadpour2020limitedflexibility}. 

\textbf{Demand-side flexibility. }On the other hand, demand-side flexibility refers to customers' willingness to accept one of many products that are usually considered substitutes (e.g. two flights that depart within an hour). The main insights from consumer flexibility is that when customers reveal their indifference to a firm (sometimes for a discount or incentive), it greatly improves capacity utilization by helping the firm overcome uncertainty as seen in \cite{Gallego2004FlexibleProducts}. In addition, the potential discount offered also induces more demand as a larger segment of the population may now be able to afford the good or service. One concrete example of demand-side flexibility is the idea of opaque products in which customers specify a bundle of specific goods that they are indifferent between (such as the color of a notebook) and the firm chooses the exact good for them \cite{Elmachtoub2015Opaque1,Elmachtoub2019Opaque2}. 

\textbf{Patient (timing-flexible) customers.} Patient customers have been studied in many applications healthcare (e.g. scheduling non-urgent elective surgeries, see \cite{gerchak1996emergency, huh2013electiveemergent} or organ transplantation (e.g.,\cite{bertsimas2013fairness}) and ride-sharing (e.g. pooled rides, see \cite{Dogan2019rideshare,Jacob2017rideshare}). Time-flexible (patient) customers have also studied in the context of pricing problems (see, e.g.,  \cite{katta2005pricing,chen2018robust, golrezaei2020dynamic,lobel2020dynamic,abhishek2021strategic}). In dynamic pricing literature with time-flexible customers, it is assumed that customer's valuation for an item decays with their waiting time. These customers, however, time their purchasing decision strategically and the goal is to identify an optimal sequence of prices over time. This line of work investigates the impact of having time-flexible customers in pricing decisions, while in our work we investigate the benefit of time-flexible customers in resource allocation problems. (See also \cite{chawla2017stability} for work that studies pricing problems in the presence of customers with deadlines.)

%Another related line of work involves online job scheduling with deadlines (e.g. \cite{ashlagi2019Onlinematching}, \cite{azar2015truthful}), which is related to our work in that less urgent jobs will have longer deadlines.  However, one major difference between our work and that of online job scheduling is that we assume that a commitment must be made immediately, whereas in online job scheduling, a job is allowed to be partially processed or remain idle and then rejected any time before the deadline. 

{\color{black} \textbf{Upfront commitment.} A related body of work with a  notion of upfront commitment is lead time quotation for online job scheduling (see, e.g., \cite{lead_time_1, lead_time_2} and \cite{slotnick2011order} for a survey). In one version of lead-time quotation, a quote for when the job finishes must be provided immediately upon accepting an order while in an easier version of the model,  that quote can be provided any time before the order expires. Not surprisingly, \cite{lead_time_1} shows that the former setting is significantly more challenging than the latter as the best algorithms proposed for the former exhibit larger optimality gaps. Our setting is  closer to the former stringent online model where the acceptance/rejection and the lead time quotation decisions   must be made immediately. Recall that in our setting,  the acceptance/rejection needs to be made immediately and once we accept a partially patient agent, we are committed  to serving them by the next time period. Thus, at a high-level, acceptance and scheduling decisions in the aforementioned works bear some resemblance to our acceptance and serving decisions. However, the differences between our model  do not allow us to use the methodologies  developed in this line of work. In our setting, we can serve agents in parallel contrasting to serving agents sequentially as it is done in job scheduling problems. In addition, unlike job scheduling problems, the notion of processing time for an agent is not relevant in our setting.\footnote{See also \cite{azar2015truthful} for online job scheduling with deadlines.}} 

{\color{black}It is worth noting a recent follow-up study \cite{xie2022benefits} that investigates online resource allocation when decisions are made immediately, with a commitment to fulfilling promises within the next few periods. This research delves into the benefits of delaying real-time decisions under a stochastic framework. Notably, it finds that a slight delay yields the most advantages, and the benefit of delay diminishes as delays grow longer. A primary distinction between this study and ours lies in the modeling of demand: while our work considers adversarial demand, their setting assumes stochastic demand. Under the stochastic model, it is possible, as shown in \cite{xie2022benefits}, to design an algorithm with zero regret, which is not possible in adversarial models. Furthermore, in our work, we handle a mixture of flexible and inflexible agents, whereas in \cite{xie2022benefits}, all requests are flexible. As another difference, while in our work, flexibility allows us to delay serving the flexible agents by one period, in \cite{xie2022benefits}, agents' services can be delayed by $k$ periods. The authors study the impact of $k$ (their level of flexibility) on the obtained regret, showing that a little bit of flexibility goes a long way. In our case, the level of flexibility is determined by the number of flexible agents, and as observed in numerical studies, the performance of our algorithms increases linearly with the level of flexibility. } 

%Timing-flexibility has been studied in matching problems under stochastic setting, rather than adversarial setting that we consider (see. e.g., \cite{ashlagi2017min, aouad2020dynamic, akbarpour2020thickness,hu2021dynamic}). \footnote{\color{black} Please refer to \cite{feng2021batching} for a recent work that explores a similar trade-off under adversarial arrivals. In their study, the authors introduce novel algorithms tailored for multi-stage bipartite allocations involving batch arrivals. It's worth noting that, in contrast to our specific scenario, the algorithms they propose allow for the delay of acceptance decisions until the entire batch arrives, and they do not necessitate any upfront commitments.  } In these papers, customers arrive and depart according to some stochastic arrival and abandonment patterns. To design effective algorithms, one needs to optimize the time of matching while striking a balance between increasing market thickness and mitigating the risk of customers abandoning the system. One main differences between these papers and our work is that our work requires an immediate acceptance/rejection decision upon arrival of an agent, while other works allow agents to be accepted any time before they depart the system. If we want to keep agents around to increase market thickness, we must make an upfront commitment to service them in the near future. Such an upfront commitment is not required in the aforementioned line of work, resulting in a different problem setup. }  

{\color{black}\textbf{Timing-flexibility and matching.} 
Timing-flexibility has been extensively studied in matching problems within stochastic settings, as opposed to our focus on adversarial settings. Notable studies in this domain include  \cite{ashlagi2017min},  \cite{aouad2020dynamic},  \cite{akbarpour2020thickness}, and \cite{hu2021dynamic}, where customers arrive and depart based on stochastic patterns. To design effective algorithms, these studies optimize matching timing while balancing market thickness and customer abandonment risk. One key distinction from our work is that we require immediate acceptance/rejection decisions upon agent arrival, whereas other studies allow decisions at any time before agent departure. This upfront commitment to service is unique to our problem setup.

{\color{black}In a related work by \cite{feng2021batching}, similar trade-offs are explored under adversarial arrivals. They introduce algorithms for multi-stage bipartite allocations with batch arrivals, but unlike our scenario, they allow delays in acceptance decisions until the entire batch arrives, without upfront commitments.}



% {\color{red}This is not very convincing. Could we say more about the main differences in their considered models and their consequences. For example, could we say sth like  ``While in this line of work, the main goal is to optimize scheduling decisions for a single machine, in our work, we study the problem or allocating  multiple resources." Also, looking at these papers, there acceptance decisions can be delayed too and the obtained reward is a function of the lead time (so, they have a more flexible model). But, in any case, we need to state the main difference and highlight that our setting is not a special case of their setting.    }
% } 

%The remainder of our paper is organized as follows. In Section \ref{sec:model}, we present the model and define our notion of competitive ratio. In Section \ref{sec:polyra}, we define the idea of a \po{} algorithm and feasible polytope, which is the basis of all algorithms in this paper. In Sections \ref{section:two_type}, \ref{section:three_type} and \ref{section:beyond_three}, we discuss our contributions for two types, three types, and beyond three types respectively. Finally, in Section \ref{sec:numerical_studies}, we discuss numerical studies that support our theoretical results.


    

==> sections/3_-_problem_setup.tex <==
\section{Problem Setup}
\label{sec:model}
In this work, we study a model where a service-provider (decision-maker) must allocate a scarce service (or resource)  to agents arriving in an online fashion. The agents differ in both their rewards when served as well as their timing flexibility (i.e. patience). We detail the model as follows.

\subsection{Model Definition}
\label{sec:model:model_definitions}
Our model consists of $T$ discrete time periods and $K$ types of agents with rewards $0 < r_1 < \ldots < r_K$ in which the first $M \in [K-1]$ types are \textit{partially patient} (flexible), while the remaining $K - M$ types are \textit{impatient} (inflexible).\footnote{This assumption that the reward for any partially patient agent is less than that of any impatient agent is a reasonable assumption as agents who more urgently need a resource also value it more. We also assume that $M < K$ meaning that there is always at least 1 impatient type as in most applications there is always a type of agent who urgently needs the resource} (We define this precisely later.) Note that for any integer $m$, $[m]= \{1, 2, \ldots, m\}$.  Each time period $t \in [T]$ consists of an \textit{arrival phase} and a \textit{service phase}. When we accept a partially patient agent, we make a \textit{commitment} to provide them service and we must adhere to this commitment.

\textbf{Arrival phase.} For each $t \in [T]$, let $I_t = \{z_{t, 1}, \ldots, z_{t, |I_t|}\}$ be the sequence of agent arrivals in the arrival phase, where $z_{t,n} \in [K]$ is the type of the $n$th arrival in time period $t$. Upon the arrival of the $n$-th agent, we observe its type $z_{t,n}$ and must immediately {\color{black}decide}   whether to accept or reject the agent. Accepted agents must be provided service in an upcoming service phase, while rejected agents leave the system forever.

\textbf{Service Phase. } After all agents in period $t \in [T]$ have arrived, the service-provider can provide service to up to $C$ accepted agents, and collect a reward $r_i$ for each depending on their type $i \in [K]$. When we choose which $C$ agents to serve, we must follow each agents' time-flexibility. All impatient agents (i.e. types $M+1, \ldots, K$) accepted in period $t \in [T]$'s arrival phase must be serviced in period $t$'s service phase, while partially patient agents (i.e. types $1, 2, \ldots, M$) can be serviced either in period $t$'s service phase or carried over to period $t+1$ and serviced during its service phase. 

Our model can be interpreted as an extension of \cite{BallandQueyrenne2009}, incorporating the elements of partially patient agents within a multi-period setting. \cite{BallandQueyrenne2009} delves into a specific case of our model where \( M = 0 \) (indicating all agents are impatient) and \( T = 1 \) (a single time period). Mirroring the approach of \cite{BallandQueyrenne2009}, our goal is to formulate algorithms ensuring reward guarantees in the face of adversarial arrival sequences. However, our model's distinctive features, including the flexibility of certain agents and an upfront commitment, necessitate that all agents receive service timely. {\color{black} We assume that the number of periods $T$ is not known a priori to an algorithm and can be chosen adversarially. In practice, if $T$ is known, then an algorithm may be able to make better choices knowing the ``end is near". However, since we consider adversarial arrivals, knowledge of $T$ does not improve the worst-case instances as an adversary can simply choose an inflated $T$ and stop sending agents after a certain point to simulate a smaller $T$.}

We'd now like to shed light on two  assumptions related to our model:
% {\color{red} moved this here.}
\begin{enumerate}[leftmargin=*]
    \item In order to allow algorithms to take advantage of flexibility in the last period $T$, we add a dummy period $T+1$ where $I_{T+1} = \emptyset$, but we still have $C$ capacity available to serve partially patient agents from period $T$. This period is necessary for otherwise partially patient agents that arrive in the last period would not be any different from impatient agents and so an adversary could choose $T = 1$, reducing us to a problem where all agents are impatient.
    \item This work will focus on the continuous version of the resource allocation problem, where we are allowed to partially accept and serve agents. Although the continuous problem is less realistic than the discrete one, its analysis is much simpler and we can still capture all the core ideas regarding time-flexibility. For the discrete model, all of the algorithms from this paper can still be applied and are asymptotically correct as $C \to \infty$. In addition, to deal with small values of $C$, one can apply a technique used in \cite{BallandQueyrenne2009} to randomly accept or reject agents, obtaining the same performance guarantees in expectation.
\end{enumerate}
Before we discuss our objective in detail, we provide some application examples to make our model more concrete.


\subsection{Application Examples } %{\color{red} I updated this a bit. }
\label{sec:application}
{ \color{black} 
The principle of upfront commitment is especially relevant in scenarios that involve \emph{opaque service timings}. Here, while customers receive an assurance of service delivery, the precise timing remains undisclosed until later. Two real-world examples that exemplify this concept are Instacart and UPS.

% Instacart provides an example of opaque services in the realm of grocery delivery. Typically, they promise delivery within the next hour. Yet, they've broadened their offerings to include a 2-hour delivery window for those customers willing to be more patient.

Instacart is a grocery delivery platform that has recently introduced an opaque service option. Typically, the platform provides delivery within the next hour, but recently has broadened their offerings to include a 2-hour delivery window for more patient customers. Those who opt for the 2-hour delivery are analogous to our partially patient customers, while those demanding immediate delivery fit the impatient category. We can interpret each our $T$ time periods as an hourly slot with $C$ couriers available. If we accept an inflexible customer, we must serve them using one of the $C$ couriers in the current period, while for flexible agents we can also utilize couriers in the next period. Should the situation call for it, Instacart can exercise its right to limit access by deactivating specific delivery windows, thereby rejecting certain customers.

Shipping services like UPS also operate on this opaque principle. The notion of multi-day shipping, whether for end consumers via UPS or businesses through platforms like Amazon, inherently possesses this opaque quality. For instance, a UPS store offering next-day and 2-day shipping services dispatches packages every evening via a truck with a capacity of $C$ packages. While next-day shipping orders must be loaded onto this truck, the 2-day orders have some flexibility: they can either join the same truck if there's room or wait for the next day's truck. Similar to Instacart, UPS can regulate service by marking certain shipping options unavailable when required.


Beyond Instacart and UPS, there are many other arenas where services with opaque timing can leverage agent patience. For instance, an airline or travel agency might offer opaque flights aimed at customers who are indifferent to the precise timing of their departure. Those planning vacations might have the option to secure a booking for the upcoming week or select a more flexible two-week window. Similarly, for ticketed events like concerts, a model can be implemented for fans indifferent between two  consecutive show-times. In service scheduling, such as plumbing or doctor's appointments, there's potential to boost efficiency by catering to customers or patients who are flexible regarding their time slots.

In these scenarios, instead of immediately committing a customer to a specific flight, concert time, or appointment, there's significant value in offering a flexible choice. Here, agents receive a firm assurance of service, with the particulars – be it the exact flight, concert timing, or appointment – disclosed a bit later. Collectively, these examples underscore the significance of adeptly managing opaque services in contemporary business frameworks and the nuanced balancing act essential for their optimization.


%Beyond Instacart and UPS, there are many other settings where services with opaque timing can be used to take advantage of agent patience. For example, an airline or travel agency could offer opaque flights catered towards customers indifferent about the exact timing of their departure. Customers in search of vacation flights could opt for a confirmed booking in the immediate upcoming week or choose a more flexible two-week window option. A similar concept could be set up for ticketed events such as concerts for fans indifferent between two different show-times. In scheduling of services such as plumbing or doctor's appointments, one can increase efficiency by exploiting customers or patients who are indifferent between multiple time slots. In all these above scenarios, rather than locking a customer into a particular flight, concert time or appointment immediately, our work shows that there is much to gain from offering a flexible option in which agents are provided with an upfront commitment of service, but the exact flight, concert time, appointment...etc. is revealed at a slightly later time. Altogether, the examples presented above emphasize the importance of managing opaque services in today's business models and the intricate balance required to optimize them.

%%% 
% BEFORE 
% Beyond Instacart and UPS, there are many other settings where services with opaque timing can be used to take advantage of agent patience. For example, an airline or travel agency could offer opaque flights catered towards customers indifferent about the exact timing of their departure. Customers might be scouting for flights scheduled for either the upcoming week or the one following. For those who are partially flexible, the precise timing of their trip might remain fluid, leaving some wiggle room for the exact departure dates or times. In contrast, inflexible customers would have a set preference, such as requiring a flight strictly within a particular week. This opens up an avenue for travel agencies to offer opaque booking options, where discounts or incentives could be provided to those willing to be flexible about their exact travel dates, thereby optimizing flight capacities and potentially increasing revenues. These scenarios emphasize the importance of managing opaque services in today's business models and the intricate balance required to optimize them.

%The idea of an upfront commitment applies in many real-world settings with products or services that have \textit{opaque} timing. Such products guarantee upfront to provide service to a customer, but do not reveal the exact timing of this service until later. We provide two concrete examples in real-world products: Grocery delivery (Instacart) and Shipping (UPS). 

%Instacart is a grocery delivery platform that provides on-demand grocery delivery typically within the next hour. Instacart recently rolled out a 2-hour delivery option for those customers willing to wait longer for their groceries. Here, our partially patient customers are the ones who choose 2-hour delivery while our impatient customers are the ones who choose immediate delivery. We can model each of our $T$ time periods as an hour of the day. If we accept a flexible customer, we must provide them service either in the current period or in the next period, while if we accept an inflexible customer, we must serve them in the current period. Our capacity $C$ is the number of couriers available in that period. The platform can reject a customer by making the immediate delivery and/or 2 hour delivery options not available. 

%Shipping is another application where opaque products are common as the idea of multi-day shipping (i.e. 2-day shipping) both for consumers (i.e. UPS) and fulfillment (i.e. Amazon, JD.com) is inherently an opaque product as most customers are happy to receive the shipment early. For example, consider a UPS store which offers next-day shipping and 2-day shipping services. Each evening, a single truck arrives at the store and can pick up at most $C$ packages to the distribution center. Packages for customers who choose the next-day shipping option must be included on this truck, whereas packages for customers choosing the 2-day shipping option can be included on this truck (if space permits) or kept overnight at the UPS store and included on tomorrow's truck. Similar to Instacart, a shipping company can reject a customer by simply can marking the next-day or 2-day shipping options as not available. 
}

With the model definition and some motivating applications in mind, we now proceed to describe how we measure the performance of an online resource allocation algorithm under this model. 


{\color{black}\subsection{Objective and Benchmark}
\label{sec:resource_augmented_cr}
We measure the performance of our algorithms using worst-case analysis under a \textit{resource augmentation} framework (see e.g., \cite{resource_augmentation_1, resource_augmentation_2, resource_augmentation_3} or \cite{roughgarden} for a survey). To avoid confusion with the term resource, which we already use to describe our capacity, we will use the term ``feature-augmented" instead. A feature augmentation guarantee bounds the worst-case ratio between the reward of an online algorithm $\mathcal{A}$ that has access to additional feature versus the optimal offline algorithm $\textsc{opt}$ which cannot access the additional feature. %In contrast, the traditional CR bounds the same ratio when both $\mathcal{A}$ and $\textsc{opt}$ have access to the same features. 
The feature-augmented CR allows us to characterize the value of a feature for the algorithm designer. ({\color{black}Refer to Section \ref{sec:compare} for an exploration of the distinctions between the traditional  and feature-augmented CRs.})
 %The issue with using CR is that since we are forced to augment both $\mathcal{A}$ and $\textsc{opt}$'s capabilities, we often do not see an increase in CR from incorporating the feature because our offline benchmark $\textsc{opt}$ can benefit from the additional feature more so than our online algorithm $\mathcal{A}$. 

{\color{black}In our particular setting, the feature in question is the flexibility of types $1$ through $M$. Our feature augmentation bound compares the performance of an online algorithm $\mathcal{A}$ which can utilize the flexibility of these $M$ partially patient types with the offline optimal $\textsc{opt}$ which treats all $K$ types as impatient. For an algorithm $\mathcal A$, arrival sequence  $\{I_t\}_{t\in [T]}$, and $\tau \in [T]$, let $\text{Rew}_{\mathcal {A}, \tau}\left(\{I_t\}_{t\in [T]}\right)$ be the reward of algorithm $\mathcal A$ in time period $\tau$. Here, $\mathcal{A}$ is able to utilize the flexibility of types $1, 2, \ldots, M$ and potentially delay their service by one time period. Let $\textsc{opt}(I_t)$ be the optimal reward that can be obtained from $I_t$ when we treat all types as impatient. We define the \textit{per-period feature-augmented CR} of an algorithm $\mathcal{A}$ as the following:
\begin{align}
  \text{FA-CR}_{\mathcal A} \defeq \inf_{T, \{I_{t}\}_{t\in [T]}, \tau\in [T]}\left\{\frac{\text{Rew}_{\mathcal {A}, \tau}\left(\{I_t\}_{t\in [T]}\right)}{\textsc{opt}(I_\tau)}\right\}\,.
  \label{definition:racr}
\end{align}}

%% This is used for the presentation 

% \begin{minipage}{30em}
% \linespread{1.5}
% \noindent For an algorithm $\mathcal A$, arrival sequence  $\{I_t\}_{t\in [T]}$, and $\tau \in [T]$ we define: 

% \begin{itemize}
%     \item $\text{Rew}_{\mathcal {A}, \tau}\left(\{I_t\}_{t\in [T]}\right)$ is the reward of algorithm $\mathcal A$ in time period $\tau$, where $\mathcal{A}$ can utilize partially patient agents.
%     \item $\textsc{opt}(I_t)$ is the optimal reward that can be obtained from $I_t$ when we treat all types as impatient. \\
% \end{itemize}
% The \textbf{resource-augmented CR} of an algorithm $\mathcal{A}$ is defined as:
% \begin{align*}
%   \text{RA-CR}_{\mathcal A} \defeq \inf_{T, \{I_{t}\}_{t\in [T]}, \tau\in [T]}\left\{\frac{\text{Rew}_{\mathcal {A}, \tau}\left(\{I_t\}_{t\in [T]}\right)}{\textsc{opt}(I_\tau)}\right\}\,.
%   \label{definition:racr}
% \end{align*}
% \\
% \end{minipage}

The per-period feature-augmented CR bounds the ratio of the reward \textit{in each period} $\tau \in [T]$ over all input sequences $\{I_t\}_{t\in [T]}$ of arbitrary length $T$. {\color{black} \color{black} Choosing to consider per-period reward (instead of total reward) is mostly for analytical convenience as the resulting algorithms are much easier to describe and interpret. Additionally, considering this benchmark results in an algorithm that has an equally good performance across all the time periods. We note that if $\mathcal{A}$ achieves a per-period CR  of $\crr$ by equation \eqref{definition:racr}, then it is also the case that:
$ \inf_{T, \{I_{t}\}_{t\in [T]}} \frac{\sum_{\tau \in [T]} \textsc{rew}_{\mathcal{A}, \tau}( \{I_t\}_{t \in [T]}) }{\sum_{\tau \in [T]} \textsc{opt}(I_\tau)} \geq \crr \,, $
implying that the cumulative reward of $\alg$ is also at least $\crr$ times that of the optimal. Finally, ensuring  high per-period rewards can be helpful for small businesses that need steady income to keep going. Nonetheless, in our numerical studies presented in Section \ref{sec:numerical_studies}, we show that our algorithms that are designed based on the per-period feature-augmented CR notion manage to obtain high total reward.} 




Observe that  that when there are no partially patient agents, that is $M = 0$, then our definition in equation \eqref{definition:racr} is exactly the traditional CR definition applied to each time period. When $M = 0$, there is no interaction between periods, so we can assume without loss of generality that $T = 1$, reducing our model to the model from \cite{BallandQueyrenne2009}, in which the optimal CR is \begin{equation}
    \label{equation:bq_cr}
    \crr^{BQ} \defeq \left( K - \sum_{i=1}^{K-1} \frac{r_i}{r_{i+1}} \right)^{-1}\,.
\end{equation} 
%When we use the feature-augmented CR, as we vary $M$ from $0$ to $K-1$, we see that it is possible to obtain algorithms with strictly increasing feature-augmented CR, starting at $L$ when $M = 0$ and increasing up towards $1$. %{\color{red} where do we show such an increase? If there is a figure that later we will present, we can refer to it here.} 

{\color{black}\subsection{Feature-Augmented CR versus the Traditional CR}
\label{sec:compare}

In this section, we demonstrate that when using the traditional CR definition, even in scenarios where almost every type is partially patient (i.e., $M = K-1$), no algorithm can outperform $\crr^{BQ}$ in CR. Intuitively, since the traditional CR benchmark compares an online algorithm with an offline algorithm that can also utilize flexibility, as our algorithms improve with increasing $M$, so does the benchmark. On the other hand, with the feature-augmented CR, we precisely quantify how leveraging the flexibility of these partially patient agents leads to enhanced online performance.

To be more precise, let
\begin{equation} 
\label{equation:conventional_benchmark}
\text{TR-CR}_{\mathcal{A}} = \inf_{\{I_t\}_{t \in [T]}} \left\{ 
\frac{\sum_{\tau = 1}^T \textsc{rew}_{\mathcal{A}, \tau}(\{I_t\}_{t \in [T]})  }{ \textsc{opt-total} (\{ I_t \}_{t\in[T]}) }
\right\}\,
\end{equation}
represent the traditional CR of an algorithm $\mathcal{A}$. Here, the numerator calculates the total reward over $T$ periods of algorithm $\mathcal{A}$, while the denominator is the total reward of the optimal clairvoyant solution that knows $\{I_t\}_{t \in [T]}$ in advance and can utilize the flexibility of types $1$ through $M$.

Theorem \ref{flex_is_bad} establishes that in situations where nearly every agent type is patient ($M = K - 1$), no non-anticipating algorithm can achieve a CR greater than $\crr^{BQ}$.

\begin{theorem}
\label{flex_is_bad}
For any $K \geq 2$ and $M = K - 1$, no non-anticipating algorithm $\mathcal{A}$ can achieve a traditional CR (as given by  equation \eqref{equation:conventional_benchmark}) greater than $\crr^{BQ}$, i.e., $\text{TR-CR}_{\mathcal{A}} \leq \crr^{BQ}$, where $\crr^{BQ} = \frac{1}{K - \sum_{i=1}^{K-1} \frac{r_{i}}{r_{i+1}}}$.
\end{theorem}


This theorem implies that under the traditional CR, we cannot observe the value of flexibility in scenarios where nearly every agent type is patient. By endowing the offline benchmark with the ability to leverage patient agents, it becomes such a strong benchmark that it negates any additional competitive advantage an algorithm might seek from agent flexibility. 


Moreover, we would like to highlight that while our inflexible offline benchmark, used in the definition of the feature-augmented CR, has a closed-form solution making its analysis more straightforward, the flexible offline benchmark does not admit a closed-form solution. Characterizing the flexible offline benchmark $\textsc{opt-total} (\{ I_t \}_{t\in[T]})$ requires the formulation of dynamic programming or a mathematical  program to elucidate the behavior of this optimal flexible clairvoyant solution.


Although the majority of our paper focuses on theoretical results for the feature-augmented CR, we provide an extensive numerical study in Section \ref{sec:numerical_studies} where we demonstrate that the algorithms we design to optimize for the feature-augmented CR also performs well under the traditional CR definition. In the rest of this paper, for the sake of conciseness, we will simply use the term CR to refer to the feature-augmented CR from equation \eqref{definition:racr}, even though it is a slight misnomer. In Section \ref{sec:numerical_studies} when we discuss both CR definitions, we will be very clear which one we're referring to.}


% Nonetheless, determining the C of our proposed \po{} algorithm in comparison to the classical offline clairvoyant solution, as well as devising algorithms that achieve the best classical C, opens up novel avenues for research and presents exciting challenges in the field.

% It's worth noting that our notion of C may not directly account for total accumulated reward, but in practical scenarios, our designed algorithm consistently achieves both high total rewards and high per-period rewards, as demonstrated by our numerical studies in Section \ref{sec:numerical_studies}. Furthermore, as the numerical results indicate, our algorithm consistently attains a high traditional C, demonstrating the power of our feature-augmented C.


==> sections/4_-_polyra.tex <==

\section{Polytope-based Resource Allocation (POLYRA) Algorithms}
\label{sec:polyra}
We present an intuitive class of algorithms called polytope-based resource allocation (\po) algorithms. Such algorithms keep track of a state $\stateB \in \mathbb{R}_+^{K+M}$ which tracks the number of agents of each type that our algorithm has accepted so far, as well as their deadlines. Each \po{} algorithm instance is parameterized by a feasible polytope $\feasible \subset \mathbb{R}_+^{K+M}$ which intuitively describe the set of all states that our algorithm is allowed to be in. As we will explain in more detail below, a \po{} algorithm makes greedy decisions while maintaining the invariant that $\stateB \in \feasible$.

\begin{figure}
  \centering
  \begin{equation*}
    \begin{array}{r|ccccccc}
      \text{Type} \qquad  & 1 \quad               & 2 \quad               & \ldots \quad & M \quad               & M+1 \quad          & \ldots \quad & K          \\ \hline
      \text{Row 1} \qquad & \bucketij{1}{1} \quad & \bucketij{2}{1} \quad & \ldots \quad & \bucketij{M}{1} \quad & \bucket{M+1} \quad & \ldots \quad & \bucket{K} \\
      \text{Row 2} \qquad & \bucketij{1}{2} \quad & \bucketij{2}{2} \quad & \ldots \quad & \bucketij{M}{2} \quad &                    &              &
    \end{array}
  \end{equation*}
  \caption{The $K + M$ buckets in our state $\stateB$. Buckets in the first row contain agents that have been allocated a resource from the current time period, while buckets in the second row contain only partially patient agents  who have accepted that we tentatively {plan on carrying over} to period $t+1$ and servicing in that period's service phase.}
  \label{fig:buckets}
\end{figure}

\textbf{State.} At any point in time, our algorithm keeps track of a state $\stateB$ which consists of the following $K+M$ dimensional vector of non-negative numbers:
\begin{equation} 
\label{bucketdefinition}
\stateB=(\bucketOneOne, \bucketTwoOne, \ldots, \bucketMOne, \bucketMPlusOne, \ldots, \bucketK; \bucketOneTwo, \bucketTwoTwo, \ldots, \bucketMTwo)\,.
\end{equation}
We will refer to each index of the state as a \textit{bucket}. All accepted agents are assigned to a bucket and the bucket keeps track of the number of such agents assigned to it. These buckets are illustrated more visually in Figure \ref{fig:buckets}. We use $\bucketij{k}{j}$, $k\in [M]$ and $j\in [2]$, or $\bucket{k}$, $k\in \{M+1, \ldots, K\}$ to refer to both the bucket itself or as well as the number of agents assigned to it.
\begin{itemize}[leftmargin=*]
  \item \textbf{First row.}
        In any given time period $t$, the first row of buckets from Figure \ref{fig:buckets} keeps track of the number of agents of each type that have been accepted and \textit{we plan on serving} in period $t$'s service phase. More precisely, for $i \in [M]$, bucket $B_{i,1}$ and for $i \in \{M+1,\ldots, K\}$ bucket $\bucket{i}$ store agents of type $i$ that we definitely going to serve using the $C$ capacity available at the end of the current period $t$.

  \item \textbf{Second row. } 
        Each bucket in the second row $\bucketij{k}{2}$,
        $k\in [M]$ captures the number of type $k$ agents we have accepted that we tentatively \textit{plan on carrying over} to period $t+1$ and servicing in that period's service phase. 
\end{itemize}

\noindent In other words, at any moment in time, the state $\stateB$ describes how we are planning on servicing the agents we have accepted and are still waiting for service. We now describe how we update the states during the arrival phase and service phase.

{\color{black}\textbf{Arrival phase: acceptance rule.} Upon the arrival of an agent of type $i$, we will accept them if there is a way to update the state while maintaining feasibility. More precisely, we split into two cases based on whether type $i$ is impatient or partially patient.

\begin{itemize}[leftmargin= *]
  \item \textbf{Impatient  types. }If $i \in \{M+1, \ldots, K\}$, accepting such an agent would imply that we must service them using period $t$'s capacity, which means that $\bucket{i}$ would need to be incremented in $\stateB$. If this new state is feasible, then we accept this type $i$ agent, otherwise we reject them. \footnote{More precisely, under our continuous model, we find the largest value of $\epsilon \leq 1$ such that: $\stateB + \epsilon \cdot e_{i} \in \feasible$, where $e_i$ is a   vector with $K+M$ length  and all $0$'s except a $1$ at the $i$-th index.} 

  \item \textbf{Partially patient types. }If type $i \in [M]$, then we consider two possibilities, which corresponding to when we plan on servicing this agent. We first check to see if bucket $\bucketij{i}{2}$ can be incremented while maintaining feasibility. If so, we accept this agent and assign them to bucket $\bucketij{i}{2}$. Otherwise, we try the same with $\bucketij{i}{1}$ and if not, we reject the agent. \footnote{More precisely, we first find the largest $\epsilon_2 \leq 1$ for which $\stateB' = \stateB + \epsilon_2 \cdot e_{K+i}$ is feasible, where $e_{K+i}$ is a vector of all $0$'s and a 1 corresponding to bucket $\bucketij{i}{2}$ (recall equation \ref{bucketdefinition}). If $\epsilon_2 = 1$, then we are done. Otherwise, we find the largest $\epsilon_1 \leq 1 - \epsilon_2$ such that the state $\stateB' = \stateB + \epsilon_2 \cdot e_{K+i} + \epsilon_1 \cdot e_{i}$ is feasible, which corresponds to assigning a fractional $\epsilon_1$ of an agent to bucket $\bucketij{i}{1}$.}
\end{itemize}

\textbf{Service phase: updating bucket state $\stateB$}. During the service phase, we will choose to serve all the agents assigned to the first row of Figure \ref{fig:buckets}, as per the definition of the first row of buckets. Using the remaining  $\ell \defeq C - \left( \bucketij{1}{1} + \ldots + \bucketij{M}{1} + \bucket{M+1} +\ldots+ \bucket{K} \right)$, we will greedily serve the agents assigned to buckets $B_{1,2}, \ldots, B_{M, 2}$ (i.e. the second row) by prioritizing agents with higher rewards. This greedy action  can be described  using  the optimal solution to the following LP: 
\begin{align}
    (s_i^*)_{i=1}^M = \text{argmax}_{(s_i)_{i=1}^M} \quad & \sum_{i=1}^M r_i \cdot s_i \label{serving_lp}
   \qquad  \text{s.t.} \quad  \sum_{k=1}^M s_i \leq \ell \quad \text{ and } \quad s_i \in [0, \bucketij{i}{2}], \quad  i\in [M] \,. 
\end{align}
Here, $s_i^*$ is the number of agents of type $i$ that upon acceptance,  were assigned to bucket $B_{i,2}$ in time period $t$, and are served in the same time period.  

Our total reward from servicing would be $\sum_{i=1}^M r_i \cdot (s_i^* + \bucketij{i}{1}) + \sum_{i=M+1}^K r_i \cdot \bucket{i}$. We would update our state as follows:
\begin{equation}
  \widehat{\stateB} = (\bucketij{1}{2} - s_1^*, \ldots, \bucketij{M}{2} - s_M^*, \underbrace{0, \ldots, 0}_{K-M};  \underbrace{0, \ldots, 0}_{M})\,. \label{serving_rule_update_state}
\end{equation}
Here, the first $M$ coordinates represent the remaining partially patient agents that we did not service in period $t$, so we must service in period $t+1$. All other coordinates are empty because they contain agents that were served (the state $\stateB$ only keeps track of agents accepted but not yet served). }

In order for the algorithm above to be well defined, we present the following definition for any feasible polytope $\feasible$ we consider.

\begin{definition} [Valid Polytopes] \label{def:valid}
  A polytope $\feasible$ is \textit{valid} if:
  \begin{enumerate}
    \item [(i)] \label{def:valid:never_overaccept} For all $\stateB \in \feasible$, we must have the sum of the first row of $\stateB$ be at most $C$, i.e. $\sum_{i=1}^M \bucketij{i}{1} + \sum_{i=M+1}^K \bucket{i} \leq C$. Since the first row contains agents who must be served in the current time period, we certainly cannot promise this to more than $C$ agents. 
    \item [(ii)] \label{def:valid:never_overaccept_row_two} For any time period $t\in [T]$, and (feasible) buckets state $\stateB$, the updated buckets state after applying our serving rule (i.e., $\widehat \stateB$ presented in equation \eqref{serving_rule_update_state} and finding the optimal solution $s_i^*$ to equation \eqref{serving_lp}) remains feasible (i.e., $\widehat \stateB \in \feasible$). Recall that \po{} algorithms maintain the invariant that $\stateB \in \feasible$ is always true, so certainly our updating rule in equation \eqref{serving_rule_update_state} must maintain this invariant.
  \end{enumerate}
\end{definition}

Any polytope we present in this work will be valid as per Definition \ref{def:valid}. 

% \item [(ii)] For any state $\stateB$ and $\stateB'$ such that $\stateB \preceq \stateB'$ (coordinate-wise), if $\stateB' \in \feasible$, then $\stateB \in \feasible$. In other words, lowering the values in a feasible $\stateB'$ continues to make the state feasible. 
 
% We highlight that the updated buckets state $\widehat \stateB$ should be also feasible, i.e., $\widehat \stateB \in \feasible$. Such a crucial property may not be satisfied for any feasible polytope $\feasible$, but it is satisfied by all of the feasibility polytopes we consider in this paper. 

%Another property of the polytopes we consider in this paper is that if we have two states $\stateB$ and $ \stateB'$ such that $\stateB \preceq \stateB'$ (coordinate-wise), then $\stateB' \in \feasible$ implies $\stateB \in \feasible$. That is, we would like $\feasible$ to be a \emph{downward closed polytope}. This property says that our polytopes are designed so that decreasing any coordinate of a feasible state maintains feasibility. One consequence of this property is that if $\stateB$ cannot accommodate a positive amount of an incoming type $j$ agent, then we can be certain that $\stateB'$ also cannot. In other words, if a particular type $j$ cannot be accommodated in $\stateB$ early on in the arrival sequence $I_t$, then certainly it will also not be accommodated later in $I_t$ when more agents of other types may have been accepted. The two properties discussed above are summarized in the definition below.


\section{Nested POLYRA Algorithm} 
To show the versatility of our \po{} algorithms, we now present a special class of \po{} algorithms that we refer to  as \emph{nested \po{}} algorithms. These \po{} algorithms use a special class of  
 polytopes called \textit{nested polytopes} that we will define shortly.  As it will become more clear later, the nested \po{} algorithms can be viewed as a  generalization of the well-known nested booking limits policy from \cite{BallandQueyrenne2009}.

 

\begin{definition}[Nested Polytopes] \label{def:nested}
  When there are $K$ types with the first $M$ partially patient, for any $(n_1, \ldots, n_K)$ with $0 \leq n_1 \leq \ldots \leq n_K = C$, we define the nested polytope with nest sizes $(n_1, \ldots, n_K)$ to be $\feasiblenest(\nestOne, \nestTwo, \ldots,  \nestK)$ given by the vector of $$(\fbucketOneOne, \fbucketTwoOne, \ldots, \fbucketMOne, \fbucketMPlusOne, \ldots, \fbucketK; \fbucketOneTwo, \fbucketTwoTwo, \ldots, \fbucketMTwo)\subset \mathbb{R}_+^{K+M}$$ that satisfies the following two sets of constraints:
  \begin{align}
    \sum_{i=1}^k b_{i, j}                        & \leq n_k & k \in [M], j \in [2] \notag \\
    \sum_{i=1}^M b_{i, 1} + \sum_{i=M+1}^k b_{i} & \leq n_k & k \in \{M+1, \ldots, K\}
    \label{eq:nested:polytope}\tag{$\feasiblenest(\nestOne, \nestTwo, \ldots,  \nestK)$}\,.
  \end{align}
\end{definition}

% \begin{equation}
% \mathcal{B}_{\text{nest}}(3, 5, 8) = (b_{1,1}, b_{2,1}, b_{3,1}, b_{2,1}) \in \mathbb{R}^{4}_{+} \text{ s. t. } 
% \begin{array}{cccccc}
% b_{1,1} && && &\leq 3  \\
% b_{1,2} && &&  &\leq 3 \\
% b_{1,1} &+& b_{2,1} && &\leq 5 \\
% b_{1,1} &+& b_{2,1} &+& b_{3,1} &\leq 8 
% \end{array}
% \end{equation}

A nested polytope $\feasiblenest(\nestOne, \nestTwo, \ldots,  \nestK)$ imposes \emph{booking limits} on the $C$ resources we have in each time period, restricting type $i$ agents to only $n_i$ out of the $C$ resources. The limits $n_i$ are nested in a way that higher reward agents have access to more resources (note that $r_1 < \ldots < r_K$ and $n_1 \leq \ldots \leq n_K)$. The two sets of constraints above enforce these limits: the first set of constraints enforces the booking limit for partially patient agents in \textit{both rows} of our state $\stateB$ (since the same booking limits apply to both agents we plan on serving in period $t$ as well as $t+1$). The second set of constraints enforces booking limits across the entire first row for each impatient type. It is also easy to see that nested polytopes are \consistent{} as per Definition \ref{def:valid}. Property (i) is explicitly enforced as $n_K = C$ in Definition \ref{def:nested} and property (ii) is satisfied because the first set of constraints above are duplicated for $j =2$.

%{\color{red} moved this here and shortened it.} 
Observe that  when $M = 0$, our nested polytope only consider the current period's resources (since no agents are flexible) and we recover exactly their nested booking limit policy from \cite{BallandQueyrenne2009}. %Nested \po{} algorithms have many advantages. Not only are they easy to interpret and parameterized by only $K$ variables ($n_1, \ldots, n_K$), as we will show in the next section, computing the CR for any \po{} algorithm with nested polytope can be solved by an LP (Theorem \ref{theorem:polyra_nested_performance}). %As we will show later, the resulting LP is also linear in $(n_1, \ldots, n_K)$, which means we can also use it solve for the optimal choice of nest sizes $(n_1^*, \ldots, n_K^*)$ (Definition \ref{def:optimal_nested_algorithm}), resulting in the optimal nested algorithm with a CR of $\crr^{*}$; see Section \ref{section:beyond_three}, where we show that our optimized nested algorithm performs well for any arbitrary number of types.
We now provide a concrete example of a nested polytope and its interpretation as booking limits. 

\begin{figure}
    \centering
    \begin{subfigure}[c]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{polytope_example.png}
    \end{subfigure}
    \begin{subfigure}[c]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{polytope_example_2.png}
    \end{subfigure}
    \vspace{0.5em}
    \caption{Example of the nested polytope $\nestedPolyra(3, 5, 8)$ with $K = 3, M = 1, C = 8$. }
    \label{fig:nested_polytope_example}
\end{figure}

{
\color{black}
\begin{example}
    \label{example:nested_example}

    Let's consider an example with $K = 3$ agent types having rewards $r_1 < r_2 < r_3$. Here, type $1$ is flexible, meaning $M = 1$. Given a capacity $C = 8$, we can explore the nested polytope $\nestedPolyra(3, 5, 8)$. The feasible region of this polytope is illustrated on the left of Figure \ref{fig:nested_polytope_example}. The accompanying diagram on the right provides a visual representation of this polytope. In this diagram, the top row indicates the $C = 8$ units of capacity available in the current period, while the bottom row displays the $C = 8$ resources set for the next period.

The core notion of a \textit{booking limit} revolves around directing how these $C = 8$ resources are designated among type $1, 2$, and $3$ agents, ensuring specific capacities are reserved for higher reward agents. In the current period (represented by the top row in Figure \ref{fig:nested_polytope_example}), the first 3 units can cater to any agent type. The subsequent 2 units (highlighted in light green) are reserved for types 2 and 3 agents, while the remaining 3 units (in blue) are exclusively for type 3 agents. The constraints $b_{1,1} \leq 3$, $b_{1,1} + b_{2,1} \leq 5$, and $b_{1,1} + b_{2,1} + b_{3,1} \leq 8$ uphold these booking limits. As an illustration, the constraint $b_{1,1} + b_{2,1} \leq 5$ means our state $(b_{1,1}, b_{2,1}, b_{3,1}, b_{1,2})$ is feasible in $\nestedPolyra(3, 5, 8)$ only if a minimum of $8-3=5$ units of the current period's capacity is retained for type $3$ agents. For the next period's resource, we see a comparable booking limit, planning to serve up to 3 type 1 agents. Hence, the constraint $b_{1,2} \leq 3$ is in place. 

It's important to note that these booking limits primarily apply during the arrival phase when making decisions about agent acceptance. In the service phase, after attending to agents allocated to the top row, any remaining resources are used for agents in the bottom row, irrespective of previous booking limits.





   % Let there be $K = 3$ types of agents with rewards $r_1 < r_2 < r_3$ of which type $1$ is flexible (i.e. $M = 1$). Let the capacity be $C = 8$ and consider the nested polytope $\nestedPolyra(3, 5, 8)$. The feasible region of this polytope is shown on the left of Figure \ref{fig:nested_polytope_example}. We can visually represent this polytope using the diagram on the right. Here, the top row represents the $C = 8$ units of capacity we have today (period $t$) and the bottom row represents the $C = 8$ resources we have tomorrow (period $t+1$). The idea behind a \textit{booking limit} is that we restrict how these $C = 8$ resources can be allocated across type $1, 2$ and $3$ agents by reserving certain capacity for higher reward agents. For today's resources (i.e. the top row) the first 3 units can be allocated to any agent type, the next 2 (light green) can only be allocated to type 2 and 3 agents, while the last 3 units (blue) can only be allocated to type 3 agents. The constraints $b_{1,1} \leq 3$, $b_{1,1} + b_{2,1} \leq 5$ and $b_{1,1} + b_{2,1} + b_{3,1} \leq 8$ enforce these booking limits. For example, $b_{1,1} + b_{2,1} \leq 5$ implies that our state $(b_{1,1}, b_{2,1}, b_{3,1}, b_{1,2})$ can only be a feasible state in $\nestedPolyra(3, 5, 8)$ if at least $8-3$ units of today's capacity is reserved for type $3$ agents. For tomorrow's resource, we have a similar booking limit. We can plan on serving up to 3 type 1 agents with tomorrow's capacity, hence the constraint $b_{1,2} \leq 3$. Note that this booking limits interpretation only applies during the arrival phase when deciding which agents to accept/reject. During the service phase, after serving the agents assigned to the top row, we will allocate the remaining resources to the bottom row agents regardless of booking limits. 
\end{example}
}




% {\color{red} Evan: I think we should just add an explicit example here for say $K = 3, M = 1$ and how the nested polytope and constraints work. 

% Example with diagram. Take $C = 8$ with $n_1 = 3, n_2 = 5, n_3 = 8$. On the left, show the 8 capacity and divide it into 3 segments. On the right, show the set of constraints on the buckets. 

% }

% { \color{black}When $M = 0$, our nested polytope simplifies to the nested booking policies from \cite{BallandQueyrenne2009}. These policies establish reserved segments for different types of requests. The initial segment is dedicated to the highest-reward type (i.e., type $K$) and has a capacity of $n_K - n_{K-1}$. The second segment, with a capacity of $n_{K-1} - n_{K-2}$, is designated for orders involving the top two reward types (i.e., type $K$ and $K-1$). Subsequent segments cater to orders with the top three types and so on.

% To illustrate, when a request of type $K-1$ (the second-highest type) arrives, the policy initially attempts to allocate it to the second segment. If this segment is at capacity, it moves to the third segment and so on. If there is no availability in any of these segments, the order is declined. This can be expressed using our bucket definition and the constraints of the nested polytope. In this context, an arriving order of type $K-1$ is rejected when accepting it would violate the following constraints: $\sum_{i=1}^{K-1} B_i \leq n_{K-1}$ and $\sum_{i=1}^{K} B_i \leq n_K$. The first constraint indicates insufficient resource reservation for type $K-1$, and the second constraint signifies resource exhaustion. These policies are characterized by their use of conventional nesting techniques. In this work, we extend these natural policies to scenarios involving a mix of flexible and inflexible agents with varying rewards. }{\color{red}maybe add more here to explain what is happening when $M\neq 0$}

% Nested \po{} algorithms have many advantages. Not only are they easy to interpret and parameterized by only $K$ variables ($n_1, \ldots, n_K$), as we will show in the next section,  computing the CR for any \po{} algorithm with nested polytope can be solved by an LP (Theorem \ref{theorem:polyra_nested_performance}). As we will show later, the resulting LP is also linear in $(n_1, \ldots, n_K)$, which means we can also use it solve for the optimal choice of nest sizes $(n_1^*, \ldots, n_K^*)$ (Definition \ref{def:optimal_nested_algorithm}), resulting in the optimal nested algorithm with a CR of $\crr^{*}$; see Section \ref{section:beyond_three}, where we show that our optimized nested algorithm performs well for any arbitrary number of types.

\subsection{An LP Characterization of the CR of any Nested \textsc{POLYRA} Algorithms} \label{sec:CR_nested}
%From Theorem \ref{thm:opt_2} ($K = 2$) and Theorem \ref{theorem:three_type_M=2} ($K = 3, M = 2$), we have seen two examples of nested \po{} algorithm in action. In each theorem, we gave a particular instance of the nested \po{} algorithm and showed that it achieves the  optimal CR. Now, with $K > 3$ types, 
Here, we present a general way of computing the CR of any given instance of the nested \po{} algorithm.  
%{\color{red} I am assuming the result holds for any $K$, not only $K>3$.}
That is, for any given values of $n_1, \ldots, n_K$ such that $0 \le n_1 \le n_2\le \ldots \le n_K$, we show how to compute the CR achieved by a \po{} algorithm with feasible polytope $\nestedPolyra(n_1, \ldots, n_K)$.

\begin{theorem}[CR of Nested \textsc{POLYRA} Algorithms]
  \label{theorem:polyra_nested_performance}
  For any given values of $n_1, \ldots, n_K$ such that $0 \le n_1 \le n_2\le \ldots \le n_K = C$,  the CR of the nested \po{} algorithm with  polytope $\nestedPolyra(n_1, \ldots, n_K)$ is given by $\crr_{\text{nest}}(\{\nest{i}\}_{i\in [K]})$,  which is  defined by the following LP
  \begin{align}
    \crr_{\text{nest}}(\{\nest{i}\}_{i\in [K]}) \defeq \max_{\crr, \{s_i^j\}_{j \in [K], i \in [j]}} \quad & \crr \nonumber \\
    \text{s.t} \quad                              & \crr \cdot C \cdot r_j \leq \sum_{i=1}^j \nestedvar{i}{j} \cdot r_i \label{nested_lp_revenue_target} & j \in [K]                                     \\
    \lplabel[lp:nested_polytope]{\textsc{(nest)}} & \sum_{i=1}^j \nestedvar{i}{j} \leq C                                                                 & j \in [K] \label{nested_lp_capacity}          \\
      & \deltan_i \leq \nestedvar{i}{j} \leq 2 \cdot \deltan_i                                           & j \leq M, i \in [j] \label{nested_lp_j_le_M}  \\ \label{nested_lp_j_ge_M}
      & \nestedvar{i}{j} = \deltan_i                                                                      & j > M, i \in [j] \\
      & \Gamma\ge 0, s_i^j\ge 0 & j\in [K], i\in [j]\,, \label{eq:positive}
  \end{align}
  Here, $\deltan_i = \nest{i}-\nest{i-1}$ and $\nest{0}$ is defined to be zero. When $\{n_i\}_{i \in [K]}$ is understood from the context, we omit it and just write $\crr_{\text{nest}}$.
\end{theorem}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{nested_worst_cases.png}
    \caption{Worst case states $\stateB^1, \stateB^2, \stateB^3, \stateB^4$ for the nested polytope $\feasiblenest(3, 5, 7, 8)$ with $K = 4$ and $M = 2$. The shading represents the capacity that is reserved for each type. The numbers in each block correspond to the agent type designated to that block. Black numbers represent agents who were accepted and subsequently served by the end of the current period, while gray numbers signify those that were accepted but could not be served in the current period.  }
    \label{fig:nested_polytope_worst_cases}
\end{figure}

\textbf{Intuition for Theorem \ref{theorem:polyra_nested_performance} and its proof sketch}. %{\color{red} shortened this a bit.}
We can characterize any \po{} algorithm's CR with the nested polytope $\nestedPolyra(n_1, \ldots, n_K)$ by considering $K$ worst-case scenarios. If our \po{} algorithm performs well in each of these $K$ worst-case scenarios (achieving a CR of $\crr$), each associated with a state $\stateB^j$, $j\in [K]$, then it will perform well for any arbitrary arrival sequence (achieving a CR of $\crr$).

These states $\stateB^j$ are defined as follows:
\begin{itemize}
\item If $j \in [M]$, then $\stateB^j_{i,1} = \stateB^j_{i,2} = \deltan_i$ for $i \in [j]$, and all other buckets are empty.
\item If $j \in \{M+1, \ldots, K\}$, then $\stateB^j_{i,1} = \deltan_i$ for all $i \in [M]$, $\stateB^j_{i} = \deltan_i$ for all $i \in {M+1, \ldots, j}$, and all other buckets are empty.
\end{itemize}
Each scenario $\stateB^j$ represents a state where no more type $j$ agents can be accommodated, and among such states, $\stateB^j$ minimizes the total reward of agents by maximizing the number of type $1, 2, \ldots, j-1$ agents. Let $s^j_i$ be the total number of type $i$ agents serviced from $\stateB^j$ (assuming this is the state at the end of the arrival phase). The reward obtained during this period is $\sum_{i=1}^j r_i \cdot s^j_i$. To ensure that our choice of nest sizes $n_1, \ldots, n_K$ yields a $\crr$-competitive algorithm, we establish the condition $\sum_{i=1}^j r_i \cdot s^j_i \geq \crr \cdot C\cdot r_j$ (constraint \eqref{nested_lp_revenue_target}). Additionally, we must have $\sum_{i=1}^j s_{i}^j \leq C$ to allocate no more than $C$ resources in scenario $j$ (constraint \eqref{nested_lp_capacity}). Constraints \eqref{nested_lp_j_le_M} and \eqref{nested_lp_j_ge_M} limit the range of $s_{i}^j$, ensuring we serve agents in the first row and no more agents than the total between the first and second rows for scenarios $j \leq M$.

{
\color{black}
\begin{example}
We illustrate the proof of Theorem \ref{theorem:polyra_nested_performance} with a concrete example shown in Figure \ref{fig:nested_polytope_worst_cases}. Similar to Example \ref{example:nested_example}, the shading represents the resources that are ``reserved" for higher reward agents (e.g., the light green region can only contain types $2, 3$, and $4$). The numbers indicate the type of agent we plan on serving with that specific resource. This example matches the definition of $\stateB^j$ for $j \in [4]$ defined above. For each $\stateB^j$, we discuss the agents serviced if $\stateB^j$ is the final state at the end of the arrival phase.

\begin{itemize}
    \item $\stateB^1$: We will service all 6 type 1 agents. No other agents have been accepted. Thus: $s_{1}^1 = 6, s_{2}^{1} = s_3^1 = s_4^1 = 0$. The total reward is $6 \cdot r_1$. 
    \item $\stateB^2$: We service all agents on the top row and use the remaining $8-5=3$ capacity to greedily service the agents in the second row. This results in $s_1^2 = 4, s_2^2 = 4, s_3^2 = s_4^2 = 0$. The total reward is $4 \cdot r_1 + 4 \cdot r_2$. 
    \item $\stateB^3$: We service all agents, thus $s_1^3 = 3, s_2^3 = 2, s_3^3 = 2$ for a total reward of $3 \cdot r_1 + 2 \cdot r_2 + 2 \cdot r_3$. 
    \item $\stateB^4$: Similarly, we service all agents and thus $s_1^4 = 3, s_2^4 = 2, s_3^4 = 2, s_4^4 = 1$ for a total reward of $3 \cdot r_1 + 2 \cdot r_2 + 2 \cdot r_3 + r_4$. 
\end{itemize}

Plugging the above values of $s_{i}^j$ into the LP in Theorem \ref{theorem:polyra_nested_performance}, we get that the optimal $\crr$ and thus the CR of $\nestedPolyra(3, 5, 7, 8)$ is: 
$$ \crr_{\text{nest}}(3, 5, 7, 8) = \min \left( \frac{6 \cdot r_1}{8 \cdot r_1}, \frac{4 \cdot r_1 + 4 \cdot r_2}{8 \cdot r_2}, \frac{3 \cdot r_1 + 2 \cdot r_2 + 2 \cdot r_3}{8 \cdot r_3}, \frac{3 \cdot r_1 + 2 \cdot r_2 + 2 \cdot r_3 + 1 \cdot r_4}{8 \cdot r_4}  \right)\,.  $$
For any rewards $r_1 < r_2 < r_3 < r_4$, Theorem \ref{theorem:polyra_nested_performance} claims that the above minimum of 4 expressions is the CR of this nested \po{} algorithm. 
\end{example}
}
% These worst-case scenarios are illustrated in Figure \ref{fig:nested_polytope_worst_cases}.

% \iffalse
% The state $\stateB^j$ associated with scenario $j \in [K]$ is defined as follows:
% \begin{itemize}
%   \item If $j \in [M]$, then the state $\stateB^j_{i,1} = \stateB^j_{i,2} = \deltan_i$ for $i \in [j]$ and all other buckets are empty.

%   \item If $j \in \{M+1, \ldots, K\}$, then we have $\stateB^j_{i,1} = \deltan_i$ for all $i \in [M]$, $\stateB^j_{i} = \deltan_i$ for all $i \in \{M+1, \ldots, j\}$ and all other buckets are empty.
% \end{itemize}

% For each $j \in [K]$, scenario $\stateB^j$ is a state which cannot accommodate any more type $j$ agents, and out of all states for which this is true, $\stateB^j$ contains a set of agents that  minimizes the total reward of the agents in $\stateB^j$ by maxing out on the number of type $1, 2, \ldots, j-1$ agents in that order. Given that the arrival phase ends in state $\stateB^j$, let $s^j_i$ be the \textit{total} number of type $i$ agents that we would service from $\stateB^j$. Then, the reward that is obtained in this time period can be written as $\sum_{i=1}^j r_i \cdot s^j_i$. In order for our choice of nest sizes $n_1, \ldots, n_K$ to produce a $\crr$-competitive algorithm, we claim in the theorem that $\sum_{i=1}^j r_i \cdot s^j_i \geq \crr \cdot C\cdot r_j$ must be true, leading to constraint \eqref{nested_lp_revenue_target}. In addition, we must have that $\sum_{i=1}^j s_{i}^j \leq C$ as we can allocate no more than $C$ resources in total in scenario $j$, which gives rise to constraint \eqref{nested_lp_capacity}. Finally, the remaining two constraints \eqref{nested_lp_j_le_M} and \eqref{nested_lp_j_ge_M} are just bounds on the range of $s_{i}^j$ to enforce that we always serve agents in the first row and no more agents than in total between the first and second rows (for scenarios $j \leq M$).
% We demonstrate these worst-case scenarios using an example in Figure \ref{fig:nested_polytope_worst_cases}.
% \fi 

{\color{black}
\subsection{Benchmark Algorithm: BQ Nested POLYRA Algorithm}
Having defined nested \po{} algorithms, we now present a natural benchmark algorithm for our model that we refer to as \emph{BQ Nested \po{} Algorithm}. This benchmark is inspired by the algorithm designed in  \cite{BallandQueyrenne2009} for the setting without partially patient agents. 
Recall that when $M = 0$, \cite{BallandQueyrenne2009} showed that the optimal algorithm uses a nested polytope and gives an explicit formula for these nest sizes. In general, for the case when $M > 0$, one can design a nested polytope using these \textit{same} nest sizes that are optimized for the $M = 0$ case. We define this naive nested polytope formally below.

\begin{definition}[BQ Nested Polytope] 
\label{def:bq_nest}
For any number of agents $K$ with reward $r_1 < \ldots < r_K$ where the first $M \in [K-1]$ are partially patient, we define the BQ nested polytope as follows: 
$$
\feasiblenest^{BQ} \defeq \feasiblenest(n^{BQ}_1, \ldots, n^{BQ}_K)\,,
$$ 
where $(n^{BQ}_1, \ldots, n^{BQ}_K)$ are the  nest sizes from \cite{BallandQueyrenne2009}:
% {\color{red} I think the correct formula is 
% \[ \qquad n_i^{BQ} \defeq C-\left((K-i) - \sum_{j=i}^{K-1} \frac{r_j}{r_{j+1}} \right) \cdot \crr^{BQ} \cdot C \qquad i\in[K]\]
% I checked some of the proofs in which we use this quantity. To me, those are correct because you  used $\Delta n_i^{BQ}$, and not $n_i^{BQ}$, and with $\Delta n_i^{BQ}$ will not get impacted with this change. In nay case, please check these yourselves. thank you!
% } 
\begin{align} \label{eq;bQ:nest size}
 {\color{black}\qquad n_i^{BQ} \defeq \left(i - \sum_{j=1}^{i-1} \frac{r_j}{r_{j+1}} \right) \cdot \crr^{BQ} \cdot C \qquad i\in[K]\,.}
\end{align}
Here, as shown by \cite{BallandQueyrenne2009}, $\crr^{BQ}$ is 
the CR of the corresponding booking limit policy when there is no partially patient agent (i.e., $M=0$), where we recall 
%when $M = 0$. More specifically, the definition of $\crr^{BQ}$ and $n_k^{BQ}$ are below: 
$
    \crr^{BQ} = \left(K - \sum_{i=1}^{K-1} \frac{r_i}{r_{i+1}}\right)^{-1}
$ is defined in equation \eqref{equation:bq_cr}.

\end{definition}

A natural question to ask would be how well does the BQ nested \po{}  algorithm perform when $M \geq 1$? From \cite{BallandQueyrenne2009}, we only know that this algorithm achieves a CR of $\crr^{BQ}$ when $M=0$. Note that when $M = 0$, the feature-augmented CR is the same as the traditional CR. The following theorem states that this nested \po{} algorithm achieves a (feature-augmented) CR of $\crr^{BQ}$   when $M \geq 1$. 

\begin{theorem}[CR of the BQ Nested POLYRA Algorithm]
\label{theorem:bq_polytope_same_cr}
  For any number of agents $K$ with the first $M \geq 1$ partially patient, a \po{} algorithm with the BQ nested polytope (defined in Definition \ref{def:bq_nest}) achieves a (feature-augmented) CR of $\crr^{BQ}$, where $\crr^{BQ}$ is defined in equation \eqref{equation:bq_cr}.
\end{theorem}

 The proof of Theorem \ref{theorem:bq_polytope_same_cr} can be found in Appendix \ref{appendix:bq_polytope_same_cr_proof}. Theorem \ref{theorem:bq_polytope_same_cr} is a special case of Theorem \ref{theorem:polyra_nested_performance}, which characterizes the CR for \textit{any} nested algorithm given its nest sizes. Theorem \ref{theorem:bq_polytope_same_cr} implies that the BQ nested \po{} algorithm achieves the same CR of $\crr^{BQ}$  for any value of $M$. As we will see later in Section \ref{section:beyond_three}, where we focus on nested polytopes, in general for $M \geq 1$, we can achieve a CR of $\crr^* > \crr^{BQ}$ by simply optimizing the nests according to an LP that we wil present later. %presented in Definition \ref{def:optimal_nested_algorithm}.

We now turn our attention to characterizing \textit{optimal} polytopes for the special case of $K= 2, 3$. As we will see, some of them are nested while others are not.
}



==> sections/5_-_two_types.tex <==
\section{Optimal POLYRA Algorithm with Two Types}
\label{section:two_type}
Consider a special case of our model for $K = 2$ types with rewards $r_1 < r_2$, where type $1$ is partially patient and type $2$ is impatient. It turns out that nested \po{} algorithms  are optimal here. We show in the following theorem that choosing the right nest sizes  achieves the optimal CR. We then provide some intuition for why choosing the BQ nested polytope (per Definition \ref{def:bq_nest}) provides a sub-optimal algorithm.

\begin{theorem}[Optimal Algorithm with Two Types] 
\label{thm:opt_2}
    When the number of types $K = 2$ and the number of partially patient types $M = 1$ with rewards $r_1 < r_2$ and per-period capacity $C$. Then, the nested \po{} algorithm with the nested   polytope $\feasible^{(2,1)}$ achieves a CR of $\frac{2}{3 - r_1 / r_2}$, where
    \begin{equation} 
    \label{eq:feasible_two_type}
    \feasible^{(2, 1)} = \nestedPolyra \left( \frac{C}{3 - r_1 / r_2}, C \right).
    \end{equation}
    %  {\color{red} deterministic or randomized? At least, let's make this clear in a footnote.}
    Furthermore, no {\color{black} deterministic} online algorithm can achieve a higher CR than $\frac{2}{3 - r_1 / r_2}$ hence proving that our \po{} algorithm with polytope $\feasible^{(2,1)}$ is optimal.
\end{theorem}

To get an intuition for this polytope $\feasible^{(2,1)}$, it is useful to compare it to $\nestedPolyra^{BQ}$, which is defined as follows. 
\begin{align} \label{eq:two_type_bq}
\nestedPolyra^{BQ} = \nestedPolyra \left( \frac{C}{2 - r_1 / r_2}, C \right).
\end{align}
Based on Theorem \ref{theorem:bq_polytope_same_cr}, the above polytope achieves a CR of $\frac{1}{2 - r_1/r_2}$, which is strictly smaller than $\frac{2}{3 - r_1 / r_2}$ from Theorem \ref{thm:opt_2}. Notice that the only difference between $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ is the choice of the first nest size $n_1$: $\frac{C}{3 - r_1/r_2}$ versus $\frac{C}{2 - r_1/r_2}$.  We now present an example to show how two polytopes' performance differ, as well as, a proof sketch for why our polytope $\feasible^{(2,1)}$ is optimal.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{nested_example_diagram.png} 
    \vspace{0.5em}
    \caption{Comparing $\nestedPolyra^{BQ}$ (left) and $\feasible^{(2,1)}$ (right) in the special case of $(K, M) = (2, 1)$, $r_1 = 1, r_2 = 1000$ and $C = 6$. In this case, $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ and $ \feasible^{(2,1)} = \nestedPolyra(2, 6)$.
    %$n_1 = 3$ for BQ while $n_1 = 2$ for our optimal polytope. 
    The first row represents the 6 capacity in the current time period, while the second row is for the next period. The 6 capacity in the top row is divided into light blue (can be assigned to either type 1 or type 2) and red (can be assigned to type 2 only). Type 1 agents are also allowed to occupy the striped blue region in the second row (but type 2 agents are not at the moment since type 2 agents are impatient). %Out of the 6 capacity for the next period, allow type 1 agents (who are partially patient) to take up $n_1$ out of 6 units. Such capacity cannot be used by type 2 agents in the current period because type 2 agents are impatient.
    %{\color{red} it seems that the dark black color in the caption is not the same as that in the second row.} They actually are (I checked). 
    }
    \label{fig:nested_comparison}
\end{figure}
{
\color{black}

\begin{example} 
\label{example:two_types}
Consider a concrete example with $r_1 = 1, r_2 = 1000$, $T = 1$, and $C = 6$. Here, $r_2$ is significantly larger than $r_1$, approaching infinity in the limit. In this scenario, our nested polytope $\feasible^{(2,1)}$ (from equation \eqref{eq:feasible_two_type}) and the BQ nested polytope (from equation \eqref{eq:two_type_bq}) become, asymptotically as $r_2 / r_1 \to \infty$, $\nestedPolyra(2, 6)$ and $\nestedPolyra(3, 6)$ respectively (see Figure \ref{fig:nested_comparison}).

Our optimal polytope reserves $C-n_1 = 6-2 = 4$ units of capacity for higher reward agents in each period, while the BQ polytope only reserves $C- n_1 = 6 - 3 = 3$ units. Now, let's examine how the \po{} algorithms with feasible polytope $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ react to a simple arrival sequence $I_1$, which includes a dummy second period with no agent arrivals: $I_1 = \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\}, I_2 = \{\}$.

Our \po{} algorithm with polytope $\feasible^{(2,1)} = \nestedPolyra(2, 6)$ accepts $2\cdot n_1 = 4$ out of $6$ type $1$ agents from $I_1$ and then accepts $C- n_1 = 4$ out of 6 type $2$ agents. It then provides service to 2 type $1$ agents and 4 type $2$ agents for a total reward of approximately $4000$, achieving a $2/3$ approximation to the optimal reward of $6000$ in $I_1$.

The BQ nested \po{} algorithm with polytope $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ accepts $2\cdot n_1 = 6$ type $1$ agents and 3 type $2$ agents from $I_1$, and provides service to 3 type $1$ agents and $C- n_1 = 3$ type $2$ agents for a total reward of approximately $3000$, achieving a $1/2$ approximation to the optimal reward in $I_1$.

The BQ nested \po{} algorithm services only 3 type $2$ agents, while our algorithm services 4. This difference arises because the BQ nested \po{} algorithm accepts too many type $1$ agents (6 instead of 4 in our algorithm). It is essential for any good algorithm to accept some type $1$ agents because a non-anticipating algorithm cannot predict if type $2$ agents will arrive after observing the first 6 type $1$ agents. However, the BQ nested \po{} algorithm is overly pessimistic about the arrival of type $2$ agents, accepting too many type $1$ agents. This leads to poor performance if type $2$ agents do arrive. In contrast, our nested \po{} algorithm achieves good performance in both cases, resulting in better worst-case performance.

{\color{black}We remark that while achieving an optimal CR does not guarantee our algorithm outperforms the BQ algorithm in every instance, our numerical studies in Section \ref{sec:numerical_studies} demonstrate that our optimized nested algorithm surpasses the BQ benchmark algorithm in more realistic input sequences that are not stylized under both feature-augmented and traditional notions of CRs.}


%Consider a concrete example where $r_1 = 1, r_2 = 1000$ and $T = 1, C = 6$. Here, $1000$ is taking the place of a very large number, where $r_2 / r_1 \to \infty$. In this case, our nested polytope $\feasible^{(2,1)}$ from equation \eqref{eq:feasible_two_type} and the BQ nested polytope from equation \eqref{eq:two_type_bq} are (asymptotically as $r_2 / r_1 \to \infty$) $\nestedPolyra(2, 6)$ and $\nestedPolyra(3, 6)$ respectively, see Figure \ref{fig:nested_comparison}. Our optimal polytope reserves $C-n_1 = 6-2 = 4$ units of capacity for higher reward agents in each period, while the BQ polytope only reserves $C- n_1 = 6 - 3 = 3$ units. 

%Consider how the \po{} algorithms with feasible polytope $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$  react to the following simple arrival sequence $I_1$, with a dummy second period with no agent arrivals (recall our first technical assumption from Section \ref{sec:technical_assumptions}).
%$$
%\begin{array}{rclcrcl}
 %   I_1 &=& \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\} &\qquad \qquad & I_2 &=& \{\}
%\end{array}
%$$
%\begin{itemize}[leftmargin=*]
  %  \item Our \po{} algorithm with polytope $\feasible^{(2,1)} = \nestedPolyra(2, 6)$ accepts $2\cdot n_1 = 4$ out of $6$ type $1$ agents from $I_1$ and then accepts $C- n_1 = 4$ out of 6 type 2 agents. It then provides service to 2 type 1 agents and 4 type 2 agents for a total reward of about $4000$, which achieves a 2/3 approximation to the optimal $6000$ reward in $I_1$
    
  %  \item The BQ nested \po{} algorithm with polytope $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ accepts $2\cdot n_1 = 6$ type 1 agents and 3 type 2 agents from $I_1$, and provides service to $3$ type 1 agents and $C- n_1 = 3$ type 2 agents for a total reward of about $3000$, achieving a $1/2$ approximation to the optimal reward in $I_1$.
%\end{itemize}

%We see that the BQ nested \po{} algorithm only services 3 type 2 agents, while our algorithm services 4. This is because the BQ nested \po{} algorithm accepted too many type 1 agents (6, as opposed to 4 for our algorithm). It is certainly necessary for any good algorithm to accept \textit{some} type 1 agents because a non-anticipating \footnote{\color{black}A non-anticipating algorithm is synonymous with an online algorithm, one which does not have access to the future and must make decisions only on what has been observed so far in the arrival sequence.} algorithm does not know after seeing the first 6 type 1 agents whether type 2 agents will actually arrive. However, the BQ nested \po{} algorithm is overly pessimistic about the arrival of type 2 agents, and thus accepts too many type 1 agents, causing the performance to suffer if type 2 agents do arrive. The BQ nested \po{} algorithm performs very well when type 2 agents do not arrive, and poorly if type 2 agents do arrive, whereas our nested \po{} algorithm achieves good performance in both cases, which results in a better worst-case performance. \footnote{\color{black}As the CR definition implies, achieving optimal CR does not imply our algorithm outperforms the BQ algorithm on every instance. Nonetheless, we show in our numerical studies (Section \ref{sec:numerical_studies}) that our optimized nested algorithm surpasses the BQ benchmark algorithm in more realistic input sequences that are not stylized.}
%{\color{red} what about adding such thing here or in a footnote:  }



% To see why no algorithm can achieve a CR higher than $2/3$, consider the following two arrival sequences $I^a = \{I^c_1, I^c_2\}$ and $I^b = \{I^d_1, I^d_2\}$, where $T = 2$. 
% \[
% \begin{array}{rlrl}
%     I^c_1 =& \{1, 1, 1, 1, 1, 1\} \qquad & I^c_2 =& \{ \} \\
%     I^d_1 =& \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\} \qquad &I^d_2 =& \{2, 2, 2, 2, 2, 2\}
% \end{array}
% \]

% The key to arguing our $2/3$ upper bound on the CR of any online algorithm is to notice that $I^c$ and $I^d$ are identical up until the 7th agent in period 1. Any online algorithm must accept the same number of type $1$ agents from $I^c_1$ and $I^d_1$ because an online algorithm cannot differentiate between them until after the first 6 type 1 agents arrive. 

% Any algorithm with a CR of $\crr$ must accept at least $\crr \cdot 6$ of these type 1 agents in both $I_c$ and $I^d$. However, doing so leaves only $2 \cdot 6 - \crr \cdot 6$ capacity remaining for type 2 agents. Regardless of how this capacity is divided among the $T = 2$ periods, the best CR this algorithm can achieve is approximately $\frac{1000 \cdot (12 - 6 \crr)}{12000} = 1 - \frac{1}{2} \crr$. We see that when $\crr = 2/3$ is precisely when $1 - \frac{1}{2} \crr = \crr$ which gives us the desired upper bound. {\color{red} again let's try to see if we can simplify this discussion. }
\end{example}
}




==> sections/5twotypes.tex <==
\section{Optimal POLYRA Algorithm with Two Types}
\label{section:two_type}
Consider a special case of our model for $K = 2$ types with rewards $r_1 < r_2$, where type $1$ is partially patient and type $2$ is impatient. It turns out that nested \po{} algorithms  are optimal here. We show in the following theorem that choosing the right nest sizes  achieves the optimal CR. We then provide some intuition for why choosing the BQ nested polytope (per Definition \ref{def:bq_nest}) provides a sub-optimal algorithm.

\begin{theorem}[Optimal Algorithm with Two Types] 
\label{thm:opt_2}
    When the number of types $K = 2$ and the number of partially patient types $M = 1$ with rewards $r_1 < r_2$ and per-period capacity $C$. Then, the nested \po{} algorithm with the nested   polytope $\feasible^{(2,1)}$ achieves a CR of $\frac{2}{3 - r_1 / r_2}$, where
    \begin{equation} 
    \label{eq:feasible_two_type}
    \feasible^{(2, 1)} = \nestedPolyra \left( \frac{C}{3 - r_1 / r_2}, C \right).
    \end{equation}
    %  {\color{red} deterministic or randomized? At least, let's make this clear in a footnote.}
    Furthermore, no {\color{black} deterministic} online algorithm can achieve a higher CR than $\frac{2}{3 - r_1 / r_2}$ hence proving that our \po{} algorithm with polytope $\feasible^{(2,1)}$ is optimal.
\end{theorem}

To get an intuition for this polytope $\feasible^{(2,1)}$, it is useful to compare it to $\nestedPolyra^{BQ}$, which is defined as follows. 
\begin{align} \label{eq:two_type_bq}
\nestedPolyra^{BQ} = \nestedPolyra \left( \frac{C}{2 - r_1 / r_2}, C \right).
\end{align}
Based on Theorem \ref{theorem:bq_polytope_same_cr}, the above polytope achieves a CR of $\frac{1}{2 - r_1/r_2}$, which is strictly smaller than $\frac{2}{3 - r_1 / r_2}$ from Theorem \ref{thm:opt_2}. Notice that the only difference between $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ is the choice of the first nest size $n_1$: $\frac{C}{3 - r_1/r_2}$ versus $\frac{C}{2 - r_1/r_2}$.  We now present an example to show how two polytopes' performance differ, as well as, a proof sketch for why our polytope $\feasible^{(2,1)}$ is optimal.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{nested_example_diagram.png} 
    \vspace{0.5em}
    \caption{Comparing $\nestedPolyra^{BQ}$ (left) and $\feasible^{(2,1)}$ (right) in the special case of $(K, M) = (2, 1)$, $r_1 = 1, r_2 = 1000$ and $C = 6$. In this case, $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ and $ \feasible^{(2,1)} = \nestedPolyra(2, 6)$.
    %$n_1 = 3$ for BQ while $n_1 = 2$ for our optimal polytope. 
    The first row represents the 6 capacity in the current time period, while the second row is for the next period. The 6 capacity in the top row is divided into light blue (can be assigned to either type 1 or type 2) and red (can be assigned to type 2 only). Type 1 agents are also allowed to occupy the striped blue region in the second row (but type 2 agents are not at the moment since type 2 agents are impatient). %Out of the 6 capacity for the next period, allow type 1 agents (who are partially patient) to take up $n_1$ out of 6 units. Such capacity cannot be used by type 2 agents in the current period because type 2 agents are impatient.
    %{\color{red} it seems that the dark black color in the caption is not the same as that in the second row.} They actually are (I checked). 
    }
    \label{fig:nested_comparison}
\end{figure}
{
\color{black}

\begin{example} 
\label{example:two_types}
Consider a concrete example with $r_1 = 1, r_2 = 1000$, $T = 1$, and $C = 6$. Here, $r_2$ is significantly larger than $r_1$, approaching infinity in the limit. In this scenario, our nested polytope $\feasible^{(2,1)}$ (from equation \eqref{eq:feasible_two_type}) and the BQ nested polytope (from equation \eqref{eq:two_type_bq}) become, asymptotically as $r_2 / r_1 \to \infty$, $\nestedPolyra(2, 6)$ and $\nestedPolyra(3, 6)$ respectively (see Figure \ref{fig:nested_comparison}).

Our optimal polytope reserves $C-n_1 = 6-2 = 4$ units of capacity for higher reward agents in each period, while the BQ polytope only reserves $C- n_1 = 6 - 3 = 3$ units. Now, let's examine how the \po{} algorithms with feasible polytope $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ react to a simple arrival sequence $I_1$, which includes a dummy second period with no agent arrivals: $I_1 = \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\}, I_2 = \{\}$.

Our \po{} algorithm with polytope $\feasible^{(2,1)} = \nestedPolyra(2, 6)$ accepts $2\cdot n_1 = 4$ out of $6$ type $1$ agents from $I_1$ and then accepts $C- n_1 = 4$ out of 6 type $2$ agents. It then provides service to 2 type $1$ agents and 4 type $2$ agents for a total reward of approximately $4000$, achieving a $2/3$ approximation to the optimal reward of $6000$ in $I_1$.

The BQ nested \po{} algorithm with polytope $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ accepts $2\cdot n_1 = 6$ type $1$ agents and 3 type $2$ agents from $I_1$, and provides service to 3 type $1$ agents and $C- n_1 = 3$ type $2$ agents for a total reward of approximately $3000$, achieving a $1/2$ approximation to the optimal reward in $I_1$.

The BQ nested \po{} algorithm services only 3 type $2$ agents, while our algorithm services 4. This difference arises because the BQ nested \po{} algorithm accepts too many type $1$ agents (6 instead of 4 in our algorithm). It is essential for any good algorithm to accept some type $1$ agents because a non-anticipating algorithm cannot predict if type $2$ agents will arrive after observing the first 6 type $1$ agents. However, the BQ nested \po{} algorithm is overly pessimistic about the arrival of type $2$ agents, accepting too many type $1$ agents. This leads to poor performance if type $2$ agents do arrive. In contrast, our nested \po{} algorithm achieves good performance in both cases, resulting in better worst-case performance.

{\color{black}We remark that while achieving an optimal CR does not guarantee our algorithm outperforms the BQ algorithm in every instance, our numerical studies in Section \ref{sec:numerical_studies} demonstrate that our optimized nested algorithm surpasses the BQ benchmark algorithm in more realistic input sequences that are not stylized under both feature-augmented and traditional notions of CRs.}


%Consider a concrete example where $r_1 = 1, r_2 = 1000$ and $T = 1, C = 6$. Here, $1000$ is taking the place of a very large number, where $r_2 / r_1 \to \infty$. In this case, our nested polytope $\feasible^{(2,1)}$ from equation \eqref{eq:feasible_two_type} and the BQ nested polytope from equation \eqref{eq:two_type_bq} are (asymptotically as $r_2 / r_1 \to \infty$) $\nestedPolyra(2, 6)$ and $\nestedPolyra(3, 6)$ respectively, see Figure \ref{fig:nested_comparison}. Our optimal polytope reserves $C-n_1 = 6-2 = 4$ units of capacity for higher reward agents in each period, while the BQ polytope only reserves $C- n_1 = 6 - 3 = 3$ units. 

%Consider how the \po{} algorithms with feasible polytope $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$  react to the following simple arrival sequence $I_1$, with a dummy second period with no agent arrivals (recall our first technical assumption from Section \ref{sec:technical_assumptions}).
%$$
%\begin{array}{rclcrcl}
 %   I_1 &=& \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\} &\qquad \qquad & I_2 &=& \{\}
%\end{array}
%$$
%\begin{itemize}[leftmargin=*]
  %  \item Our \po{} algorithm with polytope $\feasible^{(2,1)} = \nestedPolyra(2, 6)$ accepts $2\cdot n_1 = 4$ out of $6$ type $1$ agents from $I_1$ and then accepts $C- n_1 = 4$ out of 6 type 2 agents. It then provides service to 2 type 1 agents and 4 type 2 agents for a total reward of about $4000$, which achieves a 2/3 approximation to the optimal $6000$ reward in $I_1$
    
  %  \item The BQ nested \po{} algorithm with polytope $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ accepts $2\cdot n_1 = 6$ type 1 agents and 3 type 2 agents from $I_1$, and provides service to $3$ type 1 agents and $C- n_1 = 3$ type 2 agents for a total reward of about $3000$, achieving a $1/2$ approximation to the optimal reward in $I_1$.
%\end{itemize}

%We see that the BQ nested \po{} algorithm only services 3 type 2 agents, while our algorithm services 4. This is because the BQ nested \po{} algorithm accepted too many type 1 agents (6, as opposed to 4 for our algorithm). It is certainly necessary for any good algorithm to accept \textit{some} type 1 agents because a non-anticipating \footnote{\color{black}A non-anticipating algorithm is synonymous with an online algorithm, one which does not have access to the future and must make decisions only on what has been observed so far in the arrival sequence.} algorithm does not know after seeing the first 6 type 1 agents whether type 2 agents will actually arrive. However, the BQ nested \po{} algorithm is overly pessimistic about the arrival of type 2 agents, and thus accepts too many type 1 agents, causing the performance to suffer if type 2 agents do arrive. The BQ nested \po{} algorithm performs very well when type 2 agents do not arrive, and poorly if type 2 agents do arrive, whereas our nested \po{} algorithm achieves good performance in both cases, which results in a better worst-case performance. \footnote{\color{black}As the CR definition implies, achieving optimal CR does not imply our algorithm outperforms the BQ algorithm on every instance. Nonetheless, we show in our numerical studies (Section \ref{sec:numerical_studies}) that our optimized nested algorithm surpasses the BQ benchmark algorithm in more realistic input sequences that are not stylized.}
%{\color{red} what about adding such thing here or in a footnote:  }



% To see why no algorithm can achieve a CR higher than $2/3$, consider the following two arrival sequences $I^a = \{I^c_1, I^c_2\}$ and $I^b = \{I^d_1, I^d_2\}$, where $T = 2$. 
% \[
% \begin{array}{rlrl}
%     I^c_1 =& \{1, 1, 1, 1, 1, 1\} \qquad & I^c_2 =& \{ \} \\
%     I^d_1 =& \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\} \qquad &I^d_2 =& \{2, 2, 2, 2, 2, 2\}
% \end{array}
% \]

% The key to arguing our $2/3$ upper bound on the CR of any online algorithm is to notice that $I^c$ and $I^d$ are identical up until the 7th agent in period 1. Any online algorithm must accept the same number of type $1$ agents from $I^c_1$ and $I^d_1$ because an online algorithm cannot differentiate between them until after the first 6 type 1 agents arrive. 

% Any algorithm with a CR of $\crr$ must accept at least $\crr \cdot 6$ of these type 1 agents in both $I_c$ and $I^d$. However, doing so leaves only $2 \cdot 6 - \crr \cdot 6$ capacity remaining for type 2 agents. Regardless of how this capacity is divided among the $T = 2$ periods, the best CR this algorithm can achieve is approximately $\frac{1000 \cdot (12 - 6 \crr)}{12000} = 1 - \frac{1}{2} \crr$. We see that when $\crr = 2/3$ is precisely when $1 - \frac{1}{2} \crr = \crr$ which gives us the desired upper bound. {\color{red} again let's try to see if we can simplify this discussion. }
\end{example}
}




==> sections/6_-_three_types.tex <==
\section{Optimal Algorithm with Three Types}
\label{section:three_type}
In this section, we consider a special case with $K = 3$ and $M\in \{1, 2\}$. Our main result in this section is an explicit characterization of two polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$ (defined in equations \eqref{eq:feasibleMOne} and \eqref{feasibleMTwo}) which give optimal \po{} algorithms for the case when $M = 1$ and $M = 2$, respectively. We present an innovative technique where we first construct an upper bound on the CR of any online algorithm through an LP, and then use its optimal solution values to build our polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$.
%{\color{red} It seems that you start using this notation $\feasible^{(K, M)}$. But, never defined it formally. } 
%Interestingly for $M = 1$, we show that the optimal polytope is not nested and in fact no nested polytope can achieve this performance. %{\color{red} remove ``and in fact no nested polytope can achieve this performance" as I don't think we have this result.}

% { \color{black} I think the reader can get lost here because the sub-sections are so long. It would be good to add a high-level summary of our approach.
% Outline of Our Approach 
% \begin{enumerate}
%     \item We construct an upper bound on the CR of any non-anticipating algorithm by considering how the algorithm behaves against a worst-case arrival sequence. Each constraint of the LP 
    
%     \item Using the solution variables $s_{i,t}$, we construct polytopes which \textit{mimic} this behavior against the worst-case input. 
    
%     \item We prove that our polytopes also perform well on other arrival sequences, besides the worst-case. 
% \end{enumerate}
% }

\subsection{An Upper Bound for Three Types}

In order to prove the optimality of our algorithms for $K = 3$, we first need to establish an upper bound. To do so, for each of $M = 1$ and $M = 2$, we construct  \textit{worst-case arrival sequences}, which best exemplify the main challenge that an online algorithm must face: the trade-off between a moderate reward now versus waiting for a potentially higher future reward. We then argue that to obtain a CR of $\crr$ on these worst-case arrival sequences, the behavior of non-anticipating algorithm needs to satisfy certain conditions. These conditions  lead to  an LP construction, where  the objective of the LP maximizes the CR (i.e., $\crr $ in the LP) and the constraints enforce the aforementioned conditions.

\begin{theorem}[Upper Bound on the CR with Three Types]
  \label{thm:3_type_upper_bound}
  Suppose that there are three types with $M\in \{1, 2\}$ and rewards $r_1 < r_2 < r_3$. Then, the CR of any non-anticipating algorithm $\mathcal {A}$, i.e.,  $\text{CR}_{\mathcal A}$, is at most the optimal value of the following LP, denoted by $\crr_{up}$. %{\color{red}changed the notation here.}
  \begin{align}
   \crr_{up} \defeq \max_{\crr, \{\optupper_{i,t}\}_{i\in[3], t\in[2]}} \quad && \crr & \nonumber \\
    \text{s.t.} \quad &   & \optOnet + \optTwot + \optupper_{3,t} & \leq C                                                                         & t \in [2] \label{align:Ia_capacity} \\
                      &   & \crr \cdot r_3 \cdot C                & \leq \optOnet \cdot r_1 + \optTwot \cdot r_2 + \optupper_{3,t} \cdot r_3       & t \in [2] \label{align:Ia_revenue}  \\
    \lplabel[3_class_ub]{\textsc{(upper3)}}  && \crr \cdot r_1 \cdot C &\leq(\optOneOne + \optOneTwo) \cdot r_1 \label{align:Id_revenue} \\
    && \crr \cdot r_2 \cdot C &\leq \left(C - \sum_{t=1}^M \optTwot \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_capacity}\\
    && \crr \cdot r_2 \cdot C &\leq \left(\optOneOne + \optOneTwo \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_revenue}\\
                      &   & \crr \cdot r_2 \cdot C                & \leq \optOneTwo \cdot r_1 + \optupper_{2,2} \cdot r_2 \label{align:Ib_revenue} & \text{if $M = 1$}\\
                      & & {\color{black} s_{i, t}} & {\color{black}\ge 0\, ,\quad  \crr \ge 0}\, &i\in [3], t\in [2]
  \end{align}
\end{theorem}
%{\color{red} let's make sure in all the LP's, we state the non-negativity constraints. I did it above per the referees' comments. But, the equations are not well aligned. Could you please fix this?}
%Note that in LP \ref{3_class_ub} and all other LPs presented in this paper, we assume that all decision variables are non-negative.
Next, we present a proof sketch of Theorem \ref{thm:3_type_upper_bound}. The complete proof of this theorem and the proof of all other statements in this section are presented in Section \ref{secproofthree}.

\begin{proof}{Proof Sketch of Theorem \ref{thm:3_type_upper_bound}.}
  In this proof sketch, we outline the general structure of all the upper bounds presented in this paper. Our upper bound construction takes advantage of the fact that any non-anticipating algorithm $\alg$ does not know the future, and therefore is unable to differentiate between two arrival sequences  $I$ and $I'$ until the first index at which they differ. Using this idea, we build our upper bounds around a collection of overlapping multi-period arrival sequences $\mathcal{I}$, and argue that any non-anticipating algorithm $\alg$ that claims to be $\crr$-competitive must satisfy certain conditions when dealing with each arrival sequence $\{I_t\}_{t \in [T]} \in \mathcal{I}$. We write down these conditions in terms of an LP, maximize the value of $\crr$, and get our upper bound.

  To demonstrate our idea, let us consider an example where $K = 3$, $M = 1$, and $C = 3$. Our proof can be extended to any value of $C$ and also for $M=2$. Consider the following arrival sequence $\{I_1, I_2\}$ over the course of $T=2$ time periods. 
    \[
        \begin{array}{ll}
            I_1 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2 = \{ 2, 2, 2,\: 3, 3, 3  \}
        \end{array}
    \]
    We can define the following \textit{truncations} of $\{I_1, I_2\}$ which consist of abruptly ending the entire input sequence after a certain type of agent has arrived. For example, $\{I_1^2, I_2^2\}$ represents the truncation of $\{I_1, I_2\}$ where the entire 2-period input suddenly ends after type $2$ agents arrive in the first time period.
    \[\arraycolsep=1.4pt\def\arraystretch{1.5}
        \begin{array}{ll}
            I_1^1 = \{ 1, 1, 1\} \quad                                    & I_2^1 = \{  \}         \\
            I_1^2 = \{ 1, 1, 1, \: 2, 2, 2\} \quad                        & I_2^2 = \{  \}         \\
            I_1^3 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3\} \quad             & I_2^3 = \{  \}         \\
            I_1^4 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2^4 = \{2, 2, 2  \}  \\
        \end{array}
    \]
%  $\{I_1, I_2\}$ is chosen so that we send agents in ascending order of reward over 2 time periods, while making sure all agents can be served within 2 time periods (hence not having partially patient type $1$ in $I_2$). %Such an arrival sequence best captures the core challenge of online resource allocation: the tension between committing to lower reward agents early on and waiting for higher reward agents that might not arrive. 
  
{\color{red} removed a paragraph here.} The truncated arrival sequences $\{I_1^j, I_2^j\}$ for $j \in [4]$ demonstrate that achieving a high CR requires an algorithm, $\alg$, to effectively balance performance across both $\{I_1, I_2\}$ and $\{I_1^j, I_2^j\}$ sequences. Given the overlap in these sequences, any algorithm's response to them is interconnected. For instance, if $\alg$ accepts only type 3 agents in $\{I_1, I_2\}$, maximizing the reward, it would fail to earn any reward on sequence $\{I_1^1, I_2^1\}$, as its actions up to the arrival of type 1 agents would remain unchanged between the two sequences.

  Using the ideas from the example above, we now give a sketch of how the constraints in \ref{3_class_ub} come about. Suppose we are given an algorithm $\alg$ which is $\crr$ competitive. Let $s_{i,t}$, $i \in [3], t \in [2]$, be the number of type $i$ agents that are serviced in period $t$ under $\alg$. Since types $2$ and $3$ are impatient, $s_{i,t}$ also represents the number of type $2$ and $3$ agents that $\alg$ accepts from $I_t$, while for type $1$, $s_{1,1} + s_{1,2}$ is the number of type $1$ agents that $\alg$ accepts from $I_1$. Since $\textsc{opt}_t(\{I_1, I_2\}) = r_3 \cdot C$, to be $\crr$-competitive, we must have   $\textsc{rew}_{\alg, t}(\{I_1, I_2\}) = r_1 \cdot s_{1,t} + r_2 \cdot s_{2,t} + r_3 \cdot s_{3,t} \geq \crr \cdot r_3 \cdot C$, which gives rise to constraint \eqref{align:Ia_revenue}. In addition, we certainly must have $s_{1,t} + s_{2,t} + s_{3,t} \leq C$, as given in \eqref{align:Ia_capacity}. We apply a similar reasoning
  to arrival sequences $\{I_1^1, I_2^1\}, \{I_1^2, I_2^2\}$ and $\{I_1^4, I_2^4\}$, to get the $\crr \cdot r_i \cdot C$ (for $i= 1$ or $2$) reward lower bounds in constraints \eqref{align:Id_revenue}, \eqref{align:Ic_revenue}, \eqref{align:Ic_capacity}, and \eqref{align:Ib_revenue}.\footnote{Note that $\{I^3_1, I^3_2\}$ is actually not useful as it would imply the constraint $r_1 \cdot s_{1,1} + r_2 \cdot s_{2,1} + r_3 \cdot s_{3,1} \geq \crr \cdot r_3 \cdot C$, which was already captured by $\{I_1, I_2\}$.} 
  \Halmos
\end{proof}

We will now state two \po{} algorithms which achieve the $\crr_{up}$ CR from the upper bound, one for the case where $M =1$ and another for $M = 2$. Both of these optimal algorithms require us to first compute the upper bound presented above, get an optimal solution $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in [2]})$ and use some of these values as constants in the feasible polytopes $\feasibleMOne$ for $M = 1$ and $\feasibleMTwo$ for $M = 2$. We will require some properties of this optimal upper bound solution, which are described in Lemmas \ref{lemma:3_class_tight_properties} and \ref{lemma:3_type_additional_properties} in Appendix \ref{sec:lemma:3_class_tight_properties} and \ref{sec:lemma:3_type_additional_properties}. We highlight that the upper bound only characterizes an optimal algorithm's behavior against our constructed worst-case arrival sequences, not any arbitrary arrival sequences over $T$ periods. Nonetheless, we show that how to use the upper bound solution, which represents a particular way of dealing with the worst-case arrival sequence, to construct an optimal algorithm for any arrival sequence.

\subsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 1$}{M=1}}
With $M=1$, type $1$ agents are partially patient while types $2$ and $3$ are impatient. Hence,  our state $\stateB$ contains 4 buckets as shown below:
\[ \begin{array}{r|ccc}
    \text{Type}  & 1               & 2          & 3          \\ \hline
    \text{Row 1} & \bucketij{1}{1} & \bucket{2} & \bucket{3} \\
    \text{Row 2} & \bucketij{1}{2} &            &
  \end{array} \]

Let  $\Delta_{i,j} \defeq r_i - r_j$ and $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ be the optimal solution to the upper bound LP \ref{3_class_ub}. We define our feasible polytope $\feasibleMOne$ as follows
\begin{align} \label{eq:feasibleMOne}  \feasible^{(3,1)} = \left\{ (\fbucketOneOne, \fbucketOneTwo, \fbucketTwo, \fbucketThree) \subset \mathbb{R}_+^4: \quad  \begin{array}{cll}
    \fbucketOneOne + \fbucketTwo + \fbucketThree                       & \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*                           &           \\
    \Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo & \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^* &           \\
    \fbucketOnei                                                       & \leq \optupper_{1,i}^*                                           & i \in [2]\end{array} \right\}\end{align}

\begin{theorem}[Optimality of \textsc{POLYRA} Algorithm with  Feasible  Polytope $\feasibleMOne$]
  \label{thm:opt_alg_M=1} When the number of types $K = 3$ and the number of partially patient types $M = 1$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the \po{} algorithm with feasible polytope $\feasibleMOne$ achieves a CR of $\crr_{up}$, and hence, is optimal. Here, $\crr_{up}$ %{\color{red} I think you are overloading notation $\crr^*$. Did not you use it for the nested algorithms both in the introduction and other parts of the paper. } 
  is the optimal objective value of the LP \ref{3_class_ub}.
\end{theorem}

\textbf{Discussion on Feasible Polytope $\feasibleMOne$.}
Here, we give some intuition about the constraints of $\feasibleMOne$ and why it achieves a CR of $\crr_{up}$. The first constraint, i.e., $\fbucketOneOne + \fbucketTwo + \fbucketThree \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$  simply enforces that we do not allocate more resources in a time period than $s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$ which is bounded above by $C$ as per constraint \eqref{align:Ia_capacity} of the upper bound LP \ref{3_class_ub}. In fact, as we show in property \ref{property:total_is_C} of Lemma \ref{lemma:3_class_tight_properties}, we actually have $\optupper_{1,1}^* + \optupper_{2,1}^* + \optupper_{3,1}^* = C$. The purpose of the second constraint, i.e., $\Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^*$, is to leave enough space in bucket $\bucketThree$ for type $3$ agents, which we do so by enforcing that a linear combination of the number of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ is not too large. Finally, the last constraint, i.e., $\fbucketOnei \leq \optupper_{1,i}^*, i \in [2]$,  simply makes sure that our buckets do not contain too many type $1$ agents in order to leave enough room for the type $2$ and $3$ agents. 

Observe that the feasible polytope $\feasibleMOne$ is not a nested polytope as per Definition \ref{def:nested}. In particular, in order to obtain the optimal CR of $\crr_{up}$, the algorithm has to keep track of a linear combination of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ (i.e., $\Delta_{3,1} \cdot \bucketOneOne + \Delta_{3,2} \cdot \bucketTwo$), rather than simply the sum of the agents assigned to these two buckets (i.e., $ \bucketOneOne + \bucketTwo$).

It can be shown that if we apply our \po{} algorithm with feasible polytope $\feasibleMOne$ to the worst-case arrival sequence from  $\{I_1, I_2\}$ as defined in the proof sketch of Theorem \ref{thm:3_type_upper_bound}, then the behavior of this algorithm will exactly correspond to the optimal solution $\{s_{i,t}^*\}$ in that our algorithm will serve exactly $s_{i,t}^*$ agents of type $i$ in period $t \in [2]$. In this way, our \po{} algorithm \textit{mimics} the upper bound when it encounters the worst-case arrival sequence. In Theorem \ref{thm:opt_alg_M=1}, we show that our algorithm also achieves the optimal CR on any arrival sequence, not just this worst-case arrival sequence. We now describe our polytope construction for three types when $M = 2$.

% We now comment on the proof idea of Theorem \ref{thm:opt_alg_M=1}. First, we note that the polytope $\feasibleMOne$ is consistent as per Lemma \ref{lemma:3_type_valid} which is proven in Section \ref{sec:lemma:3_type_valid}. This is crucial because recall that \po{} algorithms are only well defined when the feasible polytope is consistent. Since our polytope $\feasibleMOne$ contains many terms from the optimal upper bound LP solution (i.e. $\{s_{i,t}^*\}_{i\in[3], t \in [2]}$), we also need to show some properties of this optimal upper bound solution, which are stated in Lemmas \ref{lemma:3_class_tight_properties}, \ref{lemma:3_type_additional_properties} and proven in Sections \ref{sec:lemma:3_class_tight_properties}, \ref{sec:lemma:3_type_additional_properties}. We then show that our proposed \po{} algorithm  obtains the optimal CR against \textit{any} arrival sequence through the following casework. Suppose that for a period $t$, our state after the arrival phase is $\stateB$ and let $\ell \in \{0, 1, 2, 3\}$ be the \textit{highest} type of agent for which all the available space in $\stateB$ for type $\ell$ agents is occupied. In other words, if we were to encounter one more type $\ell$ agent, we would completely reject that agent. We define $\ell = 0$ if $\stateB$ can accommodate some positive amount of another agent of any type and still remain feasible. By our definition of $\ell$, it must be the case that $\stateB$ is able to accommodate an agent of type $k$ for all $k > \ell$. By property (ii) of consistency (Definition \ref{def:consistent}), this implies that our algorithm has not rejected a single agent of type $k$, which means that our algorithm is doing just as well as the optimal solution when it comes to type $k$ agents. For types $k' < \ell$, we may have rejected some agents that the optimal clairvoyant solution accepted, but we show that we have accepted enough such agents of type $k' < \ell$ to be $\crr^*$-competitive.



\subsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 2$}{M=2}}
With $M=2$, types $1,2$ agents are partially patient while type $3$ agents are impatient. Hence, our state $\stateB$ contains 5 buckets as shown below:
\[ \begin{array}{r|ccc}
    \text{Type}   & 1               & 2               & 3          \\ \hline
    \text{Type 1} & \bucketij{1}{1} & \bucketij{2}{1} & \bucket{3} \\
    \text{Type 2} & \bucketij{1}{2} & \bucketij{2}{2} &
  \end{array} \]

To construct the optimal algorithm for three types with two partially patient types, we  first compute the optimal solution $\left(\crr_{up}, \{s_{i,t}^*\}_{i \in [3], t \in [2]} \right)$ from the upper bound LP \ref{3_class_ub} in Theorem \ref{thm:3_type_upper_bound} and use it to construct our polytope $\feasibleMTwo$, which is defined in the following theorem.

\begin{theorem}[Optimal Algorithm for $K=3$ and $M=2$]
  \label{theorem:three_type_M=2}
 When the number of types $K = 3$ and the number of partially patient types $M = 2$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the nested \po{} algorithm with the {nested} polytope $\feasibleMTwo$, defined below, achieves a CR of $\crr_{up}$, and hence, is optimal:
  \begin{equation}\label{feasibleMTwo}
    \feasible^{(3,2)} \defeq \nestedPolyra\left(\frac{1}{2} \cdot (\optupper_{1,1}^* + \optupper_{1,2}^* ), \frac{1}{2} \cdot \left( \optupper_{1,1}^* + \optupper_{1,2}^* + \optupper_{2,1}^* +\optupper_{2,2}^*  \right)  , C \right) \, .
  \end{equation}
  Here, $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ is the optimal solution to the upper bound LP \ref{3_class_ub} and nested polytopes $\nestedPolyra$ are defined in Definition \ref{def:nested}.
\end{theorem}

\textbf{Discussion on the nested polytope $\feasibleMTwo$ and the optimal algorithm.} With two partially patient types (i.e., $M=2$), the optimal algorithm takes the form of a simple nested \po{} algorithm as per Definition \ref{def:nested}. Just like with 1 partially patient type, one can show that if we apply our \po{} algorithm with feasible polytope $\feasibleMTwo$ to the corresponding worst-case arrival sequence for $M = 2$, our \po{} algorithm will exactly serve $s_{i,t}^*$ agents of type $i\in[3]$ in time period $t\in [2]$. In this sense, we again mimic our upper bound solution as a template for making sure our algorithm is $\crr_{up}$-competitive against the worst-case arrival. It turns out that this worst-case arrival sequence is indeed the worst-case as achieving a $\crr_{up}$ CR on it implies a $\crr_{up}$ CR on all arrival sequences. To prove that such a nested polytope achieves the desired CR of $\crr_{up}$, we will apply Theorem \ref{theorem:polyra_nested_performance}, which uses an LP to characterize the CR of \textit{any} nested polytope, including ones for $K > 3$ types.

While $\feasibleMOne$ is not a nested polytope, $\feasibleMTwo$ is. Recall from the earlier discussion that $\feasibleMOne$ is not nested because it has a constraint of the form $c_1 \cdot b_{1,1} + c_2 \cdot b_2 \leq c_3$ where $c_1 \neq c_2$. On the other hand, all of  $\feasibleMTwo$'s constraints involve a linear combination of variables with coefficients all equal to $1$. This can be explained by the following intuition: Both polytopes $\feasibleMOne$ and $\feasibleMTwo$ have constraints which make sure that we do not accept too many type $1$ or $2$ agents, thus making sure enough space is reserved for type $3$ agents. When type $1$ is partially patient and type $2$ is not (i.e. $M = 1$), this constraint is of the form $\Delta_{3,1} \cdot b_{1,1} + \Delta_{3,2} \cdot b_{2}$ where the coefficients $\Delta_{3,1}\neq \Delta_{3,2}$. This is because type $1$ and $2$ differ in their flexibility so our linear combination must weigh the two differently. On the other hand, when both type $1$ and type $2$ are partially patient (i.e $M = 2$), restricting the simple sum of $b_{1,1}$ and $b_{2,1}$ is sufficient.



==> sections/6threetypes.tex <==
\section{Optimal Algorithm with Three Types}
\label{section:three_type}
In this section, we consider a special case with $K = 3$ and $M\in \{1, 2\}$. Our main result in this section is an explicit characterization of two polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$ (defined in equations \eqref{eq:feasibleMOne} and \eqref{feasibleMTwo}) which give optimal \po{} algorithms for the case when $M = 1$ and $M = 2$, respectively. We present an innovative technique where we first construct an upper bound on the CR of any online algorithm through an LP, and then use its optimal solution values to build our polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$.
%{\color{red} It seems that you start using this notation $\feasible^{(K, M)}$. But, never defined it formally. } 
%Interestingly for $M = 1$, we show that the optimal polytope is not nested and in fact no nested polytope can achieve this performance. %{\color{red} remove ``and in fact no nested polytope can achieve this performance" as I don't think we have this result.}

% { \color{black} I think the reader can get lost here because the sub-sections are so long. It would be good to add a high-level summary of our approach.
% Outline of Our Approach 
% \begin{enumerate}
%     \item We construct an upper bound on the CR of any non-anticipating algorithm by considering how the algorithm behaves against a worst-case arrival sequence. Each constraint of the LP 
    
%     \item Using the solution variables $s_{i,t}$, we construct polytopes which \textit{mimic} this behavior against the worst-case input. 
    
%     \item We prove that our polytopes also perform well on other arrival sequences, besides the worst-case. 
% \end{enumerate}
% }

\subsection{An Upper Bound for Three Types}

In order to prove the optimality of our algorithms for $K = 3$, we first need to establish an upper bound. To do so, for each of $M = 1$ and $M = 2$, we construct  \textit{worst-case arrival sequences}, which best exemplify the main challenge that an online algorithm must face: the trade-off between a moderate reward now versus waiting for a potentially higher future reward. We then argue that to obtain a CR of $\crr$ on these worst-case arrival sequences, the behavior of non-anticipating algorithm needs to satisfy certain conditions. These conditions  lead to  an LP construction, where  the objective of the LP maximizes the CR (i.e., $\crr $ in the LP) and the constraints enforce the aforementioned conditions.

\begin{theorem}[Upper Bound on the CR with Three Types]
  \label{thm:3_type_upper_bound}
  Suppose that there are three types with $M\in \{1, 2\}$ and rewards $r_1 < r_2 < r_3$. Then, the CR of any non-anticipating algorithm $\mathcal {A}$, i.e.,  $\text{CR}_{\mathcal A}$, is at most the optimal value of the following LP, denoted by $\crr_{up}$. %{\color{red}changed the notation here.}
  \begin{align}
   \crr_{up} \defeq \max_{\crr, \{\optupper_{i,t}\}_{i\in[3], t\in[2]}} \quad && \crr & \nonumber \\
    \text{s.t.} \quad &   & \optOnet + \optTwot + \optupper_{3,t} & \leq C                                                                         & t \in [2] \label{align:Ia_capacity} \\
                      &   & \crr \cdot r_3 \cdot C                & \leq \optOnet \cdot r_1 + \optTwot \cdot r_2 + \optupper_{3,t} \cdot r_3       & t \in [2] \label{align:Ia_revenue}  \\
    \lplabel[3_class_ub]{\textsc{(upper3)}}  && \crr \cdot r_1 \cdot C &\leq(\optOneOne + \optOneTwo) \cdot r_1 \label{align:Id_revenue} \\
    && \crr \cdot r_2 \cdot C &\leq \left(C - \sum_{t=1}^M \optTwot \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_capacity}\\
    && \crr \cdot r_2 \cdot C &\leq \left(\optOneOne + \optOneTwo \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_revenue}\\
                      &   & \crr \cdot r_2 \cdot C                & \leq \optOneTwo \cdot r_1 + \optupper_{2,2} \cdot r_2 \label{align:Ib_revenue} & \text{if $M = 1$}\\
                      & & {\color{black} s_{i, t}} & {\color{black}\ge 0\, ,\quad  \crr \ge 0}\, &i\in [3], t\in [2]
  \end{align}
\end{theorem}
%{\color{red} let's make sure in all the LP's, we state the non-negativity constraints. I did it above per the referees' comments. But, the equations are not well aligned. Could you please fix this?}
%Note that in LP \ref{3_class_ub} and all other LPs presented in this paper, we assume that all decision variables are non-negative.
Next, we present a proof sketch of Theorem \ref{thm:3_type_upper_bound}. The complete proof of this theorem and the proof of all other statements in this section are presented in Section \ref{secproofthree}.

\begin{proof}{Proof Sketch of Theorem \ref{thm:3_type_upper_bound}.}
  In this proof sketch, we outline the general structure of all the upper bounds presented in this paper. Our upper bound construction takes advantage of the fact that any non-anticipating algorithm $\alg$ does not know the future, and therefore is unable to differentiate between two arrival sequences  $I$ and $I'$ until the first index at which they differ. Using this idea, we build our upper bounds around a collection of overlapping multi-period arrival sequences $\mathcal{I}$, and argue that any non-anticipating algorithm $\alg$ that claims to be $\crr$-competitive must satisfy certain conditions when dealing with each arrival sequence $\{I_t\}_{t \in [T]} \in \mathcal{I}$. We write down these conditions in terms of an LP, maximize the value of $\crr$, and get our upper bound.

  To demonstrate our idea, let us consider an example where $K = 3$, $M = 1$, and $C = 3$. Our proof can be extended to any value of $C$ and also for $M=2$. Consider the following arrival sequence $\{I_1, I_2\}$ over the course of $T=2$ time periods. 
    \[
        \begin{array}{ll}
            I_1 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2 = \{ 2, 2, 2,\: 3, 3, 3  \}
        \end{array}
    \]
    We can define the following \textit{truncations} of $\{I_1, I_2\}$ which consist of abruptly ending the entire input sequence after a certain type of agent has arrived. For example, $\{I_1^2, I_2^2\}$ represents the truncation of $\{I_1, I_2\}$ where the entire 2-period input suddenly ends after type $2$ agents arrive in the first time period.
    \[\arraycolsep=1.4pt\def\arraystretch{1.5}
        \begin{array}{ll}
            I_1^1 = \{ 1, 1, 1\} \quad                                    & I_2^1 = \{  \}         \\
            I_1^2 = \{ 1, 1, 1, \: 2, 2, 2\} \quad                        & I_2^2 = \{  \}         \\
            I_1^3 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3\} \quad             & I_2^3 = \{  \}         \\
            I_1^4 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2^4 = \{2, 2, 2  \}  \\
        \end{array}
    \]
%  $\{I_1, I_2\}$ is chosen so that we send agents in ascending order of reward over 2 time periods, while making sure all agents can be served within 2 time periods (hence not having partially patient type $1$ in $I_2$). %Such an arrival sequence best captures the core challenge of online resource allocation: the tension between committing to lower reward agents early on and waiting for higher reward agents that might not arrive. 
  
{\color{red} removed a paragraph here.} The truncated arrival sequences $\{I_1^j, I_2^j\}$ for $j \in [4]$ demonstrate that achieving a high CR requires an algorithm, $\alg$, to effectively balance performance across both $\{I_1, I_2\}$ and $\{I_1^j, I_2^j\}$ sequences. Given the overlap in these sequences, any algorithm's response to them is interconnected. For instance, if $\alg$ accepts only type 3 agents in $\{I_1, I_2\}$, maximizing the reward, it would fail to earn any reward on sequence $\{I_1^1, I_2^1\}$, as its actions up to the arrival of type 1 agents would remain unchanged between the two sequences.

  Using the ideas from the example above, we now give a sketch of how the constraints in \ref{3_class_ub} come about. Suppose we are given an algorithm $\alg$ which is $\crr$ competitive. Let $s_{i,t}$, $i \in [3], t \in [2]$, be the number of type $i$ agents that are serviced in period $t$ under $\alg$. Since types $2$ and $3$ are impatient, $s_{i,t}$ also represents the number of type $2$ and $3$ agents that $\alg$ accepts from $I_t$, while for type $1$, $s_{1,1} + s_{1,2}$ is the number of type $1$ agents that $\alg$ accepts from $I_1$. Since $\textsc{opt}_t(\{I_1, I_2\}) = r_3 \cdot C$, to be $\crr$-competitive, we must have   $\textsc{rew}_{\alg, t}(\{I_1, I_2\}) = r_1 \cdot s_{1,t} + r_2 \cdot s_{2,t} + r_3 \cdot s_{3,t} \geq \crr \cdot r_3 \cdot C$, which gives rise to constraint \eqref{align:Ia_revenue}. In addition, we certainly must have $s_{1,t} + s_{2,t} + s_{3,t} \leq C$, as given in \eqref{align:Ia_capacity}. We apply a similar reasoning
  to arrival sequences $\{I_1^1, I_2^1\}, \{I_1^2, I_2^2\}$ and $\{I_1^4, I_2^4\}$, to get the $\crr \cdot r_i \cdot C$ (for $i= 1$ or $2$) reward lower bounds in constraints \eqref{align:Id_revenue}, \eqref{align:Ic_revenue}, \eqref{align:Ic_capacity}, and \eqref{align:Ib_revenue}.\footnote{Note that $\{I^3_1, I^3_2\}$ is actually not useful as it would imply the constraint $r_1 \cdot s_{1,1} + r_2 \cdot s_{2,1} + r_3 \cdot s_{3,1} \geq \crr \cdot r_3 \cdot C$, which was already captured by $\{I_1, I_2\}$.} 
  \Halmos
\end{proof}

We will now state two \po{} algorithms which achieve the $\crr_{up}$ CR from the upper bound, one for the case where $M =1$ and another for $M = 2$. Both of these optimal algorithms require us to first compute the upper bound presented above, get an optimal solution $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in [2]})$ and use some of these values as constants in the feasible polytopes $\feasibleMOne$ for $M = 1$ and $\feasibleMTwo$ for $M = 2$. We will require some properties of this optimal upper bound solution, which are described in Lemmas \ref{lemma:3_class_tight_properties} and \ref{lemma:3_type_additional_properties} in Appendix \ref{sec:lemma:3_class_tight_properties} and \ref{sec:lemma:3_type_additional_properties}. We highlight that the upper bound only characterizes an optimal algorithm's behavior against our constructed worst-case arrival sequences, not any arbitrary arrival sequences over $T$ periods. Nonetheless, we show that how to use the upper bound solution, which represents a particular way of dealing with the worst-case arrival sequence, to construct an optimal algorithm for any arrival sequence.

\subsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 1$}{M=1}}
With $M=1$, type $1$ agents are partially patient while types $2$ and $3$ are impatient. Hence,  our state $\stateB$ contains 4 buckets as shown below:
\[ \begin{array}{r|ccc}
    \text{Type}  & 1               & 2          & 3          \\ \hline
    \text{Row 1} & \bucketij{1}{1} & \bucket{2} & \bucket{3} \\
    \text{Row 2} & \bucketij{1}{2} &            &
  \end{array} \]

Let  $\Delta_{i,j} \defeq r_i - r_j$ and $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ be the optimal solution to the upper bound LP \ref{3_class_ub}. We define our feasible polytope $\feasibleMOne$ as follows
\begin{align} \label{eq:feasibleMOne}  \feasible^{(3,1)} = \left\{ (\fbucketOneOne, \fbucketOneTwo, \fbucketTwo, \fbucketThree) \subset \mathbb{R}_+^4: \quad  \begin{array}{cll}
    \fbucketOneOne + \fbucketTwo + \fbucketThree                       & \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*                           &           \\
    \Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo & \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^* &           \\
    \fbucketOnei                                                       & \leq \optupper_{1,i}^*                                           & i \in [2]\end{array} \right\}\end{align}

\begin{theorem}[Optimality of \textsc{POLYRA} Algorithm with  Feasible  Polytope $\feasibleMOne$]
  \label{thm:opt_alg_M=1} When the number of types $K = 3$ and the number of partially patient types $M = 1$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the \po{} algorithm with feasible polytope $\feasibleMOne$ achieves a CR of $\crr_{up}$, and hence, is optimal. Here, $\crr_{up}$ %{\color{red} I think you are overloading notation $\crr^*$. Did not you use it for the nested algorithms both in the introduction and other parts of the paper. } 
  is the optimal objective value of the LP \ref{3_class_ub}.
\end{theorem}

\textbf{Discussion on Feasible Polytope $\feasibleMOne$.}
Here, we give some intuition about the constraints of $\feasibleMOne$ and why it achieves a CR of $\crr_{up}$. The first constraint, i.e., $\fbucketOneOne + \fbucketTwo + \fbucketThree \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$  simply enforces that we do not allocate more resources in a time period than $s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$ which is bounded above by $C$ as per constraint \eqref{align:Ia_capacity} of the upper bound LP \ref{3_class_ub}. In fact, as we show in property \ref{property:total_is_C} of Lemma \ref{lemma:3_class_tight_properties}, we actually have $\optupper_{1,1}^* + \optupper_{2,1}^* + \optupper_{3,1}^* = C$. The purpose of the second constraint, i.e., $\Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^*$, is to leave enough space in bucket $\bucketThree$ for type $3$ agents, which we do so by enforcing that a linear combination of the number of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ is not too large. Finally, the last constraint, i.e., $\fbucketOnei \leq \optupper_{1,i}^*, i \in [2]$,  simply makes sure that our buckets do not contain too many type $1$ agents in order to leave enough room for the type $2$ and $3$ agents. 

Observe that the feasible polytope $\feasibleMOne$ is not a nested polytope as per Definition \ref{def:nested}. In particular, in order to obtain the optimal CR of $\crr_{up}$, the algorithm has to keep track of a linear combination of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ (i.e., $\Delta_{3,1} \cdot \bucketOneOne + \Delta_{3,2} \cdot \bucketTwo$), rather than simply the sum of the agents assigned to these two buckets (i.e., $ \bucketOneOne + \bucketTwo$).

It can be shown that if we apply our \po{} algorithm with feasible polytope $\feasibleMOne$ to the worst-case arrival sequence from  $\{I_1, I_2\}$ as defined in the proof sketch of Theorem \ref{thm:3_type_upper_bound}, then the behavior of this algorithm will exactly correspond to the optimal solution $\{s_{i,t}^*\}$ in that our algorithm will serve exactly $s_{i,t}^*$ agents of type $i$ in period $t \in [2]$. In this way, our \po{} algorithm \textit{mimics} the upper bound when it encounters the worst-case arrival sequence. In Theorem \ref{thm:opt_alg_M=1}, we show that our algorithm also achieves the optimal CR on any arrival sequence, not just this worst-case arrival sequence. We now describe our polytope construction for three types when $M = 2$.

% We now comment on the proof idea of Theorem \ref{thm:opt_alg_M=1}. First, we note that the polytope $\feasibleMOne$ is consistent as per Lemma \ref{lemma:3_type_valid} which is proven in Section \ref{sec:lemma:3_type_valid}. This is crucial because recall that \po{} algorithms are only well defined when the feasible polytope is consistent. Since our polytope $\feasibleMOne$ contains many terms from the optimal upper bound LP solution (i.e. $\{s_{i,t}^*\}_{i\in[3], t \in [2]}$), we also need to show some properties of this optimal upper bound solution, which are stated in Lemmas \ref{lemma:3_class_tight_properties}, \ref{lemma:3_type_additional_properties} and proven in Sections \ref{sec:lemma:3_class_tight_properties}, \ref{sec:lemma:3_type_additional_properties}. We then show that our proposed \po{} algorithm  obtains the optimal CR against \textit{any} arrival sequence through the following casework. Suppose that for a period $t$, our state after the arrival phase is $\stateB$ and let $\ell \in \{0, 1, 2, 3\}$ be the \textit{highest} type of agent for which all the available space in $\stateB$ for type $\ell$ agents is occupied. In other words, if we were to encounter one more type $\ell$ agent, we would completely reject that agent. We define $\ell = 0$ if $\stateB$ can accommodate some positive amount of another agent of any type and still remain feasible. By our definition of $\ell$, it must be the case that $\stateB$ is able to accommodate an agent of type $k$ for all $k > \ell$. By property (ii) of consistency (Definition \ref{def:consistent}), this implies that our algorithm has not rejected a single agent of type $k$, which means that our algorithm is doing just as well as the optimal solution when it comes to type $k$ agents. For types $k' < \ell$, we may have rejected some agents that the optimal clairvoyant solution accepted, but we show that we have accepted enough such agents of type $k' < \ell$ to be $\crr^*$-competitive.



\subsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 2$}{M=2}}
With $M=2$, types $1,2$ agents are partially patient while type $3$ agents are impatient. Hence, our state $\stateB$ contains 5 buckets as shown below:
\[ \begin{array}{r|ccc}
    \text{Type}   & 1               & 2               & 3          \\ \hline
    \text{Type 1} & \bucketij{1}{1} & \bucketij{2}{1} & \bucket{3} \\
    \text{Type 2} & \bucketij{1}{2} & \bucketij{2}{2} &
  \end{array} \]

To construct the optimal algorithm for three types with two partially patient types, we  first compute the optimal solution $\left(\crr_{up}, \{s_{i,t}^*\}_{i \in [3], t \in [2]} \right)$ from the upper bound LP \ref{3_class_ub} in Theorem \ref{thm:3_type_upper_bound} and use it to construct our polytope $\feasibleMTwo$, which is defined in the following theorem.

\begin{theorem}[Optimal Algorithm for $K=3$ and $M=2$]
  \label{theorem:three_type_M=2}
 When the number of types $K = 3$ and the number of partially patient types $M = 2$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the nested \po{} algorithm with the {nested} polytope $\feasibleMTwo$, defined below, achieves a CR of $\crr_{up}$, and hence, is optimal:
  \begin{equation}\label{feasibleMTwo}
    \feasible^{(3,2)} \defeq \nestedPolyra\left(\frac{1}{2} \cdot (\optupper_{1,1}^* + \optupper_{1,2}^* ), \frac{1}{2} \cdot \left( \optupper_{1,1}^* + \optupper_{1,2}^* + \optupper_{2,1}^* +\optupper_{2,2}^*  \right)  , C \right) \, .
  \end{equation}
  Here, $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ is the optimal solution to the upper bound LP \ref{3_class_ub} and nested polytopes $\nestedPolyra$ are defined in Definition \ref{def:nested}.
\end{theorem}

\textbf{Discussion on the nested polytope $\feasibleMTwo$ and the optimal algorithm.} With two partially patient types (i.e., $M=2$), the optimal algorithm takes the form of a simple nested \po{} algorithm as per Definition \ref{def:nested}. Just like with 1 partially patient type, one can show that if we apply our \po{} algorithm with feasible polytope $\feasibleMTwo$ to the corresponding worst-case arrival sequence for $M = 2$, our \po{} algorithm will exactly serve $s_{i,t}^*$ agents of type $i\in[3]$ in time period $t\in [2]$. In this sense, we again mimic our upper bound solution as a template for making sure our algorithm is $\crr_{up}$-competitive against the worst-case arrival. It turns out that this worst-case arrival sequence is indeed the worst-case as achieving a $\crr_{up}$ CR on it implies a $\crr_{up}$ CR on all arrival sequences. To prove that such a nested polytope achieves the desired CR of $\crr_{up}$, we will apply Theorem \ref{theorem:polyra_nested_performance}, which uses an LP to characterize the CR of \textit{any} nested polytope, including ones for $K > 3$ types.

While $\feasibleMOne$ is not a nested polytope, $\feasibleMTwo$ is. Recall from the earlier discussion that $\feasibleMOne$ is not nested because it has a constraint of the form $c_1 \cdot b_{1,1} + c_2 \cdot b_2 \leq c_3$ where $c_1 \neq c_2$. On the other hand, all of  $\feasibleMTwo$'s constraints involve a linear combination of variables with coefficients all equal to $1$. This can be explained by the following intuition: Both polytopes $\feasibleMOne$ and $\feasibleMTwo$ have constraints which make sure that we do not accept too many type $1$ or $2$ agents, thus making sure enough space is reserved for type $3$ agents. When type $1$ is partially patient and type $2$ is not (i.e. $M = 1$), this constraint is of the form $\Delta_{3,1} \cdot b_{1,1} + \Delta_{3,2} \cdot b_{2}$ where the coefficients $\Delta_{3,1}\neq \Delta_{3,2}$. This is because type $1$ and $2$ differ in their flexibility so our linear combination must weigh the two differently. On the other hand, when both type $1$ and type $2$ are partially patient (i.e $M = 2$), restricting the simple sum of $b_{1,1}$ and $b_{2,1}$ is sufficient.



==> sections/7_-_beyond_3.tex <==
\section{A Near-optimal Nested POLYRA  Algorithm{} for \texorpdfstring{$K > 3$}{K > 3}}
\label{section:beyond_three}
We proceed with the case where $K > 3$. For $K = 2$ and $K = 3$, we were able to find \po{} algorithms with optimal polytopes through presenting a \textit{tight} upper bound on the CR of any non-anticipating algorithm and constructing a \po{} algorithm whose CR matches that upper bound. Recall that to construct our upper bounds for $K = 2$ and $K = 3$, we presented  \textit{worst-case} arrival sequences over $T = 2$ time periods %which looks like the following: 
%\begin{align}
 %   \label{intuitive_worst_case_arrival}
  %  \begin{split}
   %     I_1 &= \{ \underbrace{1, \ldots, 1}_{C}, \underbrace{2, \ldots, 2}_{C}, \ldots, \underbrace{K, \ldots, K}_{C} \} \\
    %    I_2 &= \{ \underbrace{M+1, \ldots, M+1}_{C}, \ldots, \underbrace{K, \ldots, K}_{C} \}
    %\end{split}
%\end{align}
%Such a sequence 
that present a significant challenge for any non-anticipating algorithm  that has  decide how many lower reward agents to accept without knowing if higher reward agents will actually arrive. 
While our worst-case arrival sequences   can certainly be extended to $K > 3$, unfortunately it may not lead to a tight upper bound (i.e. one that is actually attainable by an algorithm). See Appendix \ref{appendix:not_tight_example} for more details. There, we show that slight modifications of our worst-case arrival sequences can lead to a tighter upper bound, implying that our worst-case construction does not lead to an attainable upper bound. 

%For example, depending on the values of $r_1, \ldots, r_K$ and $M$, it may be the case that the following arrival sequence $\{I_1', I_2'\}$ presents a stronger challenge to a non-anticipating algorithm than $\{I_1, I_2\}$ by omitting type $M$ from $I_1$. 
%\begin{align}
 %   \label{alternative_worst_case_arrival}
   % \begin{split}
  %  I_1' &= \{ \underbrace{1, \ldots, 1}_{C}, \ldots, \underbrace{M-1, \ldots, M-1}_{C}, \underbrace{M+1, \ldots, M+1}_{C} \ldots, \underbrace{K, \ldots, K}_{C} \} \\
 %   I_2' &= \{ \underbrace{M+1, \ldots, M+1}_{C}, \ldots, \underbrace{K, \ldots, K}_{C} \}
  %  \end{split}
%\end{align}
%When $r_{M}$ and $r_{M+1}$ are close, type $M$ agents are ``more valuable" to a non-anticipating algorithm than type $M+1$ agents due to the former's flexibility. Therefore, intuitively can make $\{I_1, I_2\}$ more difficult by removing type $M$. In general, an adversary may choose a worst-case arrival sequence with only the first $m \in [M]$ out of $M$ flexible types in period 1, and removing types $m+1, \ldots, M$. This phenomena only occurs for $K > 3$ because with a small number of types, it turns out that removing a type is always makes the arrival sequence easier. A concrete example of this phenomena, as well as other reasons $\{I_1, I_2\}$ may not be the ``worst" can be found in 
%See Appendix \ref{appendix:not_tight_example} for more details.

Given the challenge of constructing tight upper bounds, for $K > 3$, we turn our attention back to nested \po{} algorithms. We show that it is easy to optimize the size of the nests of a nested \po{} algorithm in order to achieve a CR of $\crr^*$ which is the highest CR out of all nested algorithms (Definition \ref{def:optimal_nested_algorithm}). We show theoretically that this optimal nested algorithm has two nice properties: 
\begin{enumerate}
    \item For $M \geq 1$, $\crr^{*} > \crr^{BQ}$, meaning that optimizing our nest sizes results in a better theoretical performance than using our benchmark, the BQ nested polytope (Theorem \ref{theorem:our_alg_beats_bq}). 
    \item $\crr^*$ is at least 80\% of the optimal CR (Theorem \ref{thm:optimality_gap}). We show this by exhibiting an upper bound $\overline{\crr}_{up}$ and showing that $\crr^* \geq 0.8 \cdot \overline{\crr}_{up}$.
\end{enumerate}

% Our main contribution in this section will be to show that the class of nested \po{} algorithms is near-optimal. To do so, we show the construction of an \textit{optimal} nested polytope $\nestedPolyra^*$, which achieves a CR of $\crr^*$ that is the highest out of all nested \po{} algorithms (Definition \ref{def:optimal_nested_algorithm}). Then, we show that $\crr^* \geq 0.8 \cdot \overline{\crr}_{up}$, where $\overline{\crr}_{up}$ is an upper bound on the CR of any non-anticipating algorithm. Thus, we show that the class of nested algorithms is achieves at least 80\% of the optimal CR. 


% \begin{itemize}
%     \item In Section \ref{sec:simple_upper}, we present a different (looser) upper bound $\crr_{\up} \geq \crr^*$, which admits a nice closed-form solution that will be useful for analysis (Theorem \ref{thm:loose_upper_bound}).
%     \item In Section \ref{sec:CR_nested}, we present a formula (in terms of an LP) which computes the CR for any instance of the nested \po{} algorithm (Theorem \ref{theorem:polyra_nested_performance}). 
%     \item In Section \ref{sec:near_optimal}, inspired by the LP from Theorem \ref{theorem:polyra_nested_performance}, we present a specific instance of the nested \po{} algorithm that has a simple closed-form solution for its nest sizes $(\overline{n}_1, \ldots \overline{n}_K)$. We show that this particular instance of the nested polytope attains at least $80\%$ of the optimal CR given by the upper bound from Theorem \ref{thm:loose_upper_bound}. 
% \end{itemize}
%\begin{itemize}[leftmargin=*]
    %\item We characterize the CR of \textit{any} \po{} algorithm with nested polytope through a LP (Theorem \ref{theorem:polyra_nested_performance}). The LP takes as input the nest sizes $(n_i)_{i=1}^K$ and the objective of the LP provides the CR of the \po{} algorithm with polytope $\nestedPolyra(n_1, \ldots, n_K)$. {\color{red} If we move this part up, this section would be easier to navigate. But, I am slightly worried about the proof sketch of theorem 6. It was a bit too technical. If we implement this change, the next two bullet points can be merged.}

  %  \item 
   % We present an optimal choice of nests $(n_i^*)_{i=1}^K$ that obtains the highest CR of $\crr^{*}$ {\color{red} that is what I meant by overloading $\crr^{*}$} for any nested polytope. %Since the LP from Theorem \ref{theorem:polyra_nested_performance} is also linear in $(n_i)_{i=1}^K$, we   treat $(n_i)_{i=1}^K$ as \textit{variables} and solve another LP which provides the optimal choice of nests $(n_i^*)_{i=1}^K$ that obtains the highest CR of $\crr^{*}$ {\color{red} that is what I meant by overloading $\crr^{*}$} for any nested polytope (Definition \ref{def:optimal_nested_algorithm}). {\color{red} I recall we could not solve for the actual optimal nest sizes; we did some relaxation. If yes, please revisit this part. }

   % \item We show that our optimized nested \po{} algorithm is guaranteed to have a CR that is close to optimal, namely that for any non-anticipating algorithm with a CR of $\crr$, we have that $\crr^* \geq 0.8 \cdot \crr$. {\color{red} Instead of that, why don't we say 0.8 of the optimal CR? Do we have notation for the optimal CR? }
%\end{itemize}


% Seeing how a similar upper bound to the ones presented for $K = 2$ and $K = 3$ is not tight for $K > 3$, we turn out attention to presenting a \po{} algorithm with nested polytope which has a CR at least $0.8 \cdot \crr^*$. Here,  $\crr^*$ is the best CR that any algorithm can obtain.  To do this, we will do the following:
% \begin{itemize}
%   \item In Section \ref{sec:simple_upper}, we present a different (looser) upper bound $\crr_{\up} \geq \crr^*$, which admits a nice closed-form solution that will be useful for analysis (Theorem \ref{thm:loose_upper_bound}).
%   \item In Section \ref{sec:CR_nested}, we present a formula (in terms of an LP) which computes the CR for any instance of the nested \po{} algorithm (Theorem \ref{theorem:polyra_nested_performance}).
%   \item In Section \ref{sec:near_optimal}, inspired by the LP from Theorem \ref{theorem:polyra_nested_performance}, we present a specific instance of the nested \po{} algorithm that has a simple closed-form solution for its nest sizes $(\overline{n}_1, \ldots \overline{n}_K)$. We show that this particular instance of the nested polytope attains at least $80\%$ of the optimal CR given by the upper bound from Theorem \ref{thm:loose_upper_bound}.
% \end{itemize}




\subsection{ Optimal Nested POLYRA Algorithms and Their Performance }
%{\color{red} made this a subsection assuming you'll move the previous part up}
While the LP from Theorem \ref{theorem:polyra_nested_performance} can be used to compute the CR of any nested \po{} algorithm, we notice that this LP is also linear in the variables $\deltan_i$ (and hence also in $n_i$). Therefore, we can solve the following LP to find the nested \po{} that results in the best CR across all nested \po{} algorithms. 

\begin{definition}[Optimized Nested POLYRA Algorithms] \label{def:optimal_nest}
Consider the following LP
    \label{def:optimal_nested_algorithm}
    \begin{align*}
        \crr^* \defeq \max_{\Gamma, \{s_i^j\}_{j \in [K], i \in [j]}, \{\deltan_i\}_{i \in [K]}} \quad & \crr \\
        \text{s.t.} \quad &  \eqref{nested_lp_revenue_target}, \eqref{nested_lp_capacity}, \eqref{nested_lp_j_le_M}, \eqref{nested_lp_j_ge_M}, \eqref{eq:positive}\,.
    \end{align*}
We define $\crr^*$ to be the optimal value of the above LP and $n_k^* \defeq \sum_{i=1}^k \deltan_i^*$ where $(\deltan_i^*)_{i=1}^K$ are the optimal solution for the variables $(\deltan_i)_{i=1}^K$. We define the nested polytope with nests $(n_k^*)_{k=1}^K$ to be the optimal nested polytope $\nestedPolyra^*$:
\begin{equation}
    \label{eq:nested_polyra_definition}
    \nestedPolyra^* \defeq \nestedPolyra(n_1^*, \ldots, n_K^*)\,.
\end{equation}
The \po{} algorithm using $\nestedPolyra^*$ is called the \textit{optimized nested \po{} algorithm} and by our construction, achieves a CR of $\crr^*$.
\end{definition} 

{\color{black}The following theorem shows that the CR of our optimized nested \po{} algorithm  (i.e., $\crr^*$) is strictly greater than the CR of the BQ nested \po{} algorithm, denoted by $\crr^{BQ}$, justifying the need to optimize the nest sizes. See also our numerical studies for a comparison of  our optimized nested \po{} algorithm and the BQ nested \po{} algorithm.}  
{
\color{black}
\begin{theorem}[Optimized Nested POLYRA Alg. vs. the BQ Nested POLYRA Alg.]
    \label{theorem:our_alg_beats_bq}
    For any $K$ types of agents with rewards $r_1 < \ldots < r_K$ with $M \geq 1$ partially patient types, we have that $\crr^* > \crr^{BQ}$, where $\crr^* $, defined in Definition \ref{def:optimal_nested_algorithm}, is the CR of our optimized nested \po{} algorithm and $\crr^{BQ}$, defined in equation \eqref{equation:bq_cr}, is the CR of the BQ nested \po{} algorithm. 
\end{theorem}
%The intuition behind this result is as follows. 
The proof of this statement can be found in Appendix \ref{appendix:nested_vs_bq}. In the proof, we show that 
when $M = 0$ (i.e., there are no partially patient agents), $\crr^*$ obtained by solving the LP in Definition \ref{def:optimal_nested_algorithm} is the same as $\crr^{BQ}$. However, when $M \geq 1$, the LP we solve in Definition \ref{def:optimal_nested_algorithm}  accounts for the $M$ partially patient types,  leading to  a strictly  higher objective value (CR). This demonstrates the fact that the BQ nested \po{} algorithm is optimized for the $M = 0$ case and our nested polytope can do strictly better than for $M \geq 1$ (i.e. when there are partially patient agents). 
}

In addition to being strictly better than the CR of the BQ nested \po{} algorithm, the CR of our optimized nested \po{} algorithm is also guaranteed to be close to optimal, i.e., the best possible CR.

\begin{theorem}[CR of our Optimized POLYRA Alg.]
\label{theorem:main_optimality_gap}
For any rewards $r_1 < \ldots < r_K$ and flexible types $M \in [K-1]$, let $\crr^*$ be the CR of the optimized nested \po{} algorithm (per Definition \ref{def:optimal_nested_algorithm}). Then, for any non-anticipating deterministic algorithm with a CR  of $\crr$, it is the case that $\crr^* \geq 0.8 \cdot \crr\,$.
\end{theorem}
%{\color{red} shortened this}

{\color{black}
\noindent In Appendix \ref{sec:theorem:main_optimality_gap}, we confirm the validity of this statement by following these steps:

\begin{enumerate}
    \item 
In Lemma \ref{thm:loose_upper_bound}, we introduce an approximate closed-form upper bound, denoted as $\overline{\crr}_{up}$, for the CR of any deterministic non-anticipating algorithm.
    \item Subsequently, we provide a specific example of a nested polytope that has nested sizes represented by $(\overline{\deltan_i})_{i=1}^K$. While this polytope may not necessarily be the optimal nested configuration, it does achieve a CR denoted as $\crr_{nest}$. It's important to note that $\crr_{nest}$ satisfies the condition $\crr_{nest} \leq \crr^*$ as defined in Definition \ref{lem:bar_gamma}.
    \item Following that, we demonstrate that $\crr_{nest}$ has a lower bound of at least 80\% of $\overline{\crr}_{up}$ (as shown in Lemma \ref{thm:optimality_gap}). This finding also implies that $\crr^*$ (the CR of the optimized nested \po{} algorithm) cannot be less than 80\% of $\overline{\crr}_{up}$, thereby providing proof for Theorem \ref{theorem:main_optimality_gap}.
\end{enumerate}
}

==> sections/8_-_numerical_studies.tex <==

{\color{black}
\section{Numerical Studies}
\label{sec:numerical_studies} 
In this section, we complement our theoretical results with numerical studies. We evaluate our optimized nested \po{} algorithms (as defined in Theorem \ref{theorem:polyra_nested_performance}) in real-world inspired settings where the arrival sequence is no longer adversarial and compare its performance with the BQ nested \po{} algorithm (Definition \ref{def:bq_nest}). We evaluate the performance of the two algorithms not only using our feature-augmented CR definition, but also under a more traditional CR definition. 

\subsection{Setup.} 
We fix the number of types at $K = 5$, the total number of resources in each time period $C=100$, the number of time periods is $T= 10$, and the number of partially patient types $M\in \{0, 1, 2, 3, 4\}$. 

\textbf{Agent Rewards.} We fix $r_1 = 1$. For each $i \in \{2, 3, 4, 5\}$, we draw $r_i \mid r_{i-1} \sim \left(r_{i-1} \cdot \text{Unif}(1, 3)\right)$. In other words, the reward of each agent type ranges uniformly from 1 to 3 times that of the previous agent type, in increasing order. 

\textbf{Arrival Sequence Generation.} 
First, we draw a \( K \)-dimensional probability distribution \( p \) from a Dirichlet distribution with uniform parameters, i.e., \( p \sim \text{Dirichlet}(1, \ldots, 1) \). This distribution represents the likelihood of the arrival of each of the \( K \) types.

For every period \( t \) ranging from 1 to \( T \), we determine the total number of arrivals, denoted by \( |I_t| \). This number is drawn from a distribution given by \(\max(0, \lfloor \text{Norm}(1.1 \cdot C, \sigma \cdot C)\rfloor) \), where ``Norm" refers to the Gaussian distribution. The mean of this distribution suggests that the demand (total number of arriving agents) is approximately 10\% higher than the available capacity \( C \) and the parameter \( \sigma \) controls the variability of demand in each period.

Each individual agent that arrives in period \( t \) is represented in sequence as \( z_{t, 1}, \ldots, z_{t, |I_t|} \). The type of every arriving agent is determined independently based on the categorical distribution derived from \( p \). To be precise, the probability that an agent \( z_{t,n} \) is of type \( k \) is given by \( P(z_{t,n} = k) = p_k \), where we recall that \( p \sim \text{Dirichlet}(1, \ldots, 1) \).

 In our experiments, we explore the effects of varying both \( M \) and \( \sigma \). A single instance of our simulation study involves drawing the agent rewards $(r_1, \ldots, r_5)$ and an arrival sequence $\{I_t\}_{t=1}^T$. We run our optimized nested algorithm (notated by $\alg^*$) and the BQ nested \po{} algorithm (denoted by $\alg^{BQ}$) on this arrival sequence and compute the following metrics.
\begin{itemize}[leftmargin=*]
    \item \textbf{Theoretical FA-CR Lower Bound}. Let $\crr^*$ and $\crr^{BQ}$ be the theoretical lower bounds on the feature-augmented CR of $\alg^*$ and $\alg^{BQ}$ respectively. Note that this metric is calculated purely based on $r_1, \ldots, r_5$ and the number of flexible types $M\in \{0, 1, 2, 3, 4\}$ irrespective of the actual arrival sequence. 
    \item \textbf{Empirical FA-CR}. For each arrival sequence, we can compute the empirical feature-augmented CR of that instance by measuring the worst-case ratio between an algorithm's reward and the optimal reward (without flexibility) over each of the $T$ periods. For each of the two algorithms $\alg \in \{\alg^*, \alg^{BQ}\}$, we define:
    \begin{align*}
        \textsc{fa-cr}_{\alg}(\{I_t\}_{t=1}^T) \defeq \min_{\tau \in [T]} \frac{\text{Rew}_{\alg, \tau}(\{I_t\}_{t=1}^T)}{\textsc{opt}(I_t)}\,.
    \end{align*}
    Recall that $\textsc{opt}(I_t)$ is the optimal offline reward from the agents arriving in period $t$ without access to flexibility for types $1, 2, \ldots, M$. 

    \item \textbf{Empirical TR-CR}. We introduce a more conventional CR notion termed the empirical total reward or traditional (TR) CR. It's defined as the ratio between the total reward our algorithm achieves over the $T$ periods and the optimal total reward of an algorithm that knows the arrival sequence in advance and \textbf{has the ability to utilize flexibility}. For any arrival sequence ${I_t}$, let $\textsc{opt-total}(\{I_t\}_{t=1}^T)$ represent the optimal total reward in hindsight achievable from $\{I_t\}_{t=1}^T$, where flexibility of types $1, 2, \ldots, M$ is available. There are several methods to determine $\textsc{opt-total}(\{I_t\}_{t=1}^T)$; one of the most straightforward is via the following mathematical  program.


     Given an arrival sequence $\{I_t\}_{t=1}^T$, let $n_{t, k}$ denote the count of type $k$ arrivals in $I_t$. We employ decision variables: $a_{t,k}$ is the count of type $k$ agents accepted from $I_t$, and $s_{t,k}$ represents the subset of $a_{t,k}$ designated for service in period $t$. The goal is to maximize the reward from all accepted agents. The formulation is detailed below.
    \begin{align}
        \textsc{opt-total}(\{I_t\}_{t=1}^T) &= \max_{\{s_{t,k}, a_{t,k}\}_{t \in [T], i \in [K]}} \sum_{t=1}^T \sum_{k=1}^K r_k \cdot a_{t,k} \nonumber \\
        \text{s.t.} \quad & \sum_{k=1}^K s_{t, k} + \sum_{k=1}^M (a_{t-1, k} - s_{t-1, k}) \leq C \label{opttotal:capacity} &t \in [T] \\
        &  a_{t,k} \leq n_{t,k} & t \in [T], k \in [K] \label{opttotal:accept} \\
        &  s_{t,k} = a_{t,k} & t \in [T], k \in \{M+1, \ldots, K\} \label{opttotal:serve} \\ 
        & s_{t, k}, a_{t,k} \in \mathbb{Z} \nonumber
    \end{align}
    For notational convenience, we define $a_{-1, k} = s_{-1, k} = 0$ for all $k \in [K]$. Constraint \eqref{opttotal:capacity} is the capacity constraint, where the first summation are the agents from $I_t$ we serve, while the second summation represent the unserved flexible agents from period $t-1$. Constraints \eqref{opttotal:accept} simply ensures that we do not accept more agents than arrive. Constraint \eqref{opttotal:serve} ensures that all inflexible agents are served in the current period. Note that although some of the variables are redundant, we believe this notation is the easiest to understand. For each of the two algorithms $\alg \in \{\alg^*, \alg^{BQ}\}$, we define the Total Reward CR (\textsc{tr-cr}):
    \begin{align*}
        \textsc{tr-cr}_{\alg}(\{I_t\}_{t=1}^T) \defeq  \frac{\sum_{\tau \in [T]} \text{Rew}_{\alg, \tau}(\{I_t\}_{t=1}^T)}{\textsc{opt-total}(\{I_t\}_{t=1}^T)}\,.
    \end{align*}
\end{itemize}

\captionsetup[sub]{font=footnotesize,justification=centering}
\captionsetup[subfigure]{font=scriptsize,labelfont=scriptsize, justification=centering}

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[c]{0.4\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{trcr.pdf}
        \subcaption{Average \textsc{tr-cr} by $M$}
        \label{sim:by_M_left}
    \end{subfigure}
    \begin{subfigure}[c]{0.4\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{facr.pdf}
        \subcaption{Average \textsc{fa-cr} by $M$}
        \label{sim:by_M_right}
    \end{subfigure}
    \begin{subfigure}[c]{0.15\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{legend.png}
    \end{subfigure}
    \vspace{0.5em}
    \caption{Average 
    TR-CR and FA-CR across 250 problem instances  with  $M\in\{0, 1, \ldots, 4\}$ and  $\sigma \in \{0.1, 0.5, 1.0\}$. For FA-CR, the theoretical lower bounds $\crr^*$ and $\crr^{BQ}$ are also shown.}
    \label{sim:by_M}
\end{figure} 

\begin{figure}[hbt!]
    \begin{subfigure}[c]{0.45\textwidth}
    \footnotesize
    \centering
   \begin{tabular}{l|ccc}
      $M$ & $\sigma = 0.1$ & $\sigma=0.5$ & $\sigma=1.0$  \\ \hline
        $0$ & (1.00, 1.00)   & (1.00, 1.00) & (1.00, 1.00) \\
        $1$ & (1.01, 0.98)   & (1.02, 1.01) & (1.02, 1.08) \\
        $2$ & (1.02, 1.02)   & (1.03, 1.08) & (1.05, 1.09) \\
        $3$ & (1.04, 1.04)   & (1.05, 1.09) & (1.06, 1.13) \\
        $4$ & (1.04, 1.08)   & (1.04, 1.08) & (1.05, 1.19)
    \end{tabular}
    \subcaption{\textsc{tr-cr}}
    \label{sim:improvement_left}
     \end{subfigure}
    \begin{subfigure}[c]{0.45\textwidth}
    \centering
    \footnotesize
   \begin{tabular}{l|ccc}
      $M$ & $\sigma = 0.1$ & $\sigma=0.5$ & $\sigma=1.0$  \\ \hline
        $0$ & (1.00, 1.00)   & (1.00, 1.00) & (1.00, 1.00) \\
        $1$ & (0.99, 0.88)   & (1.03, 0.97) & (1.04, 1.09) \\
        $2$ & (1.01, 0.97)   & (1.08, 1.11) & (1.11, 1.21) \\
        $3$ & (1.05, 1.24)   & (1.13, 1.22) & (1.17, 1.29) \\
        $4$ & (1.13, 1.37)   & (1.16, 1.36) & (1.19, 1.45)
    \end{tabular}
    \vspace{0.5em}
    \subcaption{\textsc{fa-cr}}
    \label{sim:improvement_right}

     \end{subfigure}
     \caption{Ratio of average and minimum (worst) empirical CR between $\alg^*$ and $\alg^{BQ}$. For each algorithm $\alg^*$ and $\alg^{BQ}$ we compute its average empirical CR and minimum empirical CR across the 250 instances. In each tuple above, the first value is the ratio of these two average CRs and the second value is the ratio of these two minimum (i.e. worst) CRs. Both TR-CR and FA-CR are shown as labeled. }
    \label{sim:improvement}
\end{figure}

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}[c]{0.47\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{trcr_boxplot.pdf}
        \subcaption{Distribution of \textsc{tr-cr}}
    \end{subfigure}
    \begin{subfigure}[c]{0.47\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{facr_boxplot.pdf}
        \subcaption{Distribution of \textsc{fa-cr}}
    \end{subfigure}
    \vspace{0.5em}
    \caption{Boxplot of the CRs obtained by $\alg^*$ in {\color{black} blue} and $\alg^{BQ}$ in {\color{red}red} across the 250 problem instances. The plot shows three values of $(M, \sigma)$, namely $(4, 1.0), (3, 0.5)$ and $(1, 0.1)$.}
    \label{sim:cdf}
\end{figure} 
 
\subsection{Results}
For each combination of 
$M \in \{0, 1, 2, 3, 4\}$ and $\sigma \in \{0.1, 0.5, 1.0\}$, we generated 250 arrival sequences. We then calculated three key metrics for both $\alg^{*}$ and $\alg^{BQ}$: the theoretical FA-CR, empirical FA-CR, and empirical TR-CR. For all figures in this section, the left-side corresponds to TR-CR while the right-side is FA-CR. The average values for these metrics are depicted in Figure \ref{sim:by_M}. Figure \ref{sim:improvement} 
provides a direct performance comparison between $\alg^*$ and $\alg^{BQ}$.  
For each $M, \sigma$ pair, the first value in the tuple is the ratio of the average CR (either FA-CR or TR-CR) of $\alg^*$ versus the average CR of $\alg^{BQ}$ over the 250 instances, which we refer to as the \emph{ratio of average CRs}. The second value denotes the ratio of the minimum (i.e. worst-performing) CR of $\alg^*$ to that of $\alg^{BQ}$ across the same instances, termed the \emph{ratio of worst CRs}. Finally, Figure \ref{sim:cdf} shows a box-plot of the CRs from $\alg^*$ and $\alg^{BQ}$ for a select number of $(M, \sigma)$ combinations. We highlight some of the insights from these figures below. 

%\textbf{Value of Flexibility.} Figure \ref{sim:by_M_left} emphasizes the considerable benefits of introducing flexibility. Recall that for $M=0$, there's a lack of flexibility. By integrating flexibility, the TR-CR under $\alg^*$ displays marked improvements, ranging from 0.8\% to 12\%, dictated by the number of flexible agents \(M\) and variations in the arrival sequence $\sigma$. Crucially, as \(M\)  and $\sigma$ increase, these enhancements are even more pronounced. We will comment on this further.

\textbf{The relation between CRs and the number of flexible types.} Figures \ref{sim:by_M_left} and \ref{sim:by_M_right} demonstrate that as the number of flexible agent types $M$ rises, both TR-CR and FA-CR increase linearly. Contrary to the notion that ``a little bit of flexibility goes a long way", our findings suggest performance improvements are proportional to increased flexibility. 
Notably, Figure \ref{sim:by_M_left} highlights the substantial gains from introducing flexibility. For instance, in Figure \ref{sim:by_M_left}, compared to $M = 0$ (without flexibility), the TR-CR under $\alg^*$ shows improvements between 2.5\% to 12\% for $\sigma=1$ and $0.8\%$ to $5.1\%$ for $\sigma=0.1$ as $M$ increases from $1$ to $4$.

Conversely, the TR-CR and FA-CR of $\alg^{BQ}$—an algorithm with nest sizes that remain indifferent to $M$—plateau as $M$ grows. This underscores the notion that merely having flexible agents is insufficient; we must also design algorithms that adeptly harness this flexibility.





% \textbf{Value of Flexibility. } Figure \ref{sim:by_M_left} emphasizes the considerable benefits of our algorithm $\mathcal{A}^*$ introducing flexibility. The average TR-CR and FA-CR increase with $M$ by up to 

% \textbf{The }
% Furthermore, by comparing $\alg^*$ to $\alg^{BQ}$, we highlight the need to 





%\textbf{Even though $\alg^$ was designed for FA-CR, it also performs well in TR-CR.} We set up $\alg^$'s nest sizes using a linear program focused on the best FA-CR (see Definition \ref{def:optimal_nest}). The fact that its TR-CR also shows improvement over $\alg^{BQ}$, as displayed in Figure \ref{sim:by_M_left}, underlines the value of adjusting nest sizes based on the number of flexible types, a tactic we used in developing $\alg^*$.

%\textbf{Even though $\alg^*$ was designed for FA-CR, it also performs well in TR-CR (both average and worst-case).} While $\alg^*$ was designed with FA-CR in mind, it exhibits strong performance across both the average and worst-case scenarios in TR-CR and FA-CR. Our design of $\alg^*$'s nest sizes was driven by a linear program aiming at optimizing FA-CR (see Definition \ref{def:optimal_nest}). However, its broad-spectrum performance as evidenced in Figure \ref{sim:by_M_left} underscores its superior TR-CR relative to $\alg^{BQ}$.
 %The fact that its TR-CR also shows improvement over $\alg^{BQ}$, as displayed in Figure \ref{sim:by_M_left}, underlines the value of adjusting nest sizes based on the number of flexible types, a tactic we used in developing $\alg^*$. Further, from the data in Figure \ref{sim:improvement}, we observe that $\alg^*$ also outperforms $\alg^{BQ}$ in both average and worst-case scenarios across TR-CR and FA-CR metrics.
 %For instance, considering the average TR-CR performance with 
%$M=3$ and $\sigma=0.5$, the ratio stands at $1.05$, showcasing that $\alg^*$ delivers better results on average compared to $\alg^{BQ}$. Delving into worst-case scenarios, like the FA-CR with $M=1$ and $\sigma =1$, the ratio reaches a significant 1.45, accentuating the superior resilience and performance of $\alg^*$.

\textbf{\( \alg^* \) excels in TR-CR, even though it was primarily designed for FA-CR.}
Although \( \alg^{*} \) was designed to optimize nest sizes for the FA-CR (Definition \ref{def:optimal_nest}), it demonstrates impressive performance in both average and worst-case scenarios for TR-CR. This observation is evident in Figure \ref{sim:improvement_left}, where the ratio of averages and the worst-case ratio for TR-CRs are almost always greater than 1. By optimizing for the FA-CR, \( \alg^* \) determines nest sizes that more effectively exploit flexibility, irrespective of the specific performance metric, be it FA-CR or TR-CR.

%Recall that we designed the nest sizes of $\alg^*$ using an LP that gives the optimal FA-CR (see Definition \ref{def:optimal_nest}).
%This design choice is evident from the both the ratio of average CR's and the ratio of worst CR's almost always exceeding 1 in Figure \ref{sim:improvement}. 
%One key advantage of $\alg^*$ is its ability to adjust nest sizes based on the number of flexible types. This advantage is clear in Figure \ref{sim:improvement}, where $\alg^*$ almost always outperforms $\alg^{BQ}$ in both ratio of average and worst CRs across both CR metrics.
%For context: when $M = 3$ and $\sigma = 0.5$, the average empirical TR-CR of $\alg^*$ is $1.05$ times that of $\alg^{BQ}$. Similarly, the worst-case empirical TR-CR of $\alg^*$ is $1.09$ times that of $\alg^{BQ}$. 
%This design choice becomes evident when we look at Figure \ref{sim:by_M_left}, where $\alg^*$ consistently achieves better TR-CR results than $\alg^{BQ}$.

\textbf{The performance disparity between \( \alg^* \) and \( \alg^{BQ} \) widens with greater volatility in the arrival sequence.}
As depicted in Figure \ref{sim:improvement}, the performance advantage of \( \alg^* \) over \( \alg^{BQ} \) becomes more pronounced as the volatility parameter \( \sigma \) increases for both the TR-CR and FA-CR metrics. Specifically, for any fixed \( M > 0 \), the advantage of \( \alg^* \) over \( \alg^{BQ} \) increases with \( \sigma \), by up to 19\% in average CR. Even more striking, the ratio of worst CRs surges by up to 45\% under the same conditions. This trend underscores that as the unpredictability of the arrival sequences heightens, the capacity to adapt flexibly becomes increasingly vital. Our theoretical findings bolster this observation, emphasizing that flexibility in algorithms offers enhanced resilience against uncertainties in agent arrivals. Furthermore, while exploiting flexibility improves the average case by a significant margin, it benefits the worst case by an even greater degree.


\textbf{The CR distributions for \( \alg^* \) appear to stochastically dominate those of \( \alg^{BQ} \).}
To provide a holistic view, Figure \ref{sim:cdf} presents boxplots for both FA-CR and TR-CR across three chosen configurations: \( (M=4, \sigma=1) \), \( (M=3, \sigma=0.5) \), and \( (M=1, \sigma=0.1) \). The distribution statistics, including the 1st quartile, median, and 3rd quartile, consistently indicate superior performance by \( \alg^* \) over \( \alg^{BQ} \). This trend is further substantiated in Figure \ref{sim:cdf} within Appendix \ref{appendix:K=10}, where the empirical cumulative distribution function (CDF) is plotted for the aforementioned \( (M, \sigma) \) combinations across 250 instances.

}


==> sections/two_and_three_types_together.tex <==
\section{Optimal POLYRA Algorithm with Two or Three Types}

In this section, we show that a \po{} algorithm is able to achieve the optimal CR for two and three types. For two types, the polytope follows the nested structure described in Section \ref{sec:polyra}, but unfortunately, this is not necessarily the case for three types. 


\subsection{Optimal POLYRA Algorithm with Two Types}
\label{section:two_type}
Consider a special case of our model for $K = 2$ types with rewards $r_1 < r_2$, where type $1$ is partially patient and type $2$ is impatient. It turns out that nested \po{} algorithms  are optimal here. We show in the following theorem that choosing the right nest sizes achieves the optimal CR. We then provide some intuition for why choosing the BQ nested polytope (per Definition \ref{def:bq_nest}) provides a sub-optimal algorithm.

\begin{theorem}[Optimal Algorithm with Two Types] 
\label{thm:opt_2}
    When the number of types $K = 2$ and the number of partially patient types $M = 1$ with rewards $r_1 < r_2$ and per-period capacity $C$. Then, the nested \po{} algorithm with the nested   polytope $\feasible^{(2,1)}$ achieves a CR of $\frac{2}{3 - r_1 / r_2}$, where
    \begin{equation} 
    \label{eq:feasible_two_type}
    \feasible^{(2, 1)} = \nestedPolyra \left( \frac{C}{3 - r_1 / r_2}, C \right).
    \end{equation}
    %  {\color{red} deterministic or randomized? At least, let's make this clear in a footnote.}
    Furthermore, no {\color{black} deterministic} online algorithm can achieve a higher CR than $\frac{2}{3 - r_1 / r_2}$ hence proving that our \po{} algorithm with polytope $\feasible^{(2,1)}$ is optimal.
\end{theorem}

To get an intuition for this polytope $\feasible^{(2,1)}$, it is useful to compare it to $\nestedPolyra^{BQ}$, which is defined as follows.  
\begin{align} \label{eq:two_type_bq}
\nestedPolyra^{BQ} = \nestedPolyra \left( \frac{C}{2 - r_1 / r_2}, C \right).
\end{align}
Based on Theorem \ref{theorem:bq_polytope_same_cr}, the above polytope achieves a CR of $\frac{1}{2 - r_1/r_2}$, which is strictly smaller than $\frac{2}{3 - r_1 / r_2}$ from Theorem \ref{thm:opt_2}. Notice that the only difference between $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ is the choice of the first nest size $n_1$: $\frac{C}{3 - r_1/r_2}$ versus $\frac{C}{2 - r_1/r_2}$.  We now present an example to show how two polytopes' performance differ, as well as, a proof sketch for why our polytope $\feasible^{(2,1)}$ is optimal.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{nested_example_diagram.png} 
    \vspace{0.5em}
    \caption{Comparing $\nestedPolyra^{BQ}$ (left) and $\feasible^{(2,1)}$ (right) in the special case of $(K, M) = (2, 1)$, $r_1 = 1, r_2 = 1000$ and $C = 6$. In this case, $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ and $ \feasible^{(2,1)} = \nestedPolyra(2, 6)$.
    %$n_1 = 3$ for BQ while $n_1 = 2$ for our optimal polytope. 
    The first row represents the 6 capacity in the current time period, while the second row is for the next period. The 6 capacity in the top row is divided into light blue (can be assigned to either type 1 or type 2) and red (can be assigned to type 2 only). Type 1 agents are also allowed to occupy the striped blue region in the second row (but type 2 agents are not at the moment since type 2 agents are impatient). %Out of the 6 capacity for the next period, allow type 1 agents (who are partially patient) to take up $n_1$ out of 6 units. Such capacity cannot be used by type 2 agents in the current period because type 2 agents are impatient.
    %{\color{red} it seems that the dark black color in the caption is not the same as that in the second row.} They actually are (I checked). 
    }
    \label{fig:nested_comparison}
\end{figure}

\begin{example} 
\label{example:two_types}
Consider a concrete example with $r_1 = 1, r_2 = 1000$, $T = 1$, and $C = 6$. Here, $r_2$ is significantly larger than $r_1$, approaching infinity in the limit. In this scenario, our nested polytope $\feasible^{(2,1)}$ (from equation \eqref{eq:feasible_two_type}) and the BQ nested polytope (from equation \eqref{eq:two_type_bq}) become, asymptotically as $r_2 / r_1 \to \infty$, $\nestedPolyra(2, 6)$ and $\nestedPolyra(3, 6)$ respectively (see Figure \ref{fig:nested_comparison}). Our optimal polytope reserves $C-n_1 = 6-2 = 4$ units of capacity for higher reward agents in each period, while the BQ polytope only reserves $C- n_1 = 6 - 3 = 3$ units. Now, let's examine how the \po{} algorithms with feasible polytope $\feasible^{(2,1)}$ and $\nestedPolyra^{BQ}$ react to a simple arrival sequence $I_1$, which includes a dummy second period with no agent arrivals: $I_1 = \{1, 1, 1, 1, 1, 1, 2, 2, 2, 2, 2, 2\}, I_2 = \{\}$.

Our \po{} algorithm with polytope $\feasible^{(2,1)} = \nestedPolyra(2, 6)$ accepts $2\cdot n_1 = 4$ out of $6$ type $1$ agents from $I_1$ and then accepts $C- n_1 = 4$ out of 6 type $2$ agents. It then provides service to 2 type $1$ agents and 4 type $2$ agents for a total reward of approximately $4000$, achieving a $2/3$ approximation to the optimal reward of $6000$ in $I_1$.

The BQ nested \po{} algorithm with polytope $\nestedPolyra^{BQ} = \nestedPolyra(3, 6)$ accepts $2\cdot n_1 = 6$ type $1$ agents and 3 type $2$ agents from $I_1$, and provides service to 3 type $1$ agents and $C- n_1 = 3$ type $2$ agents for a total reward of approximately $3000$, achieving a $1/2$ approximation to the optimal reward in $I_1$.

The BQ nested \po{} algorithm services only 3 type $2$ agents, while our algorithm services 4. This difference arises because the BQ nested \po{} algorithm accepts too many type $1$ agents (6 instead of 4 in our algorithm). It is essential for any good algorithm to accept some type $1$ agents because a non-anticipating algorithm cannot predict if type $2$ agents will arrive after observing the first 6 type $1$ agents. However, the BQ nested \po{} algorithm is overly pessimistic about the arrival of type $2$ agents, accepting too many type $1$ agents. This leads to poor performance if type $2$ agents do arrive. In contrast, our nested \po{} algorithm achieves good performance in both cases, resulting in better worst-case performance.

{\color{black}We remark that while achieving an optimal CR does not guarantee our algorithm outperforms the BQ algorithm in \textit{every} instance, our numerical studies in Section \ref{sec:numerical_studies} demonstrate that our optimized nested algorithm surpasses the BQ benchmark algorithm in more realistic input sequences that are not stylized under both feature-augmented and traditional notions of CRs.}
\end{example}

\subsection{Optimal POLYRA Algorithm with Three Types}
\iffalse
{\color{black}
For $K = 3$, while \po{} algorithms are still optimal, the structure of the optimal polytope is not necessarily nested. 

For the case $K = 3$ and $M = 1$, the optimal polytope is of the following form: 
\begin{align} \label{eq:non_nested_example}  \feasible^{(3,1)} = \left\{ (\fbucketOneOne, \fbucketOneTwo, \fbucketTwo, \fbucketThree) \subset \mathbb{R}_+^4: \quad  \begin{array}{cll}
    \fbucketOneOne + \fbucketTwo + \fbucketThree                       & \leq C                           &           \\
    (r_3 - r_1) \cdot \fbucketOneOne + (r_3 - r_2) \cdot \fbucketTwo & \leq n_2 &           \\
    \fbucketOnei                                                       & \leq n_1                                         & i \in [2]\end{array} \right\}
\end{align}
where $n_1$ and $n_2$ depend on the specific values of $r_1, r_2, r_3$. 

\textbf{Discussion on Why This Optimal Polytope is not Nested}

\textbf{Brief Discussion on how we constructed it}

\textbf{Discuss why in general it is difficult to characterize the optimal polytope.}



}
\fi










%\subsection{Optimal Algorithm with Three Types}
\label{section:three_type}
In this section, we consider a special case with $K = 3$ and $M\in \{1, 2\}$. Our main result in this section is an explicit characterization of two polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$ (defined in equations \eqref{eq:feasibleMOne} and \eqref{feasibleMTwo}) which give optimal \po{} algorithms for the case when $M = 1$ and $M = 2$, respectively. We present an innovative technique where we first construct an upper bound on the CR of any online algorithm through an LP, and then use its optimal solution values to build our polytopes $\feasible^{(3, 1)}$ and $\feasible^{(3, 2)}$.

\subsubsection{An Upper Bound for Three Types}

In order to prove the optimality of our algorithms for $K = 3$, we first need to establish an upper bound. To do so, for each of $M = 1$ and $M = 2$, we construct  \textit{worst-case arrival sequences}, which best exemplify the main challenge that an online algorithm must face: the trade-off between a moderate reward now versus waiting for a potentially higher future reward. We then argue that to obtain a CR of $\crr$ on these worst-case arrival sequences, the behavior of non-anticipating algorithm needs to satisfy certain conditions. These conditions  lead to  an LP construction, where  the objective of the LP maximizes the CR (i.e., $\crr $ in the LP) and the constraints enforce the aforementioned conditions.

\begin{theorem}[Upper Bound on the CR with Three Types]
  \label{thm:3_type_upper_bound}
  Suppose that there are three types with $M\in \{1, 2\}$ and rewards $r_1 < r_2 < r_3$. Then, the CR of any non-anticipating algorithm $\mathcal {A}$, i.e.,  $\text{CR}_{\mathcal A}$, is at most the optimal value of the following LP, denoted by $\crr_{up}$. %{\color{red}changed the notation here.}
  \begin{align}
   \crr_{up} \defeq \max_{\crr, \{\optupper_{i,t}\}_{i\in[3], t\in[2]}} \quad && \crr & \nonumber \\
    \text{s.t.} \quad &   & \optOnet + \optTwot + \optupper_{3,t} & \leq C                                                                         & t \in [2] \label{align:Ia_capacity} \\
                      &   & \crr \cdot r_3 \cdot C                & \leq \optOnet \cdot r_1 + \optTwot \cdot r_2 + \optupper_{3,t} \cdot r_3       & t \in [2] \label{align:Ia_revenue}  \\
    \lplabel[3_class_ub]{\textsc{(upper3)}}  && \crr \cdot r_1 \cdot C &\leq(\optOneOne + \optOneTwo) \cdot r_1 \label{align:Id_revenue} \\
    && \crr \cdot r_2 \cdot C &\leq \left(C - \sum_{t=1}^M \optTwot \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_capacity}\\
    && \crr \cdot r_2 \cdot C &\leq \left(\optOneOne + \optOneTwo \right) \cdot r_1 + \left( \sum_{t=1}^M \optTwot \right) \cdot r_2 \label{align:Ic_revenue}\\
                      &   & \crr \cdot r_2 \cdot C                & \leq \optOneTwo \cdot r_1 + \optupper_{2,2} \cdot r_2 \label{align:Ib_revenue} & \text{if $M = 1$}\\
                      & & {\color{black} s_{i, t}} & {\color{black}\ge 0\, ,\quad  \crr \ge 0}\, &i\in [3], t\in [2]
  \end{align}
\end{theorem}
%{\color{red} let's make sure in all the LP's, we state the non-negativity constraints. I did it above per the referees' comments. But, the equations are not well aligned. Could you please fix this?}
%Note that in LP \ref{3_class_ub} and all other LPs presented in this paper, we assume that all decision variables are non-negative.
Next, we present a proof sketch of Theorem \ref{thm:3_type_upper_bound}. The complete proof of this theorem and the proof of all other statements in this section are presented in Section \ref{secproofthree}.

\begin{proof}{Proof Sketch of Theorem \ref{thm:3_type_upper_bound}.} %{\color{red}please check out the shortened version.}
  A fundamental limitation of a non-anticipating (online) algorithm is that it cannot differentiate between two arrival sequences $I$ and $I'$ until their first divergence. Leveraging this, we structure our upper bounds using overlapping multi-period arrival sequences $\mathcal{I}$, and stipulate conditions for a $\crr$-competitive algorithm $\alg$ concerning each sequence $\{I_t\}_{t \in [T]} \in \mathcal{I}$. These conditions, when expressed as an LP, allow us to maximize $\crr$ to derive our upper bound.

  Illustratively, for $K = 3$, $M = 1$, and $C = 3$, the arrival sequence is:
    \[
        \begin{array}{ll}
            I_1 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} & I_2 = \{ 2, 2, 2,\: 3, 3, 3  \}
        \end{array}
    \]
    Such an arrival sequence is difficult because lower reward agents arrive before higher reward ones, forcing an algorithm to commit to lower reward agents before knowing whether higher reward agents will arrive. We can define the following \textit{truncations} of $\{I_1, I_2\}$ which consist of abruptly ending the entire input sequence after a certain type of agent has arrived. For example, $\{I_1^2, I_2^2\}$ represents the truncation of $\{I_1, I_2\}$ where the entire 2-period input suddenly ends after type $2$ agents arrive in the first time period.
    \[\arraycolsep=1.4pt\def\arraystretch{1.5}
        \begin{array}{ll}
            I_1^1 = \{ 1, 1, 1\} \quad                                    & I_2^1 = \{  \}         \\
            I_1^2 = \{ 1, 1, 1, \: 2, 2, 2\} \quad                        & I_2^2 = \{  \}         \\
            I_1^3 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3\} \quad             & I_2^3 = \{  \}         \\
            I_1^4 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2^4 = \{2, 2, 2  \}  \\
        \end{array}
    \]


 We now give a sketch of how the constraints in \ref{3_class_ub} come about. Suppose we are given an algorithm $\alg$ which is $\crr$ competitive. Let $s_{i,t}$, $i \in [3], t \in [2]$, be the number of type $i$ agents that are serviced in period $t$ under $\alg$. Since types $2$ and $3$ are impatient, $s_{i,t}$ also represents the number of type $2$ and $3$ agents that $\alg$ accepts from $I_t$ for $t\in [2]$, while for type $1$, $s_{1,1} + s_{1,2}$ is the number of type $1$ agents that $\alg$ accepts from $I_1$. Since $\textsc{opt}_t(\{I_1, I_2\}) = r_3 \cdot C$, to be $\crr$-competitive, we must have  $\textsc{rew}_{\alg, t}(\{I_1, I_2\}) = r_1 \cdot s_{1,t} + r_2 \cdot s_{2,t} + r_3 \cdot s_{3,t} \geq \crr \cdot r_3 \cdot C$, which gives rise to constraint \eqref{align:Ia_revenue}. In addition, we certainly must have $s_{1,t} + s_{2,t} + s_{3,t} \leq C$, as given in \eqref{align:Ia_capacity}. We apply a similar reasoning to arrival sequences $\{I_1^1, I_2^1\}, \{I_1^2, I_2^2\}$ and $\{I_1^4, I_2^4\}$, to get the $\crr \cdot r_i \cdot C$ (for $i= 1$ or $2$) reward lower bounds in constraints \eqref{align:Id_revenue}, \eqref{align:Ic_revenue}, \eqref{align:Ic_capacity}, and \eqref{align:Ib_revenue}.\footnote{Note that $\{I^3_1, I^3_2\}$ is actually not useful as it would imply the constraint $r_1 \cdot s_{1,1} + r_2 \cdot s_{2,1} + r_3 \cdot s_{3,1} \geq \crr \cdot r_3 \cdot C$, which was already captured by $\{I_1, I_2\}$.} 
  \Halmos
\end{proof}

\iffalse
\begin{proof}{Proof Sketch of Theorem \ref{thm:3_type_upper_bound}.}
  In this proof sketch, we outline the general structure of all the upper bounds presented in this paper. Our upper bound construction takes advantage of the fact that any non-anticipating algorithm $\alg$ does not know the future, and therefore is unable to differentiate between two arrival sequences  $I$ and $I'$ until the first index at which they differ. Using this idea, we build our upper bounds around a collection of overlapping multi-period arrival sequences $\mathcal{I}$, and argue that any non-anticipating algorithm $\alg$ that claims to be $\crr$-competitive must satisfy certain conditions when dealing with each arrival sequence $\{I_t\}_{t \in [T]} \in \mathcal{I}$. We write down these conditions in terms of an LP, maximize the value of $\crr$, and get our upper bound.

  To demonstrate our idea, let us consider an example where $K = 3$, $M = 1$, and $C = 3$. Our proof can be extended to any value of $C$ and also for $M=2$. Consider the following arrival sequence $\{I_1, I_2\}$ over the course of $T=2$ time periods. 
    \[
        \begin{array}{ll}
            I_1 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2 = \{ 2, 2, 2,\: 3, 3, 3  \}
        \end{array}
    \]
    We can define the following \textit{truncations} of $\{I_1, I_2\}$ which consist of abruptly ending the entire input sequence after a certain type of agent has arrived. For example, $\{I_1^2, I_2^2\}$ represents the truncation of $\{I_1, I_2\}$ where the entire 2-period input suddenly ends after type $2$ agents arrive in the first time period.
    \[\arraycolsep=1.4pt\def\arraystretch{1.5}
        \begin{array}{ll}
            I_1^1 = \{ 1, 1, 1\} \quad                                    & I_2^1 = \{  \}         \\
            I_1^2 = \{ 1, 1, 1, \: 2, 2, 2\} \quad                        & I_2^2 = \{  \}         \\
            I_1^3 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3\} \quad             & I_2^3 = \{  \}         \\
            I_1^4 = \{ 1, 1, 1, \: 2, 2, 2, \:3, 3, 3 \} \quad & I_2^4 = \{2, 2, 2  \}  \\
        \end{array}
    \]
%  $\{I_1, I_2\}$ is chosen so that we send agents in ascending order of reward over 2 time periods, while making sure all agents can be served within 2 time periods (hence not having partially patient type $1$ in $I_2$). %Such an arrival sequence best captures the core challenge of online resource allocation: the tension between committing to lower reward agents early on and waiting for higher reward agents that might not arrive. 
  
{\color{red} removed a paragraph here.} The truncated arrival sequences $\{I_1^j, I_2^j\}$ for $j \in [4]$ demonstrate that achieving a high CR requires an algorithm, $\alg$, to effectively balance performance across both $\{I_1, I_2\}$ and $\{I_1^j, I_2^j\}$ sequences. Given the overlap in these sequences, any algorithm's response to them is interconnected. For instance, if $\alg$ accepts only type 3 agents in $\{I_1, I_2\}$, maximizing the reward, it would fail to earn any reward on sequence $\{I_1^1, I_2^1\}$, as its actions up to the arrival of type 1 agents would remain unchanged between the two sequences.

  Using the ideas from the example above, we now give a sketch of how the constraints in \ref{3_class_ub} come about. Suppose we are given an algorithm $\alg$ which is $\crr$ competitive. Let $s_{i,t}$, $i \in [3], t \in [2]$, be the number of type $i$ agents that are serviced in period $t$ under $\alg$. Since types $2$ and $3$ are impatient, $s_{i,t}$ also represents the number of type $2$ and $3$ agents that $\alg$ accepts from $I_t$, while for type $1$, $s_{1,1} + s_{1,2}$ is the number of type $1$ agents that $\alg$ accepts from $I_1$. Since $\textsc{opt}_t(\{I_1, I_2\}) = r_3 \cdot C$, to be $\crr$-competitive, we must have   $\textsc{rew}_{\alg, t}(\{I_1, I_2\}) = r_1 \cdot s_{1,t} + r_2 \cdot s_{2,t} + r_3 \cdot s_{3,t} \geq \crr \cdot r_3 \cdot C$, which gives rise to constraint \eqref{align:Ia_revenue}. In addition, we certainly must have $s_{1,t} + s_{2,t} + s_{3,t} \leq C$, as given in \eqref{align:Ia_capacity}. We apply a similar reasoning
  to arrival sequences $\{I_1^1, I_2^1\}, \{I_1^2, I_2^2\}$ and $\{I_1^4, I_2^4\}$, to get the $\crr \cdot r_i \cdot C$ (for $i= 1$ or $2$) reward lower bounds in constraints \eqref{align:Id_revenue}, \eqref{align:Ic_revenue}, \eqref{align:Ic_capacity}, and \eqref{align:Ib_revenue}.\footnote{Note that $\{I^3_1, I^3_2\}$ is actually not useful as it would imply the constraint $r_1 \cdot s_{1,1} + r_2 \cdot s_{2,1} + r_3 \cdot s_{3,1} \geq \crr \cdot r_3 \cdot C$, which was already captured by $\{I_1, I_2\}$.} 
  \Halmos
\end{proof}
\fi

We will now state two \po{} algorithms which achieve the $\crr_{up}$ CR from the upper bound, one for the case where $M =1$ and another for $M = 2$. Both of these optimal algorithms require us to first compute the upper bound presented above, get an optimal solution $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in [2]})$ and use some of these values as constants in the feasible polytopes $\feasibleMOne$ for $M = 1$ and $\feasibleMTwo$ for $M = 2$. We will require some properties of this optimal upper bound solution, which are described in Lemmas \ref{lemma:3_class_tight_properties} and \ref{lemma:3_type_additional_properties} in Appendix \ref{sec:lemma:3_class_tight_properties} and \ref{sec:lemma:3_type_additional_properties}. We highlight that the upper bound only characterizes an optimal algorithm's behavior against our constructed worst-case arrival sequences, not any arbitrary arrival sequences over $T$ periods. Nonetheless, we show that how to use the upper bound solution, which represents a particular way of dealing with the worst-case arrival sequence, to construct an optimal algorithm for any arrival sequence.

\subsubsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 1$}{M=1}}
With $M=1$, type $1$ agents are partially patient while types $2$ and $3$ are impatient. %Hence,  our state $\stateB$ contains 4 buckets as shown below:
%\[ \begin{array}{r|ccc}
 %   \text{Type}  & 1               & 2          & 3          \\ \hline
  %  \text{Row 1} & \bucketij{1}{1} & \bucket{2} & \bucket{3} \\
 %   \text{Row 2} & \bucketij{1}{2} &            &
  %\end{array} \]
Let  $\Delta_{i,j} \defeq r_i - r_j$ and $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ be the optimal solution to the upper bound LP \ref{3_class_ub}. We define our feasible polytope $\feasibleMOne$ as follows
\begin{align} \label{eq:feasibleMOne}  \feasible^{(3,1)} = \left\{ (\fbucketOneOne, \fbucketOneTwo, \fbucketTwo, \fbucketThree) \subset \mathbb{R}_+^4: \quad  \begin{array}{cll}
    \fbucketOneOne + \fbucketTwo + \fbucketThree                       & \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*                           &           \\
    \Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo & \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^* &           \\
    \fbucketOnei                                                       & \leq \optupper_{1,i}^*                                           & i \in [2]\end{array} \right\}\,.
\end{align}

\begin{theorem}[Optimality of \textsc{POLYRA} Algorithm with  Feasible  Polytope $\feasibleMOne$]
  \label{thm:opt_alg_M=1} When the number of types $K = 3$ and the number of partially patient types $M = 1$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the \po{} algorithm with feasible polytope $\feasibleMOne$ achieves a CR of $\crr_{up}$, and hence, is optimal. Here, $\crr_{up}$ %{\color{red} I think you are overloading notation $\crr^*$. Did not you use it for the nested algorithms both in the introduction and other parts of the paper. } 
  is the optimal objective value of the LP \ref{3_class_ub}.
\end{theorem}


\textbf{Discussion on Feasible Polytope $\feasibleMOne$.} %{\color{red} this discussion is shortened.}
We provide insight into the constraints of $\feasibleMOne$ and its achievement of a CR of $\crr_{up}$. The first constraint ensures no over-allocation in a time period, governed by $C$ as dictated by \eqref{align:Ia_capacity} in the LP \ref{3_class_ub}. It turns out that $\optupper_{1,1}^* + \optupper_{2,1}^* + \optupper_{3,1}^* = C$ always olds (see Lemma \ref{lemma:3_class_tight_properties}). The second constraint emphasizes accommodating type $3$ agents in $\bucketThree$, by limiting a linear combination of agents in buckets $\bucketOneOne$ and $\bucketTwo$. The last constraint ensures adequate space for types $2$ and $3$ by regulating the number of type $1$ agents.Interestingly, $\feasibleMOne$ isn't a nested polytope per Definition \ref{def:nested}. For achieving the optimal CR of $\crr_{up}$, the algorithm must consider a linear combination of agents in $\bucketOneOne$ and $\bucketTwo$, rather than their mere sum.

By employing our \po{} algorithm with polytope $\feasibleMOne$ on the critical arrival sequence from $\{I_1, I_2\}$ (as outlined in the proof sketch of Theorem \ref{thm:3_type_upper_bound}), the algorithm's performance aligns with the optimal solution $\{s_{i,t}^*\}$. Essentially, our \po{} algorithm replicates the upper bound for worst-case scenarios (achieving exactly the CR), and we show it does better for all other arrivals (Theorem \ref{thm:opt_alg_M=1}). Next, we delve into the polytope construction for three types when $M = 2$.

\iffalse
\textbf{Discussion on Feasible Polytope $\feasibleMOne$.}
Here, we give some intuition about the constraints of $\feasibleMOne$ and why it achieves a CR of $\crr_{up}$. The first constraint, i.e., $\fbucketOneOne + \fbucketTwo + \fbucketThree \leq s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$  simply enforces that we do not allocate more resources in a time period than $s_{1,1}^* + s_{2,1}^* + s_{3,1}^*$ which is bounded above by $C$ as per constraint \eqref{align:Ia_capacity} of the upper bound LP \ref{3_class_ub}. In fact, as we show in property \ref{property:total_is_C} of Lemma \ref{lemma:3_class_tight_properties}, we actually have $\optupper_{1,1}^* + \optupper_{2,1}^* + \optupper_{3,1}^* = C$. The purpose of the second constraint, i.e., $\Delta_{3,1} \cdot \fbucketOneOne + \Delta_{3,2} \cdot \fbucketTwo \leq \Delta_{3,1} \cdot s_{1,1}^* + \Delta_{3,2} \cdot s_{2,1}^*$, is to leave enough space in bucket $\bucketThree$ for type $3$ agents, which we do so by enforcing that a linear combination of the number of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ is not too large. Finally, the last constraint, i.e., $\fbucketOnei \leq \optupper_{1,i}^*, i \in [2]$,  simply makes sure that our buckets do not contain too many type $1$ agents in order to leave enough room for the type $2$ and $3$ agents. 

Observe that the feasible polytope $\feasibleMOne$ is not a nested polytope as per Definition \ref{def:nested}. In particular, in order to obtain the optimal CR of $\crr_{up}$, the algorithm has to keep track of a linear combination of agents assigned to buckets $\bucketOneOne$ and $\bucketTwo$ (i.e., $\Delta_{3,1} \cdot \bucketOneOne + \Delta_{3,2} \cdot \bucketTwo$), rather than simply the sum of the agents assigned to these two buckets (i.e., $ \bucketOneOne + \bucketTwo$).

It can be shown that if we apply our \po{} algorithm with feasible polytope $\feasibleMOne$ to the worst-case arrival sequence from  $\{I_1, I_2\}$ as defined in the proof sketch of Theorem \ref{thm:3_type_upper_bound}, then the behavior of this algorithm will exactly correspond to the optimal solution $\{s_{i,t}^*\}$ in that our algorithm will serve exactly $s_{i,t}^*$ agents of type $i$ in period $t \in [2]$. In this way, our \po{} algorithm \textit{mimics} the upper bound when it encounters the worst-case arrival sequence.  Theorem \ref{thm:opt_alg_M=1} shows that our algorithm also achieves this optimal CR on any arrival sequence, not just this worst-case arrival sequence. We now describe our polytope construction for three types when $M = 2$.
\fi

\subsubsection{Optimal Three Type Algorithm for \texorpdfstring{$M = 2$}{M=2}}
With $M=2$, types $1,2$ agents are partially patient while type $3$ agents are impatient. %Hence, our state $\stateB$ contains 5 buckets as shown below:
%\[ \begin{array}{r|ccc}
%    \text{Type}   & 1               & 2               & 3          \\ \hline
 %   \text{Type 1} & \bucketij{1}{1} & \bucketij{2}{1} & \bucket{3} \\
  %  \text{Type 2} & \bucketij{1}{2} & \bucketij{2}{2} &
  %\end{array} \]
To construct the optimal algorithm for three types with two partially patient types, we  first compute the optimal solution $\left(\crr_{up}, \{s_{i,t}^*\}_{i \in [3], t \in [2]} \right)$ from the upper bound LP \ref{3_class_ub} in Theorem \ref{thm:3_type_upper_bound} and use it to construct our polytope $\feasibleMTwo$, which is defined in the following theorem.

\begin{theorem}[Optimal Algorithm for $K=3$ and $M=2$]
  \label{theorem:three_type_M=2}
 When the number of types $K = 3$ and the number of partially patient types $M = 2$, with $r_1< r_2< r_3$, and  per-period capacity $C$,  the nested \po{} algorithm with the {nested} polytope $\feasibleMTwo$, defined below, achieves a CR of $\crr_{up}$, and hence, is optimal:
  \begin{equation}\label{feasibleMTwo}
    \feasible^{(3,2)} \defeq \nestedPolyra\left(\frac{1}{2} \cdot (\optupper_{1,1}^* + \optupper_{1,2}^* ), \frac{1}{2} \cdot \left( \optupper_{1,1}^* + \optupper_{1,2}^* + \optupper_{2,1}^* +\optupper_{2,2}^*  \right)  , C \right) \, .
  \end{equation}
  Here, $(\crr_{up}, \{\optupper_{i,t}^*\}_{i\in[3], t\in[2]})$ is the optimal solution to the upper bound LP \ref{3_class_ub} and nested polytopes $\nestedPolyra$ are defined in Definition \ref{def:nested}.
\end{theorem}

\textbf{Discussion on the nested polytope $\feasibleMTwo$ and the optimal algorithm.} 
For two partially patient types ($M=2$), the optimal strategy is a straightforward nested \po{} algorithm, as indicated by Definition \ref{def:nested}. One can show that if we apply our \po{} algorithm with feasible polytope $\feasibleMTwo$ to the corresponding worst-case arrival sequence for $M = 2$, our \po{} algorithm will exactly serve $s_{i,t}^*$ agents of type $i\in[3]$ in time period $t\in [2]$.  This approach effectively mirrors the upper bound, ensuring our algorithm's $\crr_{up}$-competitiveness on worst-case arrival sequences.  To verify the nested polytope's CR of $\crr_{up}$, we use Theorem \ref{theorem:polyra_nested_performance} that utilizes an LP to characterize  the CR of any nested polytope.

While $\feasibleMOne$ is not a nested polytope, $\feasibleMTwo$ is. Recall from the earlier discussion that $\feasibleMOne$ is not nested because it has a constraint of the form $c_1 \cdot b_{1,1} + c_2 \cdot b_2 \leq c_3$ where $c_1 \neq c_2$. On the other hand, all of  $\feasibleMTwo$'s constraints involve a linear combination of variables with coefficients all equal to $1$. This can be explained by the following intuition: Both polytopes $\feasibleMOne$ and $\feasibleMTwo$ have constraints which make sure that we do not accept too many type $1$ or $2$ agents, thus making sure enough space is reserved for type $3$ agents. When type $1$ is partially patient and type $2$ is not (i.e. $M = 1$), this constraint is of the form $\Delta_{3,1} \cdot b_{1,1} + \Delta_{3,2} \cdot b_{2}$ where the coefficients $\Delta_{3,1}\neq \Delta_{3,2}$. This is because type $1$ and $2$ differ in their flexibility so our linear combination must weigh the two differently. On the other hand, when both type $1$ and type $2$ are partially patient (i.e $M = 2$), restricting the simple sum of $b_{1,1}$ and $b_{2,1}$ is sufficient.


\iffalse
\textbf{Discussion on the nested polytope $\feasibleMTwo$ and the optimal algorithm.} With two partially patient types (i.e., $M=2$), the optimal algorithm takes the form of a simple nested \po{} algorithm as per Definition \ref{def:nested}. Just like with 1 partially patient type, one can show that if we apply our \po{} algorithm with feasible polytope $\feasibleMTwo$ to the corresponding worst-case arrival sequence for $M = 2$, our \po{} algorithm will exactly serve $s_{i,t}^*$ agents of type $i\in[3]$ in time period $t\in [2]$. In this sense, we again mimic our upper bound solution as a template for making sure our algorithm is $\crr_{up}$-competitive against the worst-case arrival. It turns out that this worst-case arrival sequence is indeed the worst-case as achieving a $\crr_{up}$ CR on it implies a $\crr_{up}$ CR on all arrival sequences. To prove that such a nested polytope achieves the desired CR of $\crr_{up}$, we will apply Theorem \ref{theorem:polyra_nested_performance}, which uses an LP to characterize the CR of \textit{any} nested polytope, including ones for $K > 3$ types.

While $\feasibleMOne$ is not a nested polytope, $\feasibleMTwo$ is. Recall from the earlier discussion that $\feasibleMOne$ is not nested because it has a constraint of the form $c_1 \cdot b_{1,1} + c_2 \cdot b_2 \leq c_3$ where $c_1 \neq c_2$. On the other hand, all of  $\feasibleMTwo$'s constraints involve a linear combination of variables with coefficients all equal to $1$. This can be explained by the following intuition: Both polytopes $\feasibleMOne$ and $\feasibleMTwo$ have constraints which make sure that we do not accept too many type $1$ or $2$ agents, thus making sure enough space is reserved for type $3$ agents. When type $1$ is partially patient and type $2$ is not (i.e. $M = 1$), this constraint is of the form $\Delta_{3,1} \cdot b_{1,1} + \Delta_{3,2} \cdot b_{2}$ where the coefficients $\Delta_{3,1}\neq \Delta_{3,2}$. This is because type $1$ and $2$ differ in their flexibility so our linear combination must weigh the two differently. On the other hand, when both type $1$ and type $2$ are partially patient (i.e $M = 2$), restricting the simple sum of $b_{1,1}$ and $b_{2,1}$ is sufficient.
\fi

